Neural signature kernels as infinite-width-depth-limits of controlled ResNets

Motivated by the paradigm of reservoir computing, we consider randomly initialized controlled ResNets defined as Euler-discretizations of neural controlled differential equations (Neural CDEs), a unified architecture which enconpasses both RNNs and ResNets. We show that in the infinite-width-depth limit and under proper scaling, these architectures converge weakly to Gaussian processes indexed on some spaces of continuous paths and with kernels satisfying certain partial differential equations (PDEs) varying according to the choice of activation function, extending the results of Hayou (2022); Hayou & Yang (2023) to the controlled and homogeneous case. In the special, homogeneous, case where the activation is the identity, we show that the equation reduces to a linear PDE and the limiting kernel agrees with the signature kernel of Salvi et al. (2021a). We name this new family of limiting kernels neural signature kernels. Finally, we show that in the infinite-depth regime, finite-width controlled ResNets converge in distribution to Neural CDEs with random vector fields which, depending on whether the weights are shared across layers, are either time-independent and Gaussian or behave like a matrix-valued Brownian motion.

==> 1-Introduction.tex <==
\section{Introduction}

\subsection{Related work}

\begin{itemize}

\item Signatures and reservoir computing
    \begin{itemize}
        \item Signatures and rough paths \cite{FrizVictoir, lyons2014rough, friz2020course, chevyrev2016primer, lyons2007differential, kidger2019deep}
        \item Randomised signatures \cite{cuchiero2021discrete, cuchiero2021expressive, compagnoni2022randomized}
    \end{itemize}


\item Kernels and dynamical systems
    \begin{itemize}
        \item Signature kernel \cite{kiraly2019kernels, salvi2021signature, cass2021general, lemercier2021distribution}
        \item GPs with signature covariances \cite{toth2020bayesian, lemercier2021siggpde}
        \item Reservoir computing and kernels \cite{dong2020reservoir, gonon2022reservoir}
    \end{itemize}

 \item NNs and kernel methods: infinite-width, finite-depth 
      \begin{itemize}
          \item One layer \cite{neal2012bayesian}
          \item Feedforward \cite{lee2017deep, matthews2018gaussian}
          \item CNN \cite{novak2018bayesian, garriga2018deep}
          \item Tensor Programs \cite{yang2019scaling, Tensor_I}
      \end{itemize}

\item NNs and differential equations: infinite-depth, finite-width
    \begin{itemize}
          \item ResNet \cite{hayou2022infinite, marion2022scaling}
          \item RNN \cite{fermanian2021framing}
          \item Neural CDEs \cite{chen2018neural, kidger2020neural, morrill2021neural, salvi2021neural}
    \end{itemize}

\item Neural Tangent Kernel 
    \begin{itemize}
        \item Generic \cite{jacot2018neural, yang2020tensor}
        \item ResNet \cite{huang2020deep}
        \item RNN \cite{alemohammad2020recurrent}
    \end{itemize}

\end{itemize}


\subsection{Contributions and roadmap}

\begin{itemize}
    \item Motivated by reservoir computing, we consider several variants of recurrent ResNets that can be roughly classified into two categories: 1) the residual block change with each iteration, and 2) the residual block is shared across all the iterations (specify potential subcategories, such as matrix-valued BM).
    \item In the infinite-depth, finite-width regime these models "converge" to the popular class of Neural CDEs (be more precise).
    \item In the infinite-width, finite-depth regime these models converge to GPs satisfying some difference equations.
    \item In the infinite-width-depth regime, these architectures converge to Gaussian Processes with covariances satisfying certain differential-integral equations, varying according to the choice of non-linear activation function.
    \item Discuss difficulties in considering the infinite-depth-width regime and in which setting we can swap the two limits without changing the limiting object.
    \item Note that in the simplified setting where the chosen activation function is the identity, the limiting covariance agrees with the signature kernel and satisfies a classical Goursat PDE. 
    \item Discussion on NTK.
    \item Discussion on RKHS universality.
\end{itemize}









==> 2-Preliminaries.tex <==
\section{Preliminaries}

\subsection{Reservoir Computing}

The paradigm of reservoir computing is a neural networks approach that is similar to the way the brain works. The approach is designed to overcome some of the limitations of traditional neural networks, such as the need for a large number of training data.

The basic idea of reservoir computing is to create a neural network with a large number of nodes (i.e., a "reservoir") that are randomly connected. The input to the reservoir is fed through this random connection matrix, which acts to distort and amplify the input signal. This process creates a high-dimensional representation of the input that is then fed to a readout layer, which is trained to output the desired target signal.

The main advantage of reservoir computing is that it can learn from very little training data. This is because the reservoir nodes already have a rich representation of the input space, so the readout layer only needs to learn how to map from this representation to the target output.


In addition, reservoir computing is very efficient in terms of computational resources. The reservoir can be implemented using a simple neural network with a few hundred nodes, and it can be trained on a standard personal computer in a few minutes.

Finally, reservoir computing is robust to noise and changes in the input signal. This is because the random connection matrix creates a "smoothing" effect, which means that the reservoir will still be able to produce a reasonable output even if the input is corrupted by noise.

The main disadvantage of reservoir computing is that it is difficult to interpret the internal representation of the reservoir. This is because the connection matrix is random, so there is no simple way to understand how the nodes are connected.

Despite this disadvantage, reservoir computing has been shown to be very effective for a variety of tasks, including speech recognition, image classification, and time-series prediction.

\subsection{Neural Controlled Differential Equations}

The most natural \emph{generic} candidates for the vector fields $V^{\theta}_i(\cdot)$ are simple feed-forward neural networks $f_i(\cdot,\theta)$. 
Then Randomized Signature is the solution of a randomly initialized Neural Controlled Differential Equation (\cite{NCDEs}).

We are particularly interested, to begin with, in vector fields of the form 
\begin{equation}\label{NNs_v1}
    V_i^{\theta}(x) = A_i\varphi(x) + b_i
\end{equation}

where $\varphi : \R \to \R$ is a suitable analytic function like $ReLU, Id, tanh, sigmoid$ applied componentwise, and $A_i \in \R^{N\times N}$, $b_i \in \R^N$ have independent, normally distributed entries.

Since we expect Randomized Signatures to behave like the Signature as their dimension increases without bounds, we suspect their dot product to converge to some kernel associated to the Signature Kernel.
A result of this type would then shed light on the nature of the infinite width limit of continuous time ResNets (NCDEs).

\subsection{Kernel Methods}

We are interested in the composition 
\[
 \Phi := W \circ \psi
\]
where $\psi: \bX \to \R^{H}$ is a (randomly initialized) NN and $W : \R^{H} \to \R^{M}$ is a linear readout which needs to be learned.

\vspace{5pt}
\begin{itemize}
    \item Motivated by \emph{Reservoir Computing} literature.
    \item \textbf{Fast} physical implementations $\to$ \emph{time-critical} apllications.
    \item Lower computational/energy requirements $\to$ good  for environment and ease of implementation.
\end{itemize}

If $\D = \{ (x_i,y_i) \}_{i = 1, \dots, D} \subseteq \bX \times \R^{M}$ is a dataset of \emph{input-output} pairs and $\X, \mathcal{Y}$ its projections then we want $W$ to minimize
\[
    \mathcal{L}(W) = \norm{W\psi(\X) - \mathcal{Y}}^2_2
\]

where $\psi(\X) \in \R^{H \times D}$ is defined by $[\psi(\X)]_{\alpha}^i = [\psi(x_i)]_{\alpha}$ and, with abuse of notation, $\mathcal{Y} \in \R^{M \times D}$ is $[\mathcal{Y}]_{\beta}^i = [y_i]_{\beta}$.

\vspace{15pt}

If we apply gradient descend to the problem, with learning rate $\eta$, we obtain the following dynamics for the linear map:
\[
    \dot{W}_t = - \eta \big(  W_t \psi(\X) - \Y \big)\psi(\X)^{\top}
\]

Then the output at a point $x \in \bX$ during training is
\begin{equation*}  \begin{gathered}
    \Phi_t(x) = W_0 \psi(x) + (W_0\psi(\X) - \Y)(e^{-t \eta K(\X, \X)} - Id)K(\X, \X)^{-1} K(\X,x) 
\end{gathered}  \end{equation*}

where $K(\X,\X) \in \R^{D,D}$ is assumed invertible, defined by 
\[
[K(\X,\X)]_i^j = \psi(x_i)^{\top}\psi(x_j)
\]
and $K(\X,x) \in \R^{D}$ is defined similarly.


\vspace{15pt}

In particular at the "end of training" the result is explicitly given by
\[
    \Phi_{\infty}(x) = W_0 \psi(x) + (\Y- W_0\psi(\X))K(\X, \X)^{-1} K(\X,x) 
\]

If we sample the initial weights $W_0$ from a standard Gaussian then
we see that $\Phi_{\infty}$ defines a Gaussian Process on $\bX$ with 
mean 
\[
    \mu(x) = \Y K(\X, \X)^{-1} K(\X,x) 
\]
and covariance
\[
    C(x,x') = K(x,x') - K(\X,x)^{\top}K(\X, \X)^{-1}K(\X,x') 
\]


Thus $\Phi_{\infty}$ is distributed as the conditional expectation  $$\E[F | F(\X) = \Y]$$ of a Gaussian process $F \sim \mathcal{GP}(0,K)$ and $\mu \in \HK$ is the result of Kernel Regression (without Ridge regularization)!

It is therefore of outmost importance to understand the nature of the Kernels $K(x,y) := \psi(x)^{\top}\psi(y)$

\subsection{Notation}

Given a vector $v \in \R^n$ we write $[v]_{\alpha}$ for any of its components, similarly for a matrix $M \in \R^{n\times m}$ we write $[M]_{\alpha}^{\beta}$ for any of its entries. 
Let $\D = \{a = t_0 < \cdots < t_M = b\}$ be a partition of the interval $[a,b]$, we write $\norm{\D} := M$ and $|\D| := \max\limits_{l = 1,\dots, \norm{\D}} |t_{l} - t_{l-1}|$.




==> 3-Methods.tex <==
\section{Approach}

\subsection{Setup}

\subsubsection{The Data Space}
We are interested in studying time-series thus our data space will be
\[
    \bX := \{ x \in C^0 \cap BV([0,1];\R^d) : x(0) = 0 \text{ and } |dx| \ll \mathcal{L}^d \} = (W^{1,1}([0,1]))^d
\]
which is a normed path space with norm $\norm{\cdot}_{1-var}$.
This is the space of paths $x$ which can be written as 
\[
    x_t = \int_0^t \Dot{x}_s ds 
\]

for some $\Dot{x} \in L^1_{dt}([0,1];\R^d)$, Moreover with this identification we have 
\[
\norm{x}_{1-var, [0,t]} = \int_0^t |\Dot{x}_s| ds
\]
where $|\cdot| := \norm{\cdot}_{\R^d}$.

\textcolor{orange}{To address: we do not care about starting values.}


\subsubsection{The Feature Maps}

Fixed a map $\varphi: \R \to \R$, we consider \emph{Recurrent ResNets} $\psi_{\D}^N : \bX \to \R^N$ of type
\[
    \psi_{\D}^N(x) := \frac{1}{\sqrt{N}} Y^{\D,N}_1(x) \in \R^N
\]
where $Y^{\D,N} : \D \times \bX \to \R^N$ is defined by the following finite difference scheme:
\begin{equation*}
%\resizebox{\hsize}{!}{$
\begin{gathered}
    Y^{\D,N}_{t_{l}}(x) = Y^{\D,N}_{t_{l-1}}(x) + \sum_{k=1}^d \big( A_{k,l} \cdot \varphi(Y^{\D,N}_{t_{l-1}}(x)) + b_{k,l} \big) \Delta x^k_{t_l}
    \\
    Y^{\D,N}_0(x) = Y_0 \in \R^N \text{ and }  \Delta x^k_{t_l} = (x^k_{t_{l}}-x^k_{t_{l-1}}) \in \R
\end{gathered}
%$}
\end{equation*}

with $A_{k,l} \in \R^{N \times N}$, $b_{k,l} \in \R^N$, $\D$ partition of $[0,1]$ and $\varphi$ applied componentwise. 
The matrices and vectors $Y_0, A_{k,l}, b_{k,l}$ are sampled from normal distributions soon to be specified.

\begin{comment}
    \begin{equation*}
    %\resizebox{\hsize}{!}{$
    \begin{gathered}
        Y^{\D}_0(x) = Y_0(\theta) \in \R^N
        \\
        Y^{\D}_{t_{l}}(x) = Y^{\D}_{t_{l-1}}(x) + \sum_{k=1}^d V_{k,l}(Y^{\D}_{t_{l-1}}(x);\theta)\cdot(x^k_{t_{l}}-x^k_{t_{l-1}})
    \end{gathered}
    %$}
    \end{equation*}
    with output
    \[
        \sprod{v(\theta)}{Y^{\D}_{1}(x)}_{\R^N} \in \R
    \]
    
    where $x \in \bX := \textcolor{orange}{\{ x \in BV([0,1];\R^d) : ??? \}}$ is an input, $\D := \{0=t_0 < t_1 < \cdots < t_{\norm{\D}} = 1\}$ is a partition of $[0,1]$, $\theta \in \R^{d_{\theta}}$ are the parameters, $Y_0: \R^{d_{\theta}} \to \R^N$ is the initial value, $V_{k,l} : \R^N \times \R^{d_{\theta}} \to \R^N$ are the continuous vector fields defining the layer and $v: \R^{d_{\theta}} \to \R^N$.
    
    The most natural \emph{generic} candidates for the $V_{k,l}$ are feed-forward neural networks with weights given by $\theta$.
    For simplicity our setup will be the following:
    
    \begin{equation}\label{NNs_v1}
    \begin{gathered}
        V_{k,l}(x;\theta) = A^{\theta}_{k,l} \cdot \varphi(x) + b^{\theta}_{k,l}
        \\
        Y_0(\theta) = Y^{\theta}_0
        \\
        \theta = (v^{\theta},Y^{\theta}_0, \{A^{\theta}_{k,l},b^{\theta}_{k,l}\})
    \end{gathered}
    \end{equation}
    
    where $\varphi : \R \to \R$ is a suitable function like $ReLU, Id, tanh, sigmoid$ applied \emph{componentwise}, $A^{\theta}_{k,l} \in \R^{N\times N}$, $b^{\theta}_{k,l} \in \R^N$. At initialization $\theta$ is sampled from a distribution $\mu$ on $\R^{d_{\theta}}$.
\end{comment}

We are thus considering random, non-linear, \emph{reservoirs} \tocite defined as solutions of random dynamical systems driven by the input data.

\vspace{5pt}
Our goal is to understand the quantities
\[
    K^{\D,H}(x,y) := \E[ \psi_{\D}^N(x)^T \psi_{\D}^N(y)]
\]
where the expectation is taken over all parameters $Y_0, A_{k,l}, b_{k,l}$.

\vspace{5pt}

An explicit understanding of such an object for fixed $H$ is out of our scope, it's extremely complex due to the full dependencies between layers. Due to the \emph{Law of Large Numbers} these dependencies are "washed off " as $N \to \infty$, a regimen well known in the literature as the \emph{NNGP Limit}. 

\vspace{5pt}
The formalism of \emph{Tensor Programs} (\cite{Tensor_I}) allows us (most of the times) to explicitly characterize the limiting object.

\begin{comment}
    Our main objective is understanding the nature of the Infinite-Width-Then-Infinite-Depth Limit of such objects, in other words we want to make rigorous sense of the following distributional limit:
    \[
        \lim_{|\D| \to 0}\lim_{N \to \infty} \sprod{v}{Y^{\D}_{1}(\cdot)}_{\R^N} \in \R
    \]
    
    We are going to do so by proving this limit to be a Gaussian Process and by characterizing its covariance function (which will be indexed by path space $\bX$). \textcolor{orange}{Distribution on which space?}
\end{comment}

\subsection{The time inhomogeneous case}\label{SubSec:TimeIndep}

One of the usual simplifying assumptions made in the literature \tocite is that of sampling the entries of $A_{k,l}$ and $b_{k,l}$ independently in the depth $l$, since $l$ parametrizes time we will say that such sampling is \emph{time-independent}. 

More concretely, in this subsection we are going to understand what happens when:
\[
    [A_{k,l}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{\sigma_{A}^2}{N(t_l - t_{l-1})}), [Y_0]_{\alpha}\sim \mathcal{N}(0,\sigma_{Y_0}^2)
    \hspace{5pt} and \hspace{5pt} 
    [b_{k,l}]_{\alpha} \sim \mathcal{N}(0,\frac{\sigma_b^2}{(t_l - t_{l-1})})
\]
independently, with $\sigma_{A},\sigma_{Y_0} > 0$ , $\sigma_{b} \geq 0$ and $\D = \{0=t_0 < t_1 < \dots < t_{\norm{\D}} \}$.

\subsubsection{The Limit}

Fix partitions $\{\D_M\}_{M \in \N}$ of $[0,1]$ with $|\D_M| \downarrow 0$. We write $Y^{M,N}$ for $Y^{\D_M, N}$ for ease of notation.

\begin{theorem}
    Assume the activation function $\varphi$ to be Lipschitz. Let $\rho_M(t) := \sup \{ s \in \D_M : s \leq t\}$ and $x \in \bX \cap C^1$.
    Then the process $X^{M,N}_t := Y^{M,N}_{\rho_M(t)}(x)$ converges in distribution, as $M \to \infty$, to the solution of the following SDE
    \begin{equation}
    \begin{gathered}
        dX_t = \sum_{k=1}^d \frac{\sigma_A}{\sqrt{N}} \Dot{x}^k_t dW^k_t [\varphi(X_t)] + \sigma_b \dot{x}^k_t dB^k_t
        \\
        X_0 = Y_0
    \end{gathered}
    \end{equation}
    with $W^k_t \in \R^{N \times N}$ and $B^k_t \in \R^N$ are independent standard Brownian motions.
\end{theorem}


    \begin{equation}
    \begin{gathered}
        X_T = X_0 + \sum_{k=1}^d  \int_0^T
        \frac{\sigma_A}{\sqrt{N}} \Dot{x}^k_t dW^k_t [\varphi(X_t)] + \sigma_b \dot{x}^k_t dB^k_t
        \\
        X_0 = Y_0
        \\
        \\
        \E[ \frac{X_T \cdot X'_T}{N}] = \sigma_{Y_0}^2 + 
        \int_0^T
        \big( 
        \sigma_A^2 \E[\frac{\varphi(X_t) \cdot \varphi(X'_t)}{N}] + \sigma_b^2 \big)
        \sprod{\Dot{x}_t}{\Dot{x}'_t}_{\R^d} dt
    \end{gathered}
    \end{equation}


\begin{algorithm}[tbh]
    \caption{$Y^{N,M}_1$ as Nestor program}
    \label{Algo:TimeDep}
    \begin{algorithmic}
      \Require $Y^0: \Gtype(N)$ \Comment{initial value}
      \Require $(b_{m,k})_{k = 1, \dots, d}^{m=1,\dots,\norm{\D_M}}: \Gtype(N)$ \Comment{biases}
      \Require $(A_{m,k})_{k = 1, \dots, d}^{m=1,\dots,\norm{\D_M}}: \Atype(N, N)$ \Comment{matrices}
      \Require $v: \Gtype(N)$ \Comment{readout layer weights}
      \\
      \For{$i = 1, \dots, n$}
          \State {\it // Compute $Y^{N,M}_1 (x_i)$  (here $ Y_0^{x_i}$ is to be read as $S_0$)}
          \\
          \For{$m = 1,\dots,\norm{\mathcal{D}_M}$}
              \For{$k = 1,\dots,d$}
                \State $\alpha^i_{m,k} := \varphi(Y^{x_i}_{m-1}): \Htype(N)$ \Comment{by Nonlin;}
                \State $\beta^i_{m,k} := A_{m,k} \alpha^i_{m,k} : \Gtype(N)$ \Comment{by Matmul;}
                \State $\gamma^i_{m,k} := \beta^i_{m,k} + b_{m,k}  : \Gtype(N)$ \Comment{by LinComb;}
              \EndFor
              \State $Y^{x_i}_{m} := Y^{x_i}_{m-1} + \sum_{k=1}^d \gamma^i_{m,k} [(x_i)^k_{t_m} - (x_i)^k_{t_{m-1}}]  : \Gtype(N)$ \Comment{by LinComb;}
          \EndFor
          \\
      \EndFor
      \\
      \Ensure $(v^T Y_{\norm{\mathcal{D}_M}}^{x_i} / \sqrt{N})_{i=1,\dots,n}$
    \end{algorithmic}
\end{algorithm}


\begin{proposition} \label{Prop:DiscreteIndepKernels}
The following \textcolor{orange}{convergence in distribution} holds:
\[
\sprod{v^N}{Y^{M,N}_{1}(\cdot)} \xrightarrow[]{N \to \infty} \mathcal{GP}(0,\sigma_v^2K^M)
\]
where the covariance function $K^M: \bX \times \bX \to \R$ is, given $x,y \in \bX$, the final value $K^M_{1}(x,y)$ of the following finite difference scheme on $\D_M \times \D_M$:

\begin{equation*}
%\resizebox{0.8\hsize}{!}{$
\begin{gathered}
    K^{M}_{t_{m}}(x,y) = K^{M}_{t_{m-1}}(x,y)
    + \sum_{k=1}^d  \Big( \sigma_A^2 
    \E_{Z \sim \mathcal{N}(0, \Sigma^{M}_{t_{m-1}}(x,y))}[ \varphi(Z_1) \varphi(Z_2) ]
    + {\sigma_b^2 } \Big)  \frac{\Delta x^k_{t_m} \Delta y^k_{t_m}}{t_{m} - t_{m-1}}
    \\
    = K^{M}_{t_{m-1}}(x,y)
    + \Big( \sigma_A^2 
    \E_{Z \sim \mathcal{N}(0, \Sigma^{M}_{t_{m-1}}(x,y))}
    [ \varphi(Z_1) \varphi(Z_2) ] + {\sigma_b^2 } \Big)  
    \sprod{\frac{\Delta x_{t_m}}{\Delta t_m}}{\frac{\Delta y_{t_m}}{\Delta t_m}}_{\R^d} \Delta t_m
    \\
    \text{with } K^{M}_{0}(x,y) = \sigma_{S_0}^2
\end{gathered}
%$}
\end{equation*}
where 
\begin{equation*}
%\resizebox{0.4\hsize}{!}{$
\begin{gathered}
    \Sigma^{M}_{t}(x,y) =  
    \begin{pmatrix}
        K^{M}_{t}(x,x) & K^{M}_{t}(x,y) \\
        K^{M}_{t}(x,y) & K^{M}_{t}(y,y)
    \end{pmatrix}
\end{gathered}
%$}
\end{equation*} 
\end{proposition}

Then finally

\begin{theorem}[SomeKers]
Let $\varphi: \R \to \R$ be \textcolor{red}{?}.
Randomly initialized ResNets $\sprod{v^N}{Y^{M,N}_1(x)}$ with fields of type \ref{NNs_v1} and weights drawn independently as 
\[
    \frac{1}{\sigma_{v}}[v^N]_{\alpha}, \frac{\sqrt{\Delta t^M_l}}{\sigma_{A}}[A^{M,N}_{k, l}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{1}{N}) 
    \hspace{5pt} and \hspace{5pt} 
    \frac{1}{\sigma_{Y_0}}[Y^N_0]_{\alpha},\frac{\sqrt{\Delta t^M_l}}{\sigma_{b}}[b^{M,N}_{k,l}]_{\alpha} \sim \mathcal{N}(0,1)
\]
converge in distribution, in the \emph{infinite-width-then-infinite-depth} limit, to a Gaussian Process $\mathcal{GP}(0,\sigma_v^2K^{\varphi})$ indexed on $\bX$ where the covariance $K^{\varphi}$ is the final value $K^{\varphi}_{1}$ of the following CDE on $[0,1]$
\begin{align*}
      &K^{\varphi}_{t} (x, y) =  \sigma_{S_0 }^2 
      +  \int_{\tau = 0}^{t} 
      \Big[ 
      \sigma_A^2 \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}^{x, y}_{\tau})} 
      [ \varphi(Z_1) \varphi(Z_2) ] 
      + 
      \sigma_b^2 
      \Big] 
     \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d}   d \tau 
\end{align*}
with 
\[ 
    {\Sigma}^{x, y}_{t,s} = 
     \left(\begin{array}{c}
       K^{\varphi}_{t} (x, x), K^{\varphi}_{t} (x, y)\\
       K^{\varphi}_{t} (x, y), K^{\varphi}_{t} (y, y)
     \end{array}\right) 
\]
\end{theorem}

From which follows

\begin{corollary}
    If $\sigma = id$, then 
    \[
    K^{id}_{t} (x, y) = \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big) \exp\big \{\sigma_A^2 \int_{\tau = 0}^t \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d} d\tau \big\} - \frac{\sigma_b^2}{\sigma_A^2}
    \]
\end{corollary}

\subsection{The time homogeneous case}\label{SubSec:TimeDep}

A more complex scenario is when $A_{k,l}$ and $b_{k,l}$ are constant in depth $l$ \emph{i.e.} when they are \emph{time-dependent}. 
In this subsection we are going to understand what happens when, for all $l$, we set $A_{k,l} = A_{k}$ and $b_{k,l} = b_{k}$ with :
\[
    [A_{k}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{\sigma_{A}^2}{N}), [Y_0]_{\alpha}\sim \mathcal{N}(0,\sigma_{S_0}^2)
    \hspace{5pt} and \hspace{5pt} 
    [b_{k}]_{\alpha} \sim \mathcal{N}(0,\sigma_b^2)
\]
independently, with $\sigma_{A},\sigma_{S_0} > 0$ and $\sigma_{b} \geq 0$.

\subsubsection{The Limit : $\varphi$-Signature Kernels}

Fix partitions $\{\D_M\}_{M \in \N}$ of $[0,1]$ with $|\D_M| \downarrow 0$. We write $S^{M,N}$ for $Y^{\D_M, N}$ to differentiate this from the previous time-independent case. In other words now 

\[
    S^{M,N}_{t_m}(x) = S_0 + \sum_{l=1}^m \sum_{k=1}^d \big( A_{k} \cdot \varphi(S^{N, M}_{t_{l-1}}(x)) + b_{k} \big) \Delta x^k_{t_l}
\]

\begin{lemma}
Let $v^N \in \R^N$ with i.i.d entries $[v]_{\alpha} \sim \mathcal{N}(0,\frac{\sigma_v^2}{N})$. Then, for any $t,s \in \D_M$
\[
    \E[\sprod{v^N}{S^{M,N}_{t}(x)}\sprod{v^N}{S^{M,N}_{s}(y)}] = \frac{\sigma_v^2}{N}\E[\sprod{S^{M,N}_{t}(x)}{S^{M,N}_{s}(y)}]
\]
\end{lemma}


Using the formalism of Tensor programs \cite{Tensor_I} we are first proving that 

\begin{proposition} \label{Prop:DiscretePhiKernels}
The following \textcolor{orange}{convergence in distribution} holds:
\[
\sprod{v^N}{S^{M,N}_{1}(\cdot)} \xrightarrow[]{N \to \infty} \mathcal{GP}(0,\sigma_v^2K^M)
\]
where the covariance function $K^M: \bX \times \bX \to \R$ is, given $x,y \in \bX$, the final value $K^M_{1,1}(x,y)$ of the following finite difference scheme on $\D_M \times \D_M$:

\begin{equation*}
%\resizebox{0.8\hsize}{!}{$
\begin{gathered}
    K^{M}_{t_{m},s_n}(x,y) = K^{M}_{t_{m-1},s_n}(x,y) + K^{M}_{t_m,s_{n-1}}(x,y) - K^{M}_{t_{m-1},s_{n-1}}(x,y)
    \\
    + \sum_{k=1}^d  \Big( \sigma_A^2 
    \E_{Z \sim \mathcal{N}(0, \Sigma^{M}_{t_{m-1},s_{n-1}}(x,y))}[ \varphi(Z_1) \varphi(Z_2) ]
    + \sigma_b^2 \Big)  \Delta x^k_{t_m} \Delta y^k_{s_n} 
    \\
    \text{with } K^{M}_{0,0}(x,y) = K^{M}_{0, s_n}(x,y) = K^{M}_{t_m, 0}(x,y) = \sigma_{S_0}^2
\end{gathered}
%$}
\end{equation*}
where 
\begin{equation*}
%\resizebox{0.4\hsize}{!}{$
\begin{gathered}
    \Sigma^{M}_{t, s}(x,y) =  
    \begin{pmatrix}
        K^{M}_{t,t}(x,x) & K^{M}_{t,s}(x,y) \\
        K^{M}_{t,s}(x,y) & K^{M}_{s,s}(y,y)
    \end{pmatrix}
\end{gathered}
%$}
\end{equation*} 
\end{proposition}

Then finally

\begin{theorem}[$\varphi$-SigKer]
Let $\varphi: \R \to \R$ be a linearly bounded, absolutely continuous map with exponentially bounded derivative.
Randomly initialized ResNets $\sprod{v^N}{S^{M,N}_1(x)}$ with fields of type \ref{NNs_v1} and weights drawn independently as 
\[
    \frac{1}{\sigma_{v}}[v^N]_{\alpha}, \frac{1}{\sigma_{A}}[A^N_k]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{1}{N}) 
    \hspace{5pt} and \hspace{5pt} 
    \frac{1}{\sigma_{S_0}}[S^N_0]_{\alpha},\frac{1}{\sigma_{b}}[b^N_k]_{\alpha} \sim \mathcal{N}(0,1)
\]
converge in distribution, in the \emph{infinite-width-then-infinite-depth} limit, to a Gaussian Process $\mathcal{GP}(0,\sigma_v^2K^{\varphi})$ indexed on $\bX$ where the covariance $K^{\varphi}$ is the final value $K^{\varphi}_{1,1}$ of the following CDE on $[0,1]\times[0,1]$
\begin{align*}
      &K^{\varphi}_{t, s} (x, y) =  \sigma_{S_0 }^2 
      +  \int_{\tau = 0}^{t} \int_{\sigma = 0}^{s} 
      \Big[ 
      \sigma_A^2 \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}^{x, y}_{\tau, \sigma})} 
      [ \varphi(Z_1) \varphi(Z_2) ] 
      + 
      \sigma_b^2 
      \Big] 
     \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
\end{align*}
with 
\[ 
    {\Sigma}^{x, y}_{t,s} = 
     \left(\begin{array}{c}
       K^{\varphi}_{t, t} (x, x), K^{\varphi}_{t, s} (x, y)\\
       K^{\varphi}_{t, s} (x, y), K^{\varphi}_{s, s} (y, y)
     \end{array}\right) 
\]
\end{theorem}

From which readily follows

\begin{corollary}
    If $\sigma = id$, then 
    \[
    K^{id}_{t, s} (x, y) = \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big) SigKer_{t,s}(\sigma_A x,\sigma_A y) - \frac{\sigma_b^2}{\sigma_A^2}
    \]
\end{corollary}

In particular it follows that 
\[
    K^{\D, N}(x,y) \xrightarrow[]{N \to \infty}  K^{\D}(x,y) \xrightarrow[]{|\D| \downarrow 0} K^{\varphi}(x,y) 
\]

\subsubsection{Reproducing Kernel Hilbert Spaces and $\varphi$-Signatures}

\begin{conjecture}
        Under suitable assumptions on $\varphi$, when restricted to a compact $\mathbf{C} \subseteq \bX$, the kernels $K^{\varphi}_{1,1} : \mathbf{C}  \times \mathbf{C}   \to \R$ are Universal
        \emph{i.e} the spaces $\mathcal{H}_{K^{\varphi}_{1,1}}$ are dense in $(C^0(\mathbf{C};\R), \norm{\cdot}_{\infty})$.
\end{conjecture}

\textcolor{orange}{Write it better!}

\vspace{5pt}
Idea: There exist feature maps $Sig_{\varphi} : \bX \to T((\R^d))$ such that 
\[
    K^{\varphi}_{1,1}(x,y) = \sprod{Sig_{\varphi} (x)}{Sig_{\varphi}(y)}_{T((\R^d))}
\]
and for $I = (i_1, \dots, i_n) \in \mathbb{W}_d$ 
\[
    Sig_{\varphi}^I(x) := \int_{0 < \tau_1 < \cdots < \tau_n < 1} \Phi^I((K^{\varphi}_{\tau_i, \tau_i}(x,x))_{i = 1}^n) dx^{i_1}_{\tau_1}\cdots dx^{i_n}_{\tau_n}
\]
where $\Phi^I : \R^n \to \R$ is an analytic map.

\subsubsection{Randomized Signatures}

It is natural to ask what happens if the depth limit is taken first.
If one goes to the limit $|\D| \downarrow 0$, under \textcolor{orange}{suitable assumptions on $\varphi$}, one gets the convergence of 
the networks $S^{N, M}$ to \emph{Randomized Signatures} (\cite{cuchiero2021expressive}), which are defined as the following CDEs
\begin{equation*}
%\resizebox{\hsize}{!}{$
\begin{gathered}
    S^{\varphi}_{t}(x) = S_0 + \sum_{k=1}^d \int_0^t \big( A_k \cdot \varphi(S^{\varphi}_{\tau}(x)) + b_k \big) dx_{\tau}^k
\end{gathered}
%$}
\end{equation*}
 with $S_0 \in \R^N$, $A_k \in \R^{N \times N}$, $b_k \in \R^N$, $\varphi: \R \to \R$ applied componentwise. Entries are independently sampled just as before. 

 In particular
 \[
    K^{\D, N}(x,y)  \xrightarrow[]{|\D| \downarrow 0} K^{N}(x,y) := \frac{1}{N}\E[S^{\varphi}_{1}(x)^{T}S^{\varphi}_{1}(y)]
 \]

 What happens if we then let $N \to \infty$? Do we end up with the following commuting diagram?

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.3]{Pictures/commuting.png}
    %\caption{Caption}
    %\label{fig:my_label}
\end{figure}

\begin{theorem}
        In the case $\varphi = id$ 
        \[
            \frac{1}{N}\sprod{S^{id}_t(x)}{S^{id}_s(y)}_{\R^N} 
            \xrightarrow[N \to \infty]{\mathbb{L}^2}
            K^{id}_{t,s}(x,y)
        \]

        moreover the convergence is of order $\mathcal{O}(\frac{1}{N})$
\end{theorem}


==> 4-Experiments.tex <==
\section{Experiments}

==> 5-Conclusions.tex <==
\section{Conclusions}

==> Appendices.tex <==

\iffalse
\section{Kernel Methods and SGD}

We are interested in the composition 
\[
 \Phi := W \circ \psi
\]
where $\psi: \bX \to \R^{H}$ is a (randomly initialized) NN and $W : \R^{H} \to \R^{M}$ is a linear readout which needs to be learned.

\vspace{5pt}
\begin{itemize}
    \item Motivated by \emph{Reservoir Computing} literature.
    \item \textbf{Fast} physical implementations $\to$ \emph{time-critical} apllications.
    \item Lower computational/energy requirements $\to$ good  for environment and ease of implementation.
\end{itemize}

If $\D = \{ (x_i,y_i) \}_{i = 1, \dots, D} \subseteq \bX \times \R^{M}$ is a dataset of \emph{input-output} pairs and $\X, \mathcal{Y}$ its projections then we want $W$ to minimize
\[
    \mathcal{L}(W) = \norm{W\psi(\X) - \mathcal{Y}}^2_2
\]

where $\psi(\X) \in \R^{H \times D}$ is defined by $[\psi(\X)]_{\alpha}^i = [\psi(x_i)]_{\alpha}$ and, with abuse of notation, $\mathcal{Y} \in \R^{M \times D}$ is $[\mathcal{Y}]_{\beta}^i = [y_i]_{\beta}$.

\vspace{15pt}

If we apply gradient descend to the problem, with learning rate $\eta$, we obtain the following dynamics for the linear map:
\[
    \dot{W}_t = - \eta \big(  W_t \psi(\X) - \Y \big)\psi(\X)^{\top}
\]

Then the output at a point $x \in \bX$ during training is
\begin{equation*}  \begin{gathered}
    \Phi_t(x) = W_0 \psi(x) + (W_0\psi(\X) - \Y)(e^{-t \eta K(\X, \X)} - Id)K(\X, \X)^{-1} K(\X,x) 
\end{gathered}  \end{equation*}

where $K(\X,\X) \in \R^{D,D}$ is assumed invertible, defined by 
\[
[K(\X,\X)]_i^j = \psi(x_i)^{\top}\psi(x_j)
\]
and $K(\X,x) \in \R^{D}$ is defined similarly.


\vspace{15pt}

In particular at the "end of training" the result is explicitly given by
\[
    \Phi_{\infty}(x) = W_0 \psi(x) + (\Y- W_0\psi(\X))K(\X, \X)^{-1} K(\X,x) 
\]

If we sample the initial weights $W_0$ from a standard Gaussian then
we see that $\Phi_{\infty}$ defines a Gaussian Process on $\bX$ with 
mean 
\[
    \mu(x) = \Y K(\X, \X)^{-1} K(\X,x) 
\]
and covariance
\[
    C(x,x') = K(x,x') - K(\X,x)^{\top}K(\X, \X)^{-1}K(\X,x') 
\]


Thus $\Phi_{\infty}$ is distributed as the conditional expectation  $$\E[F | F(\X) = \Y]$$ of a Gaussian process $F \sim \mathcal{GP}(0,K)$ and $\mu \in \HK$ is the result of Kernel Regression (without Ridge regularization)!

It is therefore of outmost importance to understand the nature of the Kernels $K(x,y) := \psi(x)^{\top}\psi(y)$


\newpage
\fi

\appendix
\onecolumn


\section{Preliminaries}

In this section we are going to state some preliminary results and considerations which we are going to refer to through the entirety of the text. Since we are mainly interested in studying time-series, our data space will be a space of paths, more specifically we are going to consider the space
\[
    \bX := \{ x \in C^0([0,1];\R^d) : x(0) = 0, \exists \Dot{x} \in L^2([0,1]; \R^d) \}
\]
\emph{i.e.} $\bX$ is the space of continous paths which have a square integrable derivative. 
$\bX$ is the closed subset of the Sobolev space $\big( W^{1,2}([0,1]) \big)^d$ made of those functions starting at the origin.


Note that every path $x \in \bX$ can be uniquely written as 
\[
    x_t = \int_0^t \Dot{x}_s ds 
\]
thus it naturally corresponds to the space $L^2([0,1]; \R^d)$ trough the identification $x \mapsto \Dot{x}$.
This identification gives the space the natural norm $\norm{x}_{\bX} = \norm{\Dot{x}}_{L^2}$.

This norm is equivalent to the induced norm from $\big( W^{1,2}([0,1]) \big)^d$ since 
\begin{equation*}
    \begin{gathered}
        \norm{\Dot{x}}^2_{L^2} \leq \norm{x}^2_{W^{1,2}} = \int_0^1 |x_s|^2 ds + \norm{\Dot{x}}^2_{L^2}
        =  \int_0^1 |\int_0^s \Dot{x}_r dr|^2 ds + \norm{\Dot{x}}^2_{L^2} \\
        \leq \int_0^1 \int_0^1 |\Dot{x}_r|^2 dr ds + \norm{\Dot{x}}^2_{L^2} = 2\norm{\Dot{x}}^2_{L^2}
    \end{gathered}
\end{equation*} for $x \in \bX$, hence $(\bX, \norm{\cdot}_{\bX})$ is a Banach space.

Moreover one can easily see that every $x \in \bX$ has bounded variation and 
\[
\norm{x}_{1-var, [0,1]} = \int_0^1 |\Dot{x}_t| dt \leq \sqrt{\int_0^1 |\Dot{x}_t|^2 dt} = \norm{x}_{\bX}
\]

\subsection{Assumption on  activation functions}
Now we are going to state the main assumptions on the activation function $\varphi: \R \to \R$ and prove some important technical results of which we will frequently make use in the following sections. 
We will particularly be interested in how regularity assumptions made on $\varphi$ influence the regularity of the expectations of Equation (\ref{eqn:hom_kernel}) and (\ref{eqn:inhom_kernel}). 

Here are the crucial assumptions we make on the activation:

\begin{assumption}\label{assumption:linear-bound}
  The activation function $\varphi: \R \to \R$ is linearly bounded  \emph{i.e.} such that
  there exist some $M > 0$ such that  $| \varphi (x) | \leq M (1 + | x |)$.
\end{assumption}

\begin{assumption}\label{assumption:exp-bounded-der}
  The activation function $\varphi: \R \to \R$ is absolutely continuous and with exponentially bounded derivative.
\end{assumption}

\vspace{10pt}
\begin{lemma}\label{app:lipR_to_lipRn}
    If the activation function $\varphi: \R \to \R$ is $K$-Lipschitz then its componentwise extension $\varphi: \R^n \to \R^n$ is $K$-Lipschitz too.
    If the activation function $\varphi: \R \to \R$ is $M$-linealy-bounded then its componentwise extension is $\sqrt{2n}M$-linealy-bounded.
\end{lemma}
\begin{proof}
    Regarding the first proposition, for $x,y \in \R^n$ we have
    \begin{equation*}
        \begin{gathered}
            |\varphi(x)-\varphi(y)|^2_{\R^n} = \sum_{i=1}^n |\varphi(x_i)-\varphi(y_i)|^2 \leq \sum_{i=1}^n K^2|x_i-y_i|^2 = K^2 |x-y|^2_{\R^n}
        \end{gathered}
    \end{equation*}

    Concerning the second, notice how
    \begin{equation*}
        \begin{gathered}
            |\varphi(x)|^2_{\R^n} = \sum_{i=1}^n |\varphi(x_i)|^2 \leq \sum_{i=1}^n M^2(1+|x_i|)^2 \leq 2M^2 \sum_{i=1}^n (1+|x_i|^2)
            \\
            = 2M^2(n+|x|^2_{\R^n}) \leq 2nM^2(1+|x|^2_{\R^n})
        \end{gathered}
    \end{equation*}
    thus $|\varphi(x)|_{\R^n} \leq \sqrt{2n}M(1+|x|_{\R^n})$ since $\sqrt{1 + \epsilon} \leq 1 + \sqrt{\epsilon}$ for all $\epsilon \geq 0$.
\end{proof}

\vspace{10pt}
\begin{definition}
    Let $PSD_2$ denote the set of $2\times 2$ positive semidefinite matrices, this means 
    \[
    PSD_2 := \{ \Sigma \in \R^{2 \times 2} :  \Sigma =  \Sigma^{T} ; ([\Sigma]_1^2)^2 \leq [\Sigma]_1^1 [\Sigma]_2^2 ; 0 \leq [\Sigma]_1^1 \wedge [\Sigma]_2^2 \}
    \]
    For a fixed $R > 0$ we define the space
    \[
        PSD_2(R) := \{ \Sigma \in PSD_2 : \frac{1}{R} \leq [\Sigma]_1^1, [\Sigma]_2^2 \leq R\}
    \]
\end{definition}

\begin{lemma}\label{lemma:split_on_PSD_R}
Under {\tmstrong{Assumption \ref{assumption:exp-bounded-der}}} and for any $R>0$ the map
  \begin{eqnarray*}
    & V_{\varphi} : \tmop{PSD}_2 (R) \rightarrow \R & \\
    & \Sigma \mapsto \mathbb{E}_{(Z_x, Z_y) \sim \mathcal{N} (0,
    \Sigma)} [\varphi (Z_x) \varphi (Z_y)] & 
  \end{eqnarray*}
 is $\kappa_R$-Lipschitz for some $\kappa_R > 0$, i.e.
  \[
  |V_{\varphi} (\Sigma) - V_{\varphi} (\tilde{\Sigma})|  \leq  \kappa_R \| \Sigma -
    \tilde{\Sigma} \|_{\infty} 
  \]
\end{lemma}

\begin{proof}
    This is the content of Theorem F.4 in \cite{novak2018bayesian}.
\end{proof}

\begin{proposition}
  Under {\tmstrong{Assumption \ref{assumption:linear-bound}}}, there exists a {positive} constant $\tilde{M}>0$ such that 
  \[ | V_{\varphi} (\Sigma) | \leq \tilde{M} \left( 1 + \sqrt{[\Sigma]_1^1} \right)
     \left( 1 + \sqrt{[\Sigma]_2^2} \right) \]
\end{proposition}

\begin{proof}
  In fact given a PSD matrix $\Sigma \in \mathbb{R}^{2 \times 2}$ we have
  \[ \Sigma = A A^T \]
  where
  \[ A = \left(\begin{array}{c}
       \alpha, 0\\
       \beta \gamma, \beta \sqrt{1 - \gamma^2}
     \end{array}\right) \]
  with
  \[ \alpha = \sqrt{[\Sigma]_1^1}, \beta = \sqrt{[\Sigma]_2^2} \infixand
     \gamma = \frac{[\Sigma]_1^2}{\sqrt{[\Sigma]_1^1 [\Sigma]_2^2}} \]
  Then {it can be easily observed that}
  \begin{eqnarray*}
    \mathbb{E}_{(Z_x, Z_y) \sim \mathcal{N} (0, \Sigma)} [\varphi (Z_x)
    \varphi (Z_y)] & = & \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})}
    \left[ \varphi (\alpha Z_1) \varphi \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right]
  \end{eqnarray*}
  so that
\begin{equation*}
\resizebox{\hsize}{!}{$
\begin{gathered}
    | V_{\varphi} (\Sigma) |  =  \left| \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} \left[ \varphi (\alpha Z_1) \varphi \left( \beta \left( \gamma
    Z_1 + \sqrt{1 - \gamma^2} Z_2 \right) \right) \right] \right|
    \\
     \leq  \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} \left[ |
    \varphi (\alpha Z_1) | \left| \varphi \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right| \right]
    \\
     \leq  M^2 \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} \left[
    (1 + | (\alpha Z_1) |) \left( 1 + \left| \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right| \right) \right]
    \\
     =  M^2 \left[ 1 + \alpha \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} [| Z_1 |] + \beta \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} \left[ \left| \gamma Z_1 + \sqrt{1 - \gamma^2} Z_2 \right|
    \right]+ \alpha \beta \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})}
    \left[ | Z_1 | \left| \gamma Z_1 + \sqrt{1 - \gamma^2} Z_2 \right| \right]
    \right]
    \\
     \leq  M^2 \left[ 1 + (\alpha + \beta | \gamma |) \mathbb{E}_{Z
    \sim \mathcal{N} (0, \tmop{Id})} [| Z_1 |] + \beta \sqrt{1 -
    \gamma^2} \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} [| Z_2 |] +
    \alpha \beta | \gamma | \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} [| Z_1 |^2] + \alpha \beta \sqrt{1 - \gamma^2} \mathbb{E}_{Z
    \sim \mathcal{N} (0, \tmop{Id})} [| Z_1 Z_2 |] \right]
    \\
     \leq  \bar{M} \left( 1 + \alpha + \beta | \gamma | + \beta \sqrt{1 -
    \gamma^2} + \alpha \beta | \gamma | + \alpha \beta \sqrt{1 - \gamma^2}
    \right)
\end{gathered}
$}
\end{equation*}
   
{where the first inequality follows from Jensen's inequality, the second from Assumption \ref{assumption:linear-bound}, the third from the triangle inequality, and the fourth from the fact that $\mathcal{N}(0,Id)$ has finite moments with $\bar{M}$ a constant incorporating $M^2$ and these bounds}.

Using ${\gamma^2 \leq 1}$, for some constant $\tilde{M} $ one has
  \begin{eqnarray*}
    | V_{\varphi} (\Sigma) | & \leq & \tilde{M} (1 + \alpha + \beta + \alpha \beta) =
    \tilde{M} (1 + \alpha) (1 + \beta)
  \end{eqnarray*}
  
\end{proof}


\vspace{10pt}
We end the section showing the explicit characterization of the maps $V_{\varphi}$ for some selected\footnote{by the availability in the literature.} activation functions. We write $V_{\varphi}$ with the obvious meaning.

\begin{proposition}\label{app:charact-Phi}
    Defining $\gamma(\Sigma) := \frac{[\Sigma]_1^2}{\sqrt{[\Sigma]_1^2[\Sigma]_2^2}}$ we have
    \begin{equation}
        \begin{gathered}
            V_{id}(\Sigma) = [\Sigma]_1^2 = [\Sigma]_2^1
            \\
            V_{ReLU}(\Sigma) = \frac{1}{2}\left(1 + \frac{\sqrt{1- \gamma(\Sigma)^2}}{\gamma(\Sigma)}  - arccos(\gamma(\Sigma))\right) [\Sigma]_1^2
            \\
            V_{erf}(\Sigma) = \frac{2}{\pi} arcsin \left( \frac{[\Sigma]_1^2}{\sqrt{(0.5 + [\Sigma]_1^1)(0.5 + [\Sigma]_2^2)}} \right)
        \end{gathered}
    \end{equation}
\end{proposition}

\begin{proof}
    See \cite{yang2019wide}[Facts B.2, B.3].
\end{proof}

% \newpage
\section{Inhomogeneous Case}

In this section of the appendix we are going to prove all the results stated for the inhomogeneous case.

Recall that the \emph{inhomogeneous} models had the following structure: fixed a partition $\D$, the \emph{hidden dimension} $N$ and the activation function $\varphi: \R \to \R$ we have defined the models as 
\[
    \psi^{\D, N}_{in}(x) := \sprod{v^N}{Y^{\D,N}_1(x)}_{\R^N}
\]
where $v^N \sim \mathcal{N}(0,\frac{1}{N})$ and $Y^{\D,N} : \D \times \bX \to \R^N$ is the final value of 
\begin{equation*} \begin{gathered}
    Y^{\D,N}_{t^{\D}_{l}}(x) = Y^{\D,N}_{t^{\D}_{l-1}}(x) + \sum_{k=1}^d \big( A_{k,l} \varphi(Y^{\D,N}_{t^{\D}_{l-1}}(x)) + b_{k,l} \big) \Delta x^k_{t^{\D}_l}
    \\
    Y^{\D,N}_0(x) = Y_0 \in \R^N \text{ and }  \Delta x^k_{t^{\D}_l} = (x^k_{t^{\D}_{l}}-x^k_{t^{\D}_{l-1}}) \in \R
\end{gathered} \end{equation*}
with $\varphi$ applied componentwise and  the components of $A_{k,l} \in \R^{N \times N}$, $b_{k,l} \in \R^N$ sampled according to
\begin{equation*}
\begin{gathered}
    [A_{k,l}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{\sigma_{A}^2}{N(t_l - t_{l-1})})    \hspace{15pt}   
    [Y_0]_{\alpha}\sim \mathcal{N}(0,\sigma_{Y_0}^2) \hspace{15pt}
    [b_{k,l}]_{\alpha} \sim \mathcal{N}(0,\frac{\sigma_b^2}{(t_l - t_{l-1})})
\end{gathered}
\end{equation*}
independently from each other and from $v^N$.


The section will be subdivided in two main parts: in the first we consider the infinite-width-then-depth limit and in the second the Infinite-Depth-then-Width one.

\subsection{The infinite-width-then-depth limit}\label{app:sec:inhom-inf-W-D-limit}

The main goal in this subsection is to prove Theorem \ref{thm:main-inhom-Kernels} which we restate here:
\begin{theorem}
Let the activation function $\varphi: \R \to \R$ be a linearly bounded, absolutely continuous map with exponentially bounded derivative. Let $\{\D_M\}$ be a sequence of partitions of $[0,1]$ with $|\D_M| \to 0$.
For any subset $\X = \{x_1, \dots, x_n\} \subset \bX$ the following convergence in distribution holds
\[
    \lim_{M \to \infty} \lim_{N \to \infty} \psi^{\D_M, N}_{in}(\X)
    =
    \mathcal{N}(0,\kappa^{in}_{\varphi}(\X, \X))
\]
where the map $\kappa^{in}_{\varphi} : \bX \times \bX \to \R$ is given by the unique
final values $\kappa^{x,y}_{\varphi}(1)$ of the following differential equation.

\begin{equation}\label{eqn:app_inhom_kernel_pre}
\begin{gathered}
      \kappa_{\varphi}^{x,y}(t) =  \sigma_{S_0 }^2  + 
      \int_{\tau = 0}^{t} 
      \Big[ 
      \sigma_A^2 \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}^{x, y}_{\tau})} 
      [ \varphi(Z_1) \varphi(Z_2) ] 
      + 
      \sigma_b^2 
      \Big] 
     \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d}   d \tau 
\end{gathered}
\end{equation}
with 
\[ 
    {\Sigma}^{x, y}_{t} = 
     \left(\begin{array}{c}
       \kappa_{\varphi}^{x,x}(t), \kappa_{\varphi}^{x,y}(t)\\
       \kappa_{\varphi}^{x,y}(t), \kappa_{\varphi}^{y, y}(t)
     \end{array}\right) 
\]

\emph{i.e.} the finite dimensional distributions of the stochastic process $\psi^{\D_M,N}_{in}(\cdot)$ indexed on $\bX$ 
    converge weakly to the corresponding ones of the Gaussian Process $\mathcal{GP}(0,\kappa^{in}_{\varphi})$.
\end{theorem}

We split the lengthy proof in two parts:
\begin{enumerate}
    \item The infinite width-convergence of the finite dimensional distributions 
    \[
    \mathcal{L}(\psi^{\D_M, N}_{in}(\X) ) \xrightarrow[]{N \to \infty} \mathcal{N}(0, \kappa_{\D_M}(\X,\X))
    \]
    to those of a Gaussian process $\mathcal{GP}(0,\kappa_{\D_M})$ defined by a Kernel computed as the final value of a finite difference scheme on the "partition" $\D_M$ of $[0,1]$. This will be done using Tensor Programs \cite{yang2019wide} 
    % in \ref{subsubsec:discrete-inhom-Kernel}.
    
    \item The infinite-depth convergence of the \emph{discrete Kernels} $\kappa_{\D_M}$ to a limiting Kernel $\kappa_{\varphi}$ which solves the differential equation (\ref{eqn:app_inhom_kernel_pre}). 
    % This will be done in \ref{subsubsec:conv-inhom-Kernel}.
\end{enumerate}


\subsubsection{Infinite-width limit with fixed depth}\label{subsubsec:discrete-inhom-Kernel}

Fix a partition $\D = \{0 = t_0, \dots, t_m, \dots, t_{\norm{\D}}=1\}$ of $[0,1]$.
Using the formalism of \emph{Tensor Programs}, we next identify the infinite-Width distributional limits of our \emph{inhomogeneous} networks.


\begin{theorem}\label{thm:inhom-discrete-phi-SigKer}
Let the activation function $\varphi: \R \to \R$ be linearly bounded
\footnote{in the sense that $\exists C > 0.$ such that $|\phi(x)| \leq C(1+|x|)$.}.
For any subset $\X = \{x_1, \dots, x_n\} \subset \bX$ the following convergence in distribution holds
\[
    \lim_{N \to \infty} \psi^{\D, N}_{in}(\X) 
    =
    \mathcal{N}(0,\kappa_{\D}(\X, \X))
\]
where the map $\kappa_{\D} : \bX \times \bX \to \R$ is defined as the solution $\kappa_{\D}(1)$ of the following finite difference scheme on $\D$
\begin{equation}\label{eqn:inhom-discrete-kernel}
%\resizebox{0.8\hsize}{!}{$
\begin{gathered}
     \kappa_{\D}^{x,y}(t_{m}) = \kappa_{\D}^{x,y}(t_{m-1}) 
    + \Big( \sigma_A^2 
    \E_{Z \sim \mathcal{N}(0, \Sigma_{\D}^{x,y}(t_{m-1}))}[ \varphi(Z_1) \varphi(Z_2) ]
    + \sigma_b^2 \Big) \frac{\sprod{\Delta x_{t_m}}{\Delta y_{t_{m}} }_{\R^d}}{t_{m} - t_{m-1}}
\end{gathered}
\end{equation}
with $\kappa_{\D}^{x,y}(0) = \sigma_{Y_0}^2$ and where 
\[
   \Sigma_{\D}^{x,y}(t) =  
    \begin{pmatrix}
        \kappa_{\D}^{x,x}(t) & \kappa_{\D}^{x,y}(t) \\
        \kappa_{\D}^{x,y}(t) & \kappa_{\D}^{y,y}(t)
    \end{pmatrix}
\]
\end{theorem}

\begin{proof}
    We use \cite{yang2019wide}[Corollary 5.5] applied to the Tensor Program of Algorithm \ref{algo:inhom} where the input variables are independently sampled according to
    \[
    [A_{k, l}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{\sigma_{A}^2}{N(t_{l} - t_{l-1})}), 
    \quad 
    [v]_{\alpha}\sim \mathcal{N}(0,{1}),
    \quad
    [Y_0]_{\alpha}\sim \mathcal{N}(0,\sigma_{Y_0}^2),
    \quad 
    [b_{k, l}]_{\alpha} \sim \mathcal{N}(0,\frac{\sigma_b^2}{t_{l} - t_{l-1}})
\]
Note how the sampling scheme follows \cite{yang2019wide}[Assumption 5.1] and how linearly bounded functions are \emph{controlled} in the sense of \cite{yang2019wide}[Definition 5.3] since for all $x \in \R$ one has $|\phi(x)| \leq C(1+|x|) \leq e^{|x| + log(C)}$.
Thus we are under the needed assumptions to apply \cite{yang2019wide}[Corollary 5.5].

There are two things to notice, done in order to satisfy the required formalism: 
\begin{itemize}
    \item In the program the output projector $v$ is sampled according to $\mathcal{N}(0,1)$ while the original $v^N \sim \mathcal{N}(0,\frac{1}{N})$. This does not pose any problems since the output of the formal programs uses ${v}/{\sqrt{N}}\sim \mathcal{N}(0,\frac{1}{N})$.
    \item The input paths $x_i$ enter program \ref{algo:inhom} not as \emph{Inputs} but as coefficients of \emph{LinComb}, this means that for any choice of input paths we must formally consider different algorithms. In any case, for any possible choice, the result has always the same functional form; hence \emph{a posteriori} it is legitimate to think about \emph{one} algorithm.
\end{itemize}

Note that $Y^{x}_{m}$ stands for the formal variable in program \ref{algo:inhom}, not for $Y^{\D, N}_{t_m}(x)$ even thogh this is the value which it "stores" for a fixed hidden dimension $N$.

The result in \cite{yang2019wide}[Corollary 5.5] tells us that the output vector converges in law, as $N \to \infty$, to a Gaussian distribution $\mathcal{N}(0, \Tilde{K})$ where
\[
    [\Tilde{K}]_i^j = \E_{Z \sim \mathcal{N}(\mu, \Sigma)}
    \bigg[
    Z^{Y^{x_i}_{\norm{\mathcal{D}}}} Z^{Y^{x_j}_{\norm{\mathcal{D}}}}
    \bigg]
    =
    \Sigma(Y^{x_i}_{\norm{\mathcal{D}}}, Y^{x_j}_{\norm{\mathcal{D}}})
\]

with $\mu, \Sigma$ computed according to \cite{yang2019wide}[Definition 5.2] and defined on the set of all G-vars in the program \emph{i.e.}

\begin{equation*}
    \mu(g) = \begin{cases}
      \mu^{in}(g) & \text{if $g$ is \textbf{Input} G-var}\\
      \sum_k a_k \mu(g_k) & \text{if $g$ is introduced as $\sum_k a_k g_k$ via \textbf{LinComb}}\\
      0 & \text{otherwise}
    \end{cases}
\end{equation*}
\begin{equation*}
    \Sigma(g, g') =  \begin{cases}
      \Sigma^{in}(g, g') & \text{if both $g$ and $g'$ are \textbf{Input} G-var}\\
      \sum_k a_k \Sigma(g_k, g') & \text{if $g$ is introduced as $\sum_k a_k g_k$ via \textbf{LinComb}}\\
      \sum_k a_k \Sigma(g, g_k') & \text{if $g'$ is introduced as $\sum_k a_k g'_k$ via \textbf{LinComb}}\\
      \sigma_W^2 \E_{Z \sim \mathcal{N}(\mu, \Sigma)}[\phi(Z)\phi'(Z)]& \text{if $g = Wh$, $g' = Wh'$ via \textbf{MatMul} w/ same $W$}\\
      0 & \text{otherwise}
    \end{cases}
\end{equation*}

where $h = \phi((g_k)_{k=1}^{m})$ for some function $\phi$ and $\phi(Z) := \phi((Z^{g_k})_{k=1}^{m})$, similarly for $g'$.

In our setting $\mu^{in} \equiv 0$ since all \textbf{Input} variables are independent, from which $\mu \equiv 0$; furthermore $\Sigma^{in}(g, g') = 0$ except if $g = g'$ when it takes values in $\{ \sigma^2_{Y_0}, \frac{\sigma^2_{b}}{t_l - t_{l-1}}, 1\}$ accordingly.

Following the rules of $\Sigma$, assuming $l_i, l_j \in \{1, \dots, \norm{\mathcal{D}} \}$, we obtain
\begin{eqnarray*}
  \Sigma(Y^{x_i}_{l_i}, Y^{x_j}_{l_j}) & = & \Sigma (Y^{x_i}_{l_i - 1}, Y^{x_j}_{l_j}) +
  \Sigma \left( \sum_{k = 1}^d \gamma_{k, l_i}^i \Delta (x_i)_{t_{l_i}}^k,
  Y^{x_j}_{l_j} \right)\\
  & = & \Sigma (Y^{x_i}_{l_i - 1}, Y^{x_j}_{l_j}) + \Sigma \left( \sum_{k = 1}^d
  \gamma_{k, l_i}^i \Delta (x_i)_{t_{l_i}}^k, Y^{x_j}_{l_j-1} \right)\\
  &  & + \Sigma \left( \sum_{k = 1}^d \gamma_{k, l_i}^i \Delta
  (x_i)_{t_{l_i}}^k, \sum_{l = 1}^d \gamma_{m, l_j}^j \Delta
  (x_j)_{t_{l_j}}^l \right)\\
  & = & \Sigma(Y^{x_i}_{l_i - 1}, Y^{x_j}_{l_j}) + \Sigma (Y^{x_i}_{l_i}, Y^{x_j}_{l_j-1})
  - \Sigma (Y^{x_i}_{l_i - 1}, Y^{x_j}_{l_j-1})\\
  &  & + \sum_{k, m = 1}^d \Sigma (\gamma_{k, l_i}^i, \gamma_{m, l_j}^j)
  \Delta (x_i)_{t_{l_i}}^k \Delta (x_j)_{t_{l_j}}^m
\end{eqnarray*}

Now
\[ 
    \Sigma (\gamma_{k, l_i}^i, \gamma_{m, l_j}^j) 
    = \delta_{k, m} \delta_{i, j} \frac{\sigma^2_{A}}{t_{l_i} - t_{l_i-1}}
    \E[\varphi(Z_1)\varphi(Z_2)]
    +
    \Sigma(b_{k, l_i}, b_{m, l_j})
    = \frac{\delta_{k, m} \delta_{i, j}}{t_{l_i} - t_{l_i-1}}\big[ 
    \sigma_{A}^2 
    \E[\varphi(Z_1)\varphi(Z_2)]
    + \sigma_b^2
    \big]
\]
   
where $[Z_{1,} Z_2]^{\top} \sim \mathcal{N} (0, \tilde{\Sigma}_{l_{i-1}}(x_i, x_j))$  with

\begin{eqnarray*}
  \tilde{\Sigma}_{l}(x_i, x_j) & = 
  & \left(\begin{array}{c c}
    \Sigma^M (Y^{x_i}_{l}, Y^{x_i }_{l}) & 
    \Sigma^M (Y^{x_i}_{l}, Y^{x_j }_{l})\\
    \Sigma^M (Y^{x_i}_{l}, Y^{x_j }_{l}) & 
    \Sigma^M (Y^{x_j }_{l}, Y^{x_j }_{l})
  \end{array}\right)
\end{eqnarray*}


In particular we see that if $l_i \neq l_j$ then $ \Sigma(Y^{x_i}_{l_i}, Y^{x_j}_{l_j}) = \Sigma (Y^{x_i}_{l_{i \wedge j}}, Y^{x_j}_{l_{i \wedge j }})$.
Thus if we set, for $t_{l_i} \in \D$,  $\kappa_{\D}^{x_i, x_j}(t_{l_i}) := \Sigma(Y^{x_i}_{l_i}, Y^{x_j}_{l_i})$ we get
\begin{equation*}
  \kappa_{\D}^{x_i, x_j}(t_{l_i})  =  \kappa_{\D}^{x_i, x_j}(t_{l_i - 1})
  + \sum_{k = 1}^d \big( \sigma_A^2 \mathbb{E}_{(Z_x, Z_y)
  \sim \mathcal{N} (0, \tilde{\Sigma}_{l_{i-1}}(x_i, x_j))} [\varphi (Z_x) \varphi
  (Z_y)]  + \sigma_b^2 \big) \frac{\Delta (x_i)_{t_{l_i}}^k \Delta (x_j)_{t_{l_i}}^k}{t_{l_i} - t_{l_i-1}}
\end{equation*}
which is exactly what Equation \ref{eqn:inhom-discrete-kernel} states. 
Then note how 
\[
\Sigma (Y^{x_i}_{0}, Y^{x_j}_{0}) = \sigma_{Y_0}^2
\]

Thus finally we can conclude and write the entries of the matrix $\Tilde{K}$ as
\[
    [\Tilde{K}]_i^j = \kappa_{\D}^{x_i, x_j}(1)
\]

\end{proof}

\begin{algorithm}[tbh]
    \caption{$Y^{\D, N}_1$ as Nestor program}
    \label{algo:inhom}
    \begin{algorithmic}
       \STATE {\bfseries Input:} $Y^0: \Gtype(N)$ \hfill  $\triangleright$ \textit{initial value}
       \STATE {\bfseries Input:} $(b_{1,l}, \dots, b_{d,l}): \Gtype(N)$ \hfill $\triangleright$ \textit{biases}
       \STATE {\bfseries Input:} $(A_{1,l}, \dots, A_{d,l})_{l=1,\cdots,\norm{\D}}: \Atype(N, N)$ \hfill $\triangleright$ \textit{matrices}
       \STATE {\bfseries Input:} $v: \Gtype(N)$ \hfill $\triangleright$ \textit{readout layer weights}
      \\
      \FOR{$i = 1, \dots, n$}
          \STATE {\it // Compute $Y^{\D, N}_1 (x_i)$  (here $ Y_0^{x_i}$ is to be read as $Y_0$)}
          \\
          \FOR{$l = 1,\dots,\norm{\mathcal{D}}$}
              \FOR{$k = 1,\dots,d$}
                \STATE $\alpha^i_{k,l} := \varphi(Y^{x_i}_{l-1}): \Htype(N)$ \hfill  $\triangleright$ \textit{by Nonlin;}
                \STATE $\beta^i_{k,l} := A_{k, l} \alpha^i_{k,l} : \Gtype(N)$ \hfill  $\triangleright$ \textit{by Matmul;}
                \STATE $\gamma^i_{k,l} := \beta^i_{k,l} + b_{k, l}  : \Gtype(N)$ \hfill  $\triangleright$ \textit{by LinComb;}
              \ENDFOR
              \STATE $Y^{x_i}_{l} := Y^{x_i}_{l-1} + \sum_{k=1}^d \gamma^i_{k,l} [(x_i)^k_{t_l} - (x_i)^k_{t_{l-1}}]  : \Gtype(N)$ \hfill  $\triangleright$ \textit{by LinComb;}
          \ENDFOR
          \\
      \ENDFOR
      \\
      \ENSURE $(v^T Y_{\norm{\mathcal{D}}}^{x_i} / \sqrt{N})_{i=1,\dots,n}$
    \end{algorithmic}
\end{algorithm}


Actually we have proved the even stronger statement that 
\begin{corollary}
    For all $t,s \in \D$ one has the following distributional limit
    \[
     \mathcal{L}(\sprod{v^N}{Y^{\D, N}_{t}(\X)}\sprod{v^N}{Y^{\D, N}_{s}(\X)})
    \xrightarrow[N \to \infty]{} 
    \mathcal{N}(0,K^{\D}_{t\wedge s}(\X,\X))
    \]
\end{corollary}


% \subsubsection{Infinite-width-then-depth limit}\label{subsubsec:conv-inhom-Kernel}

\subsubsection{Preliminary Bounds}\label{app:subsec:inhom_bounds}

We now prove the convergence of the Kernels $\kappa_{\D_M}^{x,y}({\cdot}) : \D_M \to \R$ to a unique limit kernel $\kappa^{x,y}(\cdot) : [0,1] \to \R$ as $|\D_M| \to 0$. 

% \subsubsection{Fixing the Notation}

\begin{definition}\label{def:ker_ext}
  Fix $\D \assign \{ 0 = t_0 < \cdots < t_{\| \D \|} = 1 \}$ partition of $[0, 1]$, let $x,y \in \bX$.
  We define
  \[ \kappa_{\D}^{x,y} : \D \rightarrow \mathbb{R} \]
  as the map satisfying
  \begin{equation*}
  \begin{gathered}
  \kappa_{\D}^{x,y}(t_{m}) = \kappa_{\D}^{x,y}(t_{m-1}) + \Big( \sigma_A^2 
    \E_{Z \sim \mathcal{N}(0, \Sigma^{\D}_{x,y}(t_{m-1}))}[ \varphi(Z_1) \varphi(Z_2) ]
    + \sigma_b^2 \Big) \frac{\sprod{\Delta x_{t^{\D}_m}}{\Delta y_{t^{\D}_{m}} }_{\R^d}}{t^{\D}_{m} - t^{\D}_{m-1}}
    \\
    = \kappa_{\D}^{x,y}(t_{m-1}) + \Big( \sigma_A^2 
    \E_{Z \sim \mathcal{N}(0, \Sigma^{\D}_{x,y}(t_{m-1}))}[ \varphi(Z_1) \varphi(Z_2) ]
    + \sigma_b^2 \Big) \sprod{\frac{\Delta x_{t^{\D}_m}}{\Delta t^{\D}_{m}}}{\frac{\Delta y_{t^{\D}_{m}}}{\Delta t^{\D}_{m}} }_{\R^d} \Delta t^{\D}_{m}
  \end{gathered}
  \end{equation*}
  with $\kappa_{\D}^{x,y}(0) = \sigma_{Y_0}^2$ and 
  \[
    \Sigma_{\D}^{x,y}(t) =  
    \begin{pmatrix}
        \kappa_{\D}^{x,x}(t) & \kappa_{\D}^{x,y}(t) \\
        \kappa_{\D}^{x,y}(t) & \kappa_{\D}^{y,y}(t)
    \end{pmatrix}
  \]
\end{definition}


\begin{definition}
  We extend the map $\kappa_{\D}^{x,y} : \D \rightarrow \mathbb{R}$ to the whole interval $[0,1]$ in two ways: for any $t \in [t_m, t_{m+1})$ 
  
  1) (piecewise linear interpolation) define  the map 
  $\kappa_{\D}^{x,y} : [0, 1] \rightarrow \mathbb{R}$
  as
  \begin{equation*}
    \kappa_{\D}^{x,y} (t) =
    \kappa_{\D}^{x, y} (t_{m }) + 
    \left( \sigma_A^2 V_{\varphi} \left( \Sigma^{\tmscript{x, y}}_{\D } (t_{m }) \right) + \sigma_b^2 \right)
    \sprod{\frac{x_t - x_{t_{m}}}{t - t_{m}}}{\frac{y_t - y_{t_{m}}}{t - t_{m}} }_{\R^d} (t - t_{m})
  \end{equation*}
  2) (piecewise constant interpolation) define the map  $\Tilde{\kappa}_{\D}^{x, y} : [0, 1] \rightarrow \mathbb{R}$ as
  \[
    \Tilde{\kappa}_{\D}^{x , y}(t) = \kappa_{\D}^{x,y}(t_{m}).
  \]
   % where $t \in [t_m, t_{m+1})$.
   similarly we define the extension ${\Sigma}_{\D}^{x,y}$ and $\Tilde{\Sigma}_{\D}^{x,y}$.
\end{definition}

It is important to consider both these types of extensions. The \emph{piecewise linear}, being continuous, is used to prove convergence to a limiting map in the space of continuous functions $C^0([0,1];\R)$. The \emph{piecewise constant} is proved to converge to the same object, this time in $L^{\infty}([0,1];\R)$ since it's not continuous, and is well suited to prove how properties of the discrete kernels pass to the limit. \cris{Discuss together}

\begin{theorem} \label{inhom_simple_conv}
  Fix a sequence $\{\D_M \}_{M \in \N}$ of partitions of $[0,1]$ with $| \D_M | \rightarrow 0$.
  Then we have the following convergence in $(C^0([0,1]; \R), \norm{\cdot}_{\infty})$
  \[ \kappa_{\D_M}^{x,y} (t) \rightarrow  \kappa^{x, y}(t) \]
  where $K_{x, y} (t)$ is the unique solution to
  \begin{equation}\label{eqn:inhom-simple-conv-PDE}
   \begin{gathered}
    \kappa^{x, y} (t) =  \sigma^2_{S_0} +  \int_{0}^t
    \left( \sigma_A^2 \mathbb{E}_{(Z_x, Z_y) \sim
    \mathcal{N} (0,  \Sigma^{x, y} (s))} [\varphi (Z_x) \varphi (Z_y)] +
    \sigma_b^2 \right) \sprod{\Dot{x}_{s}}{ \Dot{y}_{s}}_{\R^d}   d s\\
     =  \sigma^2_{S_0} +  \int_{0}^t (\sigma_A^2 V_{\varphi} (\Sigma^{x, y}(s)) + \sigma_b^2) \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d}   d s
   \end{gathered}  
  \end{equation}
  with
  \[ \Sigma^{x, y}(t) = \left(\begin{array}{c}
       \kappa^{x, x} (t), \kappa^{x, y} (t)\\
       \kappa^{x, y} (t), \kappa^{y, y} (t)
     \end{array}\right) \]
\end{theorem}

\iffalse
\begin{proof}
    We can cast the PDE in the form \cite{FrizVictoir}[Definition 3.3] by considering the system $(K_{x,x}, \kappa^{x,y}, K_{y,y})$. 
    Choose as driving signal the 3-dimensional path $\int_0^t (\sprod{\Dot{x}_s}{\Dot{x}_s}, \sprod{\Dot{x}_s}{\Dot{y}_s}, \sprod{\Dot{y}_s}{\Dot{y}_s} )^T ds$ and as driving fields the functions
    \begin{equation}
        \begin{gathered}
            V_1(K_{x,x}, \kappa^{x,y}, K_{y,y}) := (\sigma_A^2 V_{\varphi} (\Sigma_{x, x}(s)) + \sigma_b^2) e_1\\
            V_2(K_{x,x}, \kappa^{x,y}, K_{y,y}) :=(\sigma_A^2 V_{\varphi} (\Sigma_{x, y}(s)) + \sigma_b^2) e_2\\
            V_3(K_{x,x}, \kappa^{x,y}, K_{y,y}) := (\sigma_A^2 V_{\varphi} (\Sigma_{y, y}(s)) + \sigma_b^2) e_3\\
        \end{gathered}
    \end{equation}
    with $\{e_1,e_2,e_3\}$ basis of $\R^3$.

    Then 
\end{proof}
\fi

\nico{With some gymnastics one could prove first the case $x=y$ using \cite{FrizVictoir}[Theorem 3.7] , then pass to the general case. The problem comes with the general case when one practically has to repeat the argument in the proof \cite{FrizVictoir}[Theorem 3.6] with some extra details due to the time-dependece of the fields... I think that doing all at the same time is not much different at this point and would use only one argument. }

The proof of Theorem \cref{inhom_simple_conv} is divided, for convenience, in the following two sections. We will first provide some technical bounds in \ref{app:subsec:inhom_bounds}.
The main proof is laid out in \ref{app:subsec:inhom_main_proof}.

The central idea will be proving that the sequence $\{ \kappa_{\D_M}^{x,y} \}_M$ is uniformly bounded and uniformly equicontinuous so to apply Ascoli-Arzelà theorem. 
We will then prove that the thus found limit is the unique solution of \cref{eqn:inhom-simple-conv-PDE} and that the whole sequence converges to it.

%% Multiline Comment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
    \begin{proof}
    
        \textit{- Roadmap}
    
        \textit{- Case $x=y$}
    
        Let $\mathbf{1} \in \R^{2 \times 2}$ be the matrix with all entries equal to $1$. Then for $a \in \R$ we have $a\mathbf{1} \in PSD$ if and only if $a \geq 0$.
        Write $\Psi(a) = V_{\varphi}((a\vee 0)\mathbf{1})$.
        Note how $\Sigma_{x, x}(t) = K_{x, x} (t) \mathbf{1}$ thus when well defined, \emph{i.e.} when $K_{x, x} (t) \geq 0$, we have $V_{\varphi}(\Sigma_{x, x}(t)) = \Psi(K_{x, x}(t))$. 
    
        Let $z_t := \int_0^t  \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d} ds$ this is a 
        
    
        It is clear that 
        
    \end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Note that the covariance matrices $\tilde{\Sigma}_{\D }^{x \comma y}$ are given as the limitng objects in Theorem \ref{thm:inhom-discrete-phi-SigKer}, this means \emph{a fortiori} that they must always be positive semidefinite, \emph{i.e.} in $PSD_2$. 

% We are going to need a more quantitative result, in the form of a uniform membership in some $PSD(R)$, in order to later leverage Lemma \ref{lemma:split_on_PSD_R}. \cris{Rephrase more precisely}

% We first prove such a result for the case $x = y$, the general case will follow easily.

The next lemma establishes a uniform (in $x \in \bX$) lower bound for the kernels $\tilde{\Sigma}_{\D }^{x \comma x}$.

\begin{lemma}
For any $ x \in \bX$, any partition $\D$ and any $t \in \D$, the kernels $\Tilde{\kappa}_{\D}^{x, x}(t), {\kappa}_{\D}^{x, x} (t) \geq \sigma_{Y_0}^2$
\end{lemma}

\begin{proof}
For any $t_m\in\mathcal{D}$ we have by \cref{def:ker_ext}
  \[ 
     \kappa_{\D}^{x,x} (t_m) = \sigma^2_{Y_0} +
     \sum_{\tmscript{\begin{array}{c}
       0 \leq l < m
     \end{array}}}\left( \sigma_A^2 V_{\varphi} \left(
     \Sigma^{\tmscript{x, x}}_{\D} (t_{l})
     \right) + \sigma_b^2 \right)
     |{\frac{\Delta x_{t_{l + 1}}}{\Delta t_{l + 1}}}|^2  \Delta t_{l + 1} 
  \]

Recall the definition of the map $V_{\varphi}$ in \cref{lemma:split_on_PSD_R}. For any $t_l\in\D$ we note that $V_{\varphi} ( \Sigma^{\tmscript{x, x}}_{\D} (t_{l})) = \E[\varphi(\sqrt{\kappa_{\D}^{x,x}(t_l)})^2]$ for $Z \sim \mathcal{N}(0,1)$ since $\Sigma^{\tmscript{x, x}}_{\D} (t_{l}) = \kappa_{\D}^{x,x}(t_l) \mathbf{1}$ with $\mathbf{1} \in R^{2\times 2}$ the matrix with all entries equal to $1$.
Thus $V_{\varphi} ( \Sigma^{\tmscript{x, x}}_{\D} (t_{l})) \geq 0$ and we can conclude that $\Tilde{\kappa}_{\D}^{x, x}(t) \geq \sigma_{Y_0}^2 $ since we are summing to $\sigma_{Y_0}^2$ only the non-negative terms
\[
\left( \sigma_A^2 V_{\varphi} \left(
     \Sigma^{\tmscript{x, x}}_{\D} (t_{l})
     \right) + \sigma_b^2 \right)
     |{\frac{\Delta x_{t_{l + 1}}}{\Delta t_{l + 1}}}|^2  \Delta t_{l + 1} 
\]

For any $t \in [0,1]$, by definition, we can write
  \begin{equation}
      \kappa_{\D}^{x \comma x} (t) =
    \kappa_{\D}^{x,x} (t_{m}) + 
    \left( \sigma_A^2 V_{\varphi} \left( \Tilde{\Sigma}^{\tmscript{x, y}}_{\D } (t_{m}) \right) + \sigma_b^2 \right) |\frac{x_t - x_{t_{m}}}{t-t_{m}}|^2_{\R^d} (t-t_{m})
  \end{equation}
  thus $\textbf{}$ is the sum of $ \kappa_{\D}^{x,x} (t_{m }) = \Tilde{\kappa}_{\D }^{x \comma x} (t) \geq \sigma_{Y_0}^2$ and the quantity
  \[
  \left( \sigma_A^2 V_{\varphi} \left( \Tilde{\Sigma}^{\tmscript{x, y}}_{\D } (t_{m}) \right) + \sigma_b^2 \right) |\frac{x_t - x_{t_{m}}}{t-t_{m}}|^2_{\R^d} (t-t_{m})
  \]
  which is $\geq 0$ by the same arguments as above.
\end{proof}

The second step is another bound, this time from above, which will be uniform on bounded subsets of $\bX$.

\begin{lemma}
  There is a constant $C_x > 0$ independent of $\D$ such that
  \[ \| \kappa_{\D}^{x, x} \|_{\infty,
     [0, 1]} \assign \sup\limits_{t \in [0, 1]} |
     \kappa_{\D}^{x, x} (t) | \leq C_x
  \]
\end{lemma}

Note how all the values taken by $\Tilde{\kappa}_{\D}^{x, x}$ are also taken by $\kappa_{\D}^{x, x}$ in the corresponding partition points, thus this statement holds \emph{a fortiori} for $\Tilde{\kappa}_{\D}^{x, x}$ too.

\begin{proof}
    Let us prove this result for $\Tilde{\kappa}_{x,x}$ first. Let $t \in \left[ t_m , t_{m + 1}  \right)$. Recall the definition of $\Tilde{\kappa}_{x,x}$
  \begin{equation*}
    \Tilde{\kappa}_{\D}^{x, x} (t) =
     \kappa_{\D}^{x,x} (t_m) = \sigma^2_{Y_0} +
     \sum_{\tmscript{\begin{array}{c}
       0 \leq l < m
     \end{array}}}\left( \sigma_A^2 V_{\varphi} \left(
     \Sigma^{\tmscript{x, x}}_{\D} (t_{l})
     \right) + \sigma_b^2 \right) \sprod{\frac{\Delta x_{{t_{l + 1}} }}{\Delta t_{l + 1}}}{
     \frac{\Delta x_{t_{l + 1}}}{\Delta t_{l + 1}}}\Delta t_{l + 1}
  \end{equation*}
We then have 
    \begin{equation*}
        \begin{gathered}
            \sprod{\frac{\Delta x_{{t_{l + 1}} }}{\Delta t_{l + 1}}}{\frac{\Delta x_{t_{l + 1}}}{\Delta t_{l + 1}}}\Delta t_{l + 1} =
            |\frac{\Delta x_{{t_{l + 1}} }}{\Delta t_{l + 1}}|_{\R^d}^2 \Delta t_{l + 1} = 
            \big|\frac{1}{\Delta t_{l + 1}}  \int_{t_l}^{t_{l+1}} \Dot{x}_t dt \big|_{\R^d}^2 \Delta t_{l + 1}\\
            \leq (\frac{1}{\Delta t_{l + 1}}  \int_{t_l}^{t_{l+1}} |\Dot{x}_t|_{\R^d} dt)^2 \Delta t_{l + 1}
            \leq \frac{1}{\Delta t_{l + 1}}  \int_{t_l}^{t_{l+1}} |\Dot{x}_t|_{\R^d}^2 dt \Delta t_{l + 1}
            = \int_{t_l}^{t_{l+1}} |\Dot{x}_t|_{\R^d}^2 dt
        \end{gathered}
    \end{equation*}
where the last inequality is by Jensen's inequality. In addition, by \cref{lemma:split_on_PSD_R} there exists a positive constant $\Tilde{M}$ such that
     \begin{equation*}
        \begin{gathered}
            |V_{\varphi}(\Sigma^{\tmscript{x, x}}_{\D} (t_{l}))| \leq \Tilde{M}(1+\sqrt{\kappa(t_l)})^2 \leq 2\Tilde{M}(1+ \kappa(t_l)).
        \end{gathered}
    \end{equation*}
  Thus
  \begin{equation*}
      \begin{gathered}
          \Tilde{\kappa}(t) \leq \sigma_{Y_0}^2 + \sum_{0 \leq l < m}
          (2\sigma_A^2 \Tilde{M}(1+ \kappa (t_l)) + \sigma_b^2 ) 
          \int_{t_l}^{t_{l+1}} |\Dot{x}_t|_{\R^d}^2 dt \\
          = \sigma_{Y_0}^2 + \int_{0}^{t_{m}}
          (2\sigma_A^2 \Tilde{M}(1+ \Tilde{\kappa}(t)) + \sigma_b^2 ) 
           |\Dot{x}_t|_{\R^d}^2 dt
      \end{gathered}
  \end{equation*}
By Gronwall inequality (\cite{FrizVictoir}, Lemma 3.2) we have
  \begin{eqnarray*}
    1 + \Tilde{\kappa}(t) & \leq & (1 + \sigma^2_{Y_0} + \sigma_b^2 \norm{x}_{\bX}^2) \exp \{ 2 \sigma_A^2 \tilde{M} \norm{x}_{\bX}^2 \}
  \end{eqnarray*}
  hence the statement of this lemma holds for $\Tilde{\kappa}_{x,x}$ with the constant
  \begin{eqnarray*}
    \Tilde{C}_x & = & (1 + \sigma^2_{Y_0} + \sigma_b^2 \norm{x}_{\bX}^2) {e^{2 \sigma_A^2 \tilde{M} \norm{x}_{\bX}^2}}  - 1
  \end{eqnarray*}

  Consider now 
  \[
    K^{\D }_{x, x} (t) =
    \kappa_{\D}^{x,x} (t_{m }) + 
    \left( \sigma_A^2 V_{\varphi} \left( \Sigma_{\tmscript{x, y}}^{\D } (t_{m }) \right) + \sigma_b^2 \right)
    |\frac{x_t - x_{t_{m}}}{t - t_{m}}|^2 (t - t_{m})
  \]
  Then we have
\begin{align*}
    |\kappa_{\D }^{x, x} (t)| &\leq 
          |\kappa_{\D}^{x,x} (t_{m})| +  (2\sigma_A^2 \Tilde{M}(1 + \Tilde{C}_x) + \sigma_b^2 ) 
          |\frac{x_t - x_{t_{m}}}{t - t_{m}}|^2 (t - t_{m})\\
          &\leq \Tilde{C}_x + (2\sigma_A^2 \Tilde{M}(1+ \Tilde{C}_x) + \sigma_b^2 ) \norm{x}_{\bX}^2
\end{align*}
Hence the  statement follows by  setting 
  \[
    C_x = \Tilde{C}_x + (2\sigma_A^2 \Tilde{M}(1+ \Tilde{C}_x) + \sigma_b^2 ) \norm{x}_{\bX}^2
  \]
\end{proof}

\begin{remark}
    Note how $C_x$ only depends on $\norm{x}_{\bX}$ and is increasing in it, thus this bound is uniform on bounded subsets of $\bX$.
\end{remark}

The following lemma shows that the kernels qre in fact elements of $PSD(R)$.

\begin{lemma}
  There is an $R = R_x \in \mathbb{R}$ such that $\tilde{\Sigma}_{\D}^{x, x}(t), {\Sigma}_{\D}^{x, x}(t) \in \tmop{PSD_2} (R)$ for every $\D$ and $t \in [0,1]$.
  Moreover, as before, this $R_x$ only depends on $\norm{x}_{\bX}$ and is increasing in it. 
\end{lemma}

\begin{proof}
  $\Tilde{\Sigma}_{\D }^{x, x}$ and ${\Sigma}_{\D }^{x \comma x}$ are $PSD_2$ since they are of form $a\mathbf{1}$ for some $a > 0$.
The diagonal elements $\Tilde{\kappa}_{\D}^{x, x}(t), \kappa_{\D}^{x,x}(t)$ are
  bounded above by a common constant $C_x$ and below by $\sigma^2_{S_0}$. 
  We thus can simply choose $R_x = C_x \vee \sigma^{-2}_{S_0}$.
\end{proof}

We will now extend the result to the case $x\neq y$.

\begin{proposition}\label{prop:inhom_bounded_set_bounds}
    Fix a $\alpha > 0$. There exist a constant $C_{\alpha}$ such that for all $x,y \in \bX$ with $\norm{x}_{\bX}, \norm{y}_{\bX} \leq \alpha$ and partition $\D$ it holds
    \[
        \sup_{0 \leq t \leq 1} \nobracket | \nobracket {\kappa}_{\D}^{x \comma y} (t) | \leq C_{\alpha} 
    \]
    Moreover for $R_{\alpha} := C_{\alpha} \vee \sigma^{-2}_{S_0}$ we get 
    \[
          \Tilde{\Sigma}_{\D }^{x \comma y} (t) \in \tmop{PSD_2}(R_{\alpha}) 
    \]
\end{proposition}


\begin{proof}
Remember how the maps $\Tilde{\Sigma}_{\D }^{x, y}(t)$ are $PSD_2$ by Tensor limiting arguments, in particular by positive semidefinitiveness  and the previous bounds
\begin{eqnarray*}
\nobracket | \nobracket \Tilde{\kappa}_{\D}^{x, y} (t) | \leq \sqrt{\Tilde{\kappa}_{\D}^{x, x} (t) \Tilde{\kappa}_{\D}^{y, y} (t)} \leq \sqrt{\Tilde{C_x }\Tilde{C_y}} \leq \Tilde{C_x} \vee \Tilde{C_y} 
\end{eqnarray*}
For $\kappa^{x,y}(t)$ we proceed similarly to before: when $t \in [t_m, t_{m+1})$ one has
\begin{equation*}
      \begin{gathered}
          |\kappa_{\D}^{x,y}(t)| \leq 
          |\kappa_{\D}^{x,y} (t_{m})| +  |(\sigma_A^2 \Tilde{M}(1+ \sqrt{\Tilde{\kappa}_{\D}^{x, x}(t)})(1+ \sqrt{\Tilde{\kappa}_{\D}^{y, y}(t)}) + \sigma_b^2 ) 
           \sprod{\frac{x_t - x_{t_{m}}}{t - t_{m}}}{\frac{y_t - y_{t_{m}}}{t - t_{m}} }_{\R^d} (t - t_{m})|\\
           \leq
           \Tilde{C_x} \vee \Tilde{C_y} + (2 \sigma_A^2 \Tilde{M}(1+ \Tilde{C_x} \vee \Tilde{C_y}) + \sigma_b^2 )
           |\sprod{\frac{x_t - x_{t_{m}}}{t - t_{m}}}{\frac{y_t - y_{t_{m}}}{t - t_{m}} }_{\R^d}| (t - t_{m})\\
           \leq \Tilde{C_x} \vee \Tilde{C_y} + (2 \sigma_A^2 \Tilde{M}(1+ \Tilde{C_x} \vee \Tilde{C_y}) + \sigma_b^2 )
           (|\frac{x_t - x_{t_{m}}}{t - t_{m}}|^2 + |\frac{y_t - y_{t_{m}}}{t - t_{m}}|^2)(t - t_{m})\\
           \leq \Tilde{C_x} \vee \Tilde{C_y} + ( 2 \sigma_A^2 \Tilde{M}(1+ \Tilde{C_x} \vee \Tilde{C_y}) + \sigma_b^2 )(\norm{x}_{\bX} + \norm{y}_{\bX}) \leq C_{\alpha}
      \end{gathered}
  \end{equation*}
where we have used $|\sprod{a}{b}| \leq  |a||b| \leq (|a|^2 + |b|^2)$ for $a,b \in \R^d$.

The second part follows from the definition of $\tmop{PSD_2}(R_{\alpha})$.
\end{proof}

\nico{Notation... }

\subsubsection{Proof of Theorem \ref{inhom_simple_conv}}\label{app:subsec:inhom_main_proof}

The central idea will be proving that, given any sequence $\D_n$ with $|\D_n| \downarrow 0$, the sequence $\{ \kappa_{\D_n}^{x, y} \}_{n}$ is uniformly bounded and uniformly equicontinuous so that by the Ascoli-Arzelà theorem, the sequence admits a uniformly convergent subsequence. Then, we will prove that the limit of this subsequence is a solution of \cref{eqn:inhom-simple-conv-PDE}. By showing that the solution of \cref{eqn:inhom-simple-conv-PDE} is actually unique we will get, via subsubsequence arguments, the convergence of the whole sequence.

\begin{proof} (Theorem \ref{inhom_simple_conv})


\textit{Part I : we first show that $\sup_{[0, 1] \times [0, 1]} | \kappa_{\D}^{x,y}
(t) - \Tilde{\kappa}_{\D}^{x, y} (t) | \to 0$ as $| \D | \rightarrow 0$.}

Note that trivially the set $\{x,y\}$ is bounded in $\bX$, we can thus fix two constants $C_{x,y}, R_{x,y}$ with the properties given in Proposition \ref{prop:inhom_bounded_set_bounds}. We will often, for ease of notation, refer to them as $C$ and $R$.

  We have, for $t \in [t_m, t_{m+1})$, that 
 \begin{align*}
     | \kappa_{\D}^{x,y} (t) - \Tilde{\kappa}_{\D}^{x, y} (t) |  & \leq
          |(\sigma_A^2 \Tilde{M}(1+ \sqrt{\Tilde{\kappa}_{\D}^{x, x}(t)})(1+ \sqrt{\Tilde{\kappa}_{\D}^{y, y}(t)}) + \sigma_b^2 ) 
           \sprod{\frac{x_t - x_{t_{m}}}{t - t_{m}}}{\frac{y_t - y_{t_{m}}}{t - t_{m}} }_{\R^d} (t - t_{m})|  \\
          &\leq  (2\sigma_A^2 \Tilde{M} (1 + C_{x,y}) + \sigma_b^2) 
          (|\frac{x_t - x_{t_{m}}}{t - t_{m}}|^2 + |\frac{y_t - y_{t_{m}}}{t - t_{m}}|^2)(t - t_{m}) \\
          &\leq (2\sigma_A^2 \Tilde{M} (1 + C_{x,y}) + \sigma_b^2) \int_{t_m}^t |\Dot{x}_s|^2 + |\Dot{y}_s|^2 ds
 \end{align*}
  
  In particular as $| \D | \rightarrow 0$ we
  have
    \begin{equation*} \begin{gathered}
    \sup_{[0, 1] \times [0, 1]} | \kappa_{\D}^{x,y}
     (t) - \Tilde{\kappa}_{\D}^{x, y} (t) | \to 0
     \end{gathered} \end{equation*}
  since, by dominated convergence, one has 
  \[
    \int_{t_m}^t |\Dot{x}_s|^2 + |\Dot{y}_s|^2 ds = \int_0^1 \mathbb{I}_{[t_m,t)} (|\Dot{x}_s|^2 + |\Dot{y}_s|^2) ds \to 0 
  \]
  

  \textit{- Part II : Ascoli-Arzelà}

  By \ref{prop:inhom_bounded_set_bounds} the sequence of functions $\{ \kappa_{\D_n}^{x, y} \}_{n}$ is unformly bounded.
  
Assume $s<t$ then one has, with the same bounds just used, that
    \begin{equation*}
      \begin{gathered}
          | \kappa_{\D}^{x,y} (t) - {\kappa}_{\D}^{x, y} (s) |  
          \leq  2(2\sigma_A^2 \Tilde{M} (1 + C_{x,y}) + \sigma_b^2) \int_{s}^t |\Dot{x}_r|^2 + |\Dot{y}_r|^2 ds
      \end{gathered}
  \end{equation*}
  thus the sequence of functions $\{ \kappa_{\D_n}^{x, y} \}_{n}$ is also uniformly equicontinuous, in fact the bound is independent from the partition. We can apply Ascoli-Arzelà to conclude that there exist a subsequence $\{\D_{n_k}\}$ with $\kappa_{\D_{n_k}}^{x, y}$ uniformly converging to a limiting $\kappa^{x,y} \in C^0([0,1];\R)$.  Since this must be the uniform limit of $\Tilde{\kappa}_{\D_{n_k}}^{x, y}$ too, by the result of \emph{Part} I,  we obtain that the corresponding limiting matrices $\Sigma^{x,y}(t) \in PSD_2(R_{x,y})$ for all $t \in [0,1]$
  \footnote{This is important to have a candidate solution to Equation (\ref{eqn:inhom-simple-conv-PDE}) which otherwise would not be well defined.}.

  \textit{- Part III :Uniqueness of solutions to Equation (\ref{eqn:inhom-simple-conv-PDE})} 
  
  Note that if the PDE (\ref{eqn:inhom-simple-conv-PDE}) admits a solution this must be unique: assume the existence of different solutions $K = (K_{x,x}, K_{x,x}, K^{x,y})$ and $ G = (G_{x,x}, G_{x,x}, G_{x,y})$ with all the $\Sigma^K$ and $\Sigma^G$ in $PSD_2$ . From Eq (\ref{eqn:inhom-simple-conv-PDE}) it is clear that $K_{x,x}, K_{y,y}, G_{x,x}, G_{y,y} \geq \sigma_{Y_0}^2$ and, by continuity, that they are bounded by some constant; thus all the $\Sigma_K$ and $\Sigma_G$ are in some in $PSD_2(\Bar{R})$. Then by the Lipschitz property of $V_{\varphi}$ one sees that
  \[
  \norm{\Sigma_K^{x,y}(t) - \Sigma_G^{x,y}(t)}_{\infty} \leq \int_0^t \sigma_A^2 k_{\Bar{R}}\norm{\Sigma_K^{x,y}(t) - \Sigma_G^{x,y}(t)}_{\infty} (|\sprod{\Dot{x}_r}{\Dot{x}_r}| + |\sprod{\Dot{x}_r}{\Dot{y}_r}| + |\sprod{\Dot{y}_r}{\Dot{y}_r}|) dr
  \]
  thus $ \norm{\Sigma_K^{x,y}(t) - \Sigma_G^{x,y}(t)}_{\infty} = 0$ by Gronwall for all $t \in [0,1]$ \emph{i.e} $K = G$.
  
  We now need to prove that the limit $\kappa^{x,y}$ of the $\kappa_{\D_{n_k}}^{x, y}$ solves the PDE, it will then follow that any sub-sequence of $\{\kappa_{\D_n}^{x,y}\}$ admits a further sub-sequence converging to the same map $\kappa^{x,y}$, giving us the convergence of the whole sequence. Thus without loss of generality we can assume in the sequel that the whole sequence converges.

  \textit{- Part IV : Limiti Kernel solves Equation (\ref{eqn:inhom-simple-conv-PDE})} 
    
  Let us prove that the limit $\kappa^{x, y}$ is, in fact,  a solution of the PDE. Let $t \in [t_m, t_{m+1})$ for some fixed $\D$, then
 \begin{equation*} \begin{gathered}
     \left| \kappa^{x, y} (t) - \sigma^2_{Y_0} +  \int_{0}^t (\sigma_A^2 V_{\varphi} (\Sigma^{x, y}(s)) + \sigma_b^2) \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d}   d s   \right|  \\
    \leq  | \kappa^{x, y} (t) - \kappa_{\D}^{x,y} (t) | + \sigma_A^2 \int_{0}^t | V_{\varphi}
    ({\Sigma}^{  x, y} (s))
    - V_{\varphi} (\tilde{\Sigma}_{\D}^{x, y} (s)) |  
    | \sprod{\Dot{x}_{s}}{\Dot{y}_{s}}_{\R^d} |    ds  \\
    + \sum_{0 \leq l < m} |\left( \sigma_A^2 V_{\varphi} \left(
     \Sigma^{\tmscript{x, x}}_{\D} (t_{l})
     \right) + \sigma_b^2 \right)||\int_{t_l}^{t_{l+1}}  \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d} ds - \sprod{\frac{\Delta x_{{t_{l + 1}} }}{\Delta t_{l + 1}}}{
     \frac{\Delta y_{t_{l + 1}}}{\Delta t_{l + 1}}}\Delta t_{l + 1}| \\
     + |\left( \sigma_A^2 V_{\varphi} \left(
     \Sigma^{\tmscript{x, x}}_{\D} (t_{m})
     \right) + \sigma_b^2 \right)||\int_{t_m}^{t}  \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d} ds - \sprod{\frac{x_t - x_{t_m}}{t - t_m}}{
     \frac{y_t - y_{t_m}}{t - t_m}}(t - t_m)|\\
     \leq | \kappa^{x, y} (t) - \kappa_{\D}^{x,y} (t) | + \sigma_A^2 \int_{0}^t | V_{\varphi}
    ({\Sigma}^{  x, y} (s))
    - V_{\varphi} (\tilde{\Sigma}_{\D}^{x, y} (s)) |  
    | \sprod{\Dot{x}_{s}}{\Dot{y}_{s}}_{\R^d} |    ds  \\
    + \left( 2 \sigma_A^2 \Tilde{M} (1 + C_{x,y}) + \sigma_b^2 \right)
    \big\{ \sum_{0 \leq l < m} |\int_{t_l}^{t_{l+1}}  \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d} ds - \sprod{\frac{\Delta x_{{t_{l + 1}} }}{\Delta t_{l + 1}}}{
     \frac{\Delta y_{t_{l + 1}}}{\Delta t_{l + 1}}}\Delta t_{l + 1}| \\
     + |\int_{t_m}^{t}  \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d} ds - \sprod{\frac{x_t - x_{t_m}}{t - t_m}}{
     \frac{y_t - y_{t_m}}{t - t_m}}(t - t_m)| \big\}
   \end{gathered} \end{equation*}
   but \cris{All this is too much for the approximation of the inner product of derivatives... can be shortened}
    \begin{equation*}
        \begin{gathered}
            |\int_{a}^{b}  \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d} ds
            - \sprod{\frac{x_b - x_{a}}{b-a}}{\frac{y_b - y_{a}}{b-a}}(b-a)| = \\
            |\int_{a}^{b}  \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d} 
            - \sprod{\frac{x_b - x_{a}}{b-a}}{\Dot{y}_s}_{\R^d} ds| = 
            |\int_{a}^{b}  \sprod{\Dot{x}_s - \frac{x_b - x_{a}}{b-a}}{ \Dot{y}_{s}}_{\R^d}  ds| \leq\\
            \int_{a}^{b} |\Dot{x}_s - \frac{x_b - x_{a}}{b-a}||\Dot{y}_{s}| ds
        \end{gathered}
    \end{equation*}
    hence
   \begin{equation*} \begin{gathered}
     \left| \kappa^{x, y} (t) - \sigma^2_{Y_0} +  \int_{0}^t (\sigma_A^2 V_{\varphi} (\Sigma^{x, y}(s)) + \sigma_b^2) \sprod{\Dot{x}_s}{ \Dot{y}_{s}}_{\R^d}   d s   \right|  \\
    \leq | \kappa^{x, y} (t) - \kappa_{\D}^{x,y} (t) | + \sigma_A^2 \int_{0}^t | V_{\varphi}
    ({\Sigma}^{  x, y} (s))
    - V_{\varphi} (\tilde{\Sigma}_{\D}^{x, y} (s)) |  
    | \sprod{\Dot{x}_{s}}{\Dot{y}_{s}}_{\R^d} |    ds  \\
    + \left( 2 \sigma_A^2 \Tilde{M} (1 + C_{x,y}) + \sigma_b^2 \right)
    \big\{ 
    \int_0^t \Big(\mathbb{I}_{[t_m, t)} |\Dot{x}_s - \frac{x_t - x_{t_{m}}}{t - t_m}| + \sum_{0 \leq l < m} \mathbb{I}_{[t_l, t_{l+1})} |\Dot{x}_s - \frac{\Delta x_{t_{l+1}}}{\Delta t_{l+1}}|\Big) |\Dot{y}_{s}| ds \big\}
   \end{gathered} \end{equation*}  
   
    Now, considering the sequence $\D_n$, by convergence 
    \[
    | \kappa^{x, y} (t) - \kappa_{\D_n}^{x, y} (t) | = o(1)
    \]
   and
    \[
        \int_{0}^t | V_{\varphi} ({\Sigma}^{  x, y} (s))  - V_{\varphi} (\tilde{\Sigma}_{\D_n}^{x, y} (s)) |  |\sprod{\Dot{x}_{s}}{\Dot{y}_{s}}_{\R^d}| ds
        \leq
        \int_{0}^t k_R  | \Sigma^{x, y} (s) - \Tilde{\Sigma}_{\D_n}^{x, y} (s) |_{\infty}  |\sprod{\Dot{x}_{s}}{\Dot{y}_{s}}_{\R^d}| ds = o(1)
    \]

    Moreover, setting $m_n$ to be such that $t \in [t_{m_n}, t_{m_n + 1})$ in $\D_n$, 
    \[\int_0^t \Big(\mathbb{I}_{[t^{\D_n}_{m_n}, t)} |\Dot{x}_s - \frac{x_t - x_{t^{\D_n}_{m_n}}}{t - t^{\D_n}_{m_n}}| + \sum_{0 \leq l < m_n} \mathbb{I}_{[t^{\D_n}_l, t^{\D_n}_{l+1})} |\Dot{x}_s - \frac{\Delta x_{t^{\D_n}_{l+1}}}{\Delta t^{\D_n}_{l+1}}|\Big) |\Dot{y}_{s}| ds = o(1)\]
    by Dominated convergence and Lebesgue differentiation theorem .
  
  thus
  \[ \left| \kappa^{x, y} (t) - \sigma^2_{Y_0} + \int_{0}^t (\sigma_A^2 V_{\varphi} (\Sigma^{x, y} (s)) + \sigma_b^2) 
     \sprod{\Dot{x}_{s}}{\Dot{y}_{s}}_{\R^d}     ds\right| = 0 \]
  i.e
  \[ \kappa^{x, y} (t) = \sigma^2_{Y_0} + \sigma^2_{Y_0} + \int_{0}^t (\sigma_A^2 V_{\varphi} (\Sigma^{x, y} (s)) + \sigma_b^2) 
     \sprod{\Dot{x}_{s}}{\Dot{y}_{s}}_{\R^d}     ds
 \]

  \nico{Be clearer with $\kappa^{x,y}$ and $K_{x,x}$}
  
\end{proof}

\subsubsection{Proof of Theorem \ref{thm:main-inhom-Kernels}}

It is finally time to prove the main result of the section, which we restate below for the reader's convenience. 
\cris{Have we not restated it already?}
\nico{Yes, but it was 9 pages ago}

Fix partitions $\{\D_M\}_{M \in \N}$ of $[0,1]$ with $|\D_M| \downarrow 0$.
Write $\psi^{\D_M, N}_{hom}(\cdot) = \sprod{v^N}{S^{\D_M,N}_1(\cdot)}$ for the ResNet initialized with the \emph{time-homogeneous} scheme.


\begin{theorem}
Let the activation function $\varphi: \R \to \R$ be a linearly bounded, absolutely continuous map with exponentially bounded derivative.
For any subset $\X = \{x_1, \dots, x_n\} \subset \bX$ the following convergence in distribution holds
\[
    \lim_{M \to \infty} \lim_{N \to \infty} \psi^{\D_M, N}_{in}(\X)
    =
    \mathcal{N}(0,\kappa^{in}_{\varphi}(\X, \X))
\]
where the map $\kappa^{in}_{\varphi} : \bX \times \bX \to \R$ is given by the unique
final values $\kappa_{\varphi}^{x,y}(1)$ of the following differential equation:

\begin{equation}\label{eqn:app_inhom_kernel}
\begin{gathered}
      \kappa_{\varphi}^{x,y}(t) =  \sigma_{Y_0 }^2  + 
      \int_{\tau = 0}^{t} 
      \Big[ 
      \sigma_A^2 \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}^{x, y}_{\tau})} 
      [ \varphi(Z_1) \varphi(Z_2) ] 
      + 
      \sigma_b^2 
      \Big] 
     \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d}   d \tau 
\end{gathered}
\end{equation}
with 
\[ 
    {\Sigma}^{x, y}_{t} = 
     \left(\begin{array}{c}
       \kappa_{\varphi}^{x,x}(t), \kappa_{\varphi}^{x,y}(t)\\
       \kappa_{\varphi}^{x,y}(t), \kappa_{\varphi}^{y, y}(t)
     \end{array}\right) 
\]

\emph{i.e.} the finite dimensional distributions of the stochastic process $\psi_{\D_M}^N(\cdot)$ indexed on $\bX$ 
    converge weakly to the corresponding ones of the Gaussian Process $\mathcal{GP}(0,\kappa^{in}_{\varphi})$.
\end{theorem}

\begin{proof}
    The proof is now just a matter of combining Theorem \ref{thm:inhom-discrete-phi-SigKer} and Theorem \ref{inhom_simple_conv}.

    Under our hypotheses Theorem \ref{thm:inhom-discrete-phi-SigKer} tells us that, for any subset $\X = \{x_1, \dots, x_n\} \subset \bX$, we have in distribution
\[
    \lim_{N \to \infty} \mathcal{L}(\psi^{\D_M, N}_{in}(\X) )
    =
    \mathcal{N}(0,\kappa_{\D_M}(\X, \X))
\]
thus to conclude we just have to prove that, still in distribution, it holds
\[
    \lim_{M \to \infty} \mathcal{N}(0,\kappa_{\D_M}(\X, \X))
    =
    \mathcal{N}(0, \kappa_{\varphi}(\X, \X))
\]
or, equivalently, that in $R^{n\times n}$ it holds $\lim_{M \to \infty} \kappa_{\D_M}(\X, \X) = \kappa_{\varphi}(\X, \X)$.

This last needed limit follows from Theorem \ref{inhom_simple_conv} with the sequence $\{\D_M \}_{M \in \N}$.

\end{proof}

We can now study some particular cases:
\begin{corollary}
    If $\varphi = id$, then 
    \begin{equation}\label{eqn:app_inhom-id-case}
        \kappa_{id}^{x,y} (t) = \big( \sigma_{Y_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big) \exp\big \{\sigma_A^2 \int_{\tau = 0}^t \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d} d\tau \big\} - \frac{\sigma_b^2}{\sigma_A^2}
    \end{equation}

    If $\varphi = ReLu$ and $x=y$, then 
    \begin{equation}\label{eqn:app_inhom-ReLU-case}
    \kappa_{ReLu}^{x,x} (t) = \big( \sigma_{Y_0}^2 + \frac{2 \sigma_b^2}{\sigma_A^2}\big) \exp\big \{\frac{\sigma_A^2}{2} \int_{\tau = 0}^t \norm{\Dot{x}_{\tau}}_{\R^d}^2 d\tau \big\} - \frac{2 \sigma_b^2}{\sigma_A^2}
    \end{equation}
\end{corollary}

\begin{proof}
    This is just a matter of computation. For the case $\varphi = id$ one has
    \[
        \E_{Z \sim \mathcal{N} (0, \Sigma)} 
      [ \varphi(Z_1) \varphi(Z_2) ]  =
      \E_{Z \sim \mathcal{N} (0, \Sigma)}
      [ Z_1 Z_2 ] =
      [\Sigma]_1^2
    \]
    hence
    \[
        \kappa_{id}^{x,y} (t) =  \sigma_{Y_0 }^2  + 
      \int_{\tau = 0}^{t} 
      \Big[ 
      \sigma_A^2 \kappa_{id}^{x,y} (s)
      + 
      \sigma_b^2 
      \Big] 
     \sprod{\Dot{x}_{s}}{ \Dot{y}_{s}}_{\R^d}   d s 
    \]

    Notice then that substituting (\ref{eqn:app_inhom-id-case}) for $K^{id}_{s} (x, y)$ in the integral leads to
    \begin{equation*}
        \begin{gathered}
          \sigma_{Y_0 }^2  + 
          \int_{\tau = 0}^{t} 
          \Big[ 
          \sigma_A^2 
          \Big\{ ( \sigma_{Y_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}) \exp \big \{\sigma_A^2 \int_{\tau = 0}^s \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d} d\tau \big\} - \frac{\sigma_b^2}{\sigma_A^2} \Big\}
          + 
          \sigma_b^2 
          \Big] 
         \sprod{\Dot{x}_{s}}{ \Dot{y}_{s}}_{\R^d}   ds =
         \\
         \sigma_{Y_0 }^2  + 
          \int_{\tau = 0}^{t} 
          \sigma_A^2 
          \big( \sigma_{Y_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big) \exp\big \{\sigma_A^2 \int_{\tau = 0}^s \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d} d\tau \big\} 
         \sprod{\Dot{x}_{s}}{ \Dot{y}_{s}}_{\R^d}   ds = 
         \\
         \sigma_{Y_0 }^2  + 
          \int_{\tau = 0}^{t} 
          ( \sigma_{Y_0}^2 + \frac{\sigma_b^2}{\sigma_A^2} )
          \partial_T \Big( \exp\big \{\sigma_A^2 \int_{\tau = 0}^T \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d} d\tau \big\} \Big)|_{T=s}   ds =
          \\
          \sigma_{Y_0 }^2  + 
           ( \sigma_{Y_0}^2 + \frac{\sigma_b^2}{\sigma_A^2} )
          \Bigg[
          \exp\big \{\sigma_A^2 \int_{\tau = 0}^t \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d} d\tau \big\}
          - 1
          \Bigg] = 
          \\
          ( \sigma_{Y_0}^2 + \frac{\sigma_b^2}{\sigma_A^2} )
          \exp\big \{\sigma_A^2 \int_{\tau = 0}^t \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d} d\tau \big\}
          - \frac{\sigma_b^2}{\sigma_A^2}
        \end{gathered}
    \end{equation*}
    which means, by uniqueness of solutions, that the thesis holds.

    For what concerns the case $\varphi = ReLU$ notice that for one dimensional Gaussian variables centered in the origin one has 
    \[
    \E_{Z \sim \mathcal{N} (0, \sigma^2)} 
      [ ReLU(Z)^2]  =
      \frac{1}{2}\E_{Z \sim \mathcal{N} (0, \sigma^2)}
      [ Z^2 ] =
      \frac{1}{2}\sigma^2
    \]
    hence since 
    \[
    \mathbb{E}_{Z \sim \mathcal{N} (0, K^{ReLU}_{s}(x,x)\mathbf{1})} 
      [ \varphi(Z_1) \varphi(Z_2) ] 
      =
      \E_{Z \sim \mathcal{N} (0, K^{ReLU}_{s}(x,x))} 
      [ ReLU(Z)^2] 
    \]
    one has
    \[
    \kappa_{ReLu}^{x,x} (t) =  \sigma_{Y_0 }^2  + 
      \int_{\tau = 0}^{t} 
      \Big[ 
      \frac{\sigma_A^2}{2}\kappa_{ReLu}^{x,x} (s)
      + 
      \sigma_b^2 
      \Big] 
     \sprod{\Dot{x}_{s}}{ \Dot{x}_{s}}_{\R^d}   d s 
    \]
    which equals $K^{id}_{t} (x, x)$ after the substitution $\sigma_A \mapsto \frac{\sigma_A}{\sqrt{2}}$.
\end{proof}

\begin{lemma}\label{app:lemma:inhom_simpler_form}
For all choices $(\sigma_{Y_0}, \sigma_A, \sigma_b)$ and for all $\varphi$ as in Theorem \ref{thm:main-inhom-Kernels} we have, with abuse of notation and the obvious meaning, that
\[
    \kappa_{\varphi}^{x,y}(t; \sigma_{Y_0}, \sigma_A, \sigma_b) = \kappa_{\varphi}^{\sigma_A x, \sigma_A y}(t; \sigma_{Y_0}, 1,{\sigma_b}{\sigma_A^{-1}})
\]
\end{lemma}

\begin{proof}
    We have
    \begin{equation*}
    \begin{gathered}
          \kappa_{\varphi}^{x,y}(t; \sigma_{Y_0}, \sigma_A, \sigma_b) =  \sigma_{Y_0 }^2  + 
          \int_{\tau = 0}^{t} 
          \Big[ 
          \sigma_A^2 \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}_{\varphi}^{x,y}{(\tau; \sigma_{Y_0}, \sigma_A, \sigma_b)}} 
          [ \varphi(Z_1) \varphi(Z_2) ] 
          + 
          \sigma_b^2 
          \Big] 
         \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d}   d \tau 
         \\
          =  \sigma_{Y_0 }^2  + 
          \int_{\tau = 0}^{t} 
          \sigma_A^2 \Big[ 
          \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}_{\varphi}^{x,y}{(\tau; \sigma_{Y_0}, \sigma_A, \sigma_b)}} 
          [ \varphi(Z_1) \varphi(Z_2) ] 
          + 
          \frac{\sigma_b^2}{\sigma_A^2} 
          \Big] 
         \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\tau}}_{\R^d}   d \tau
         \\
         =  \sigma_{Y_0 }^2  + 
          \int_{\tau = 0}^{t} 
           \Big[ 
          \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}_{\varphi}^{x,y}{(\tau; \sigma_{Y_0}, \sigma_A, \sigma_b)}} 
          [ \varphi(Z_1) \varphi(Z_2) ] 
          + 
          \frac{\sigma_b^2}{\sigma_A^2} 
          \Big] 
         \sprod{\sigma_A\Dot{x}_{\tau}}{\sigma_A \Dot{y}_{\tau}}_{\R^d}   d \tau
    \end{gathered}
    \end{equation*}
    and
    \begin{equation*}
    \begin{gathered}
          \kappa_{\varphi}^{\sigma_A x, \sigma_A y}(t; \sigma_{Y_0}, 1,{\sigma_b}{\sigma_A^{-1}}) = \sigma_{Y_0 }^2  + 
          \int_{\tau = 0}^{t} 
           \Big[ 
          \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}_{\varphi}^{\sigma_A x, \sigma_A y}{(\tau; \sigma_{Y_0}, 1,\frac{\sigma_b}{\sigma_A})}} 
          [ \varphi(Z_1) \varphi(Z_2) ] 
          + 
          \frac{\sigma_b^2}{\sigma_A^2} 
          \Big] 
         \sprod{\sigma_A\Dot{x}_{\tau}}{\sigma_A \Dot{y}_{\tau}}_{\R^d}   d \tau
    \end{gathered}
    \end{equation*}
    Thus the respective triplets solve the same equation and we can conclude by uniqueness.
\end{proof}

\subsection{The Infinite-Depth-then-Width limit}

In this section we will follow arguments used in \cite{hayou2022infinite}, extending the results obtained therein.

\subsubsection{Going to continuous time}

Here we consider the infinite depth limit and we get the solution of a SDE.

\begin{proposition}\label{prop:app-inf-dep-limit-hayou}
    Assume the activation function $\varphi$ to be Lipschitz and linearly bounded. Let $\rho_M(t) := \sup \{ s \in \D_M : s \leq t\}$ and $x \in \bX \cap C^{1,\frac{1}{2}}$ \emph{i.e.} $x$ has $\frac{1}{2}$-H\"{o}lder derivative.
    Then the process $X^{\D_M,N}_t(x) := Y^{\D_M,N}_{\rho_M(t)}(x)$ converges in distribution, as $M \to \infty$, to the solution of the following stochastic differential equation
    \begin{equation}\label{eqn:app-inhom-inf-depth-1}
    \begin{gathered}
        X^{N}_t(x) = Y_0 + \sum_{k=1}^d  \int_0^t
        \frac{\sigma_A}{\sqrt{N}} \Dot{x}^k_s dW^k_s [\varphi(X^N_s(x))] + \sigma_b \dot{x}^k_s dB^k_s
    \end{gathered}
    \end{equation}
    with $W^k_t \in \R^{N \times N}$ and $B^k_t \in \R^N$ are independent standard Brownian motions.
\end{proposition}

\cris{No need to have $X$ and $Y$ around for the same equation}

\begin{proof}
    We will transform Equation (\ref{eqn:app-inhom-inf-depth-1}) in a usual SDE form to then use the classical result \cite{kloeden1992numerical}[Theorem 10.2.2] to prove the convergence of Euler Discretizations to the unique solution. 

    We can restate Equation (\ref{eqn:app-inhom-inf-depth-1}) as
    \[
        X^{N}_t(x) = Y_0 + \int_0^t \sigma_x(s,X^{N}_s(x)) d Z_s
    \]
    for a Brownian Motion $Z_t \in \R^{\Gamma_{d,N}}$ with $\Gamma_{d,N} = d N (N+1)$.

    Take in fact 
    $Z_t = [([W_s^1]^1)^T,([W_s^1]^2)^T,\dots,([W_s^N]^1)^T,(B^1_s)^T,([W_s^2]^1)^T,\dots,(B^d_s)^T]^T$
    \emph{i.e.} 
    \[
        [Z_t]_{i = N(N+1)(k-1) + N(m-1) + 1,\dots, N(N+1)(k-1) + Nm} = 
        \begin{cases}
            [W_s^k]^m & \text{if } m = 1,\dots,N
            \\
            B^k_s & \text{if } m = N + 1
        \end{cases}
    \]
    
    and $\sigma_x : [0,1] \times \R^N \to \R^{N\times\Gamma_{d,N}}$
    \[
     [\sigma_x(s,y)]_{i = 1, \dots, N}^{j = N(N+1)(k-1) + N(m-1) + 1,\dots, N(N+1)(k-1) + Nm }
     =
     \begin{cases}
            \frac{\sigma_A}{\sqrt{N}} \Dot{x}^k_s [\varphi(y)]_m Id_{N \times N} & \text{if } m = 1,\dots,N
            \\
            \sigma_b \Dot{x}^k_s Id_{N \times N} & \text{if } m = N + 1
    \end{cases}
    \]

    It is then just a matter of checking the required conditions to apply \cite{kloeden1992numerical}[Theorem 10.2.2]:
    \begin{enumerate}
        \item There is a $K > 0$ such that $\forall t \in [0,1]. \forall y, y' \in \R^N$ one has 
        \[
        \norm{\sigma(t,y) - \sigma(t,y')}_{F} \leq K \norm{y - y'}_{\R^N}
        \]
        \item There is a $K' > 0$ such that $\forall t \in [0,1]. \forall y \in \R^N$ one has 
        \[
        \norm{\sigma(t,y)}_{F} \leq K' (1 + \norm{y }_{\R^N})
        \]
        \item There is a $K'' > 0$ such that $\forall t, s\in [0,1]. \forall y \in \R^N$ one has 
        \[
        \norm{\sigma(t,y) - \sigma(s,y)}_{F} \leq K'' (1 + \norm{y}_{\R^N}) |t-s|^{\frac{1}{2}}
        \]
    \end{enumerate}

    As a first step note how
    \[
    \norm{\sigma(t,y)}_{F}^2 = 
    N \sum_{k=1}^d (\Dot{x}^k_t)^2 \big( \sigma_b^2 +\sum_{m=1}^N  \frac{\sigma_A^2}{N} ([\varphi(y)]_m )^2\big) =
    N \norm{\Dot{x}_t}_{\R^d}^2 (\sigma_b^2 + \sigma_A^2\frac{\norm{\varphi(y)}_{\R^N}^2}{N})
    \]
    thus using sublinearity of $\varphi$ for some $M>0$ one has
    \[
    \norm{\sigma(t,y)}_{F}^2 \leq N \norm{\Dot{x}_t}_{\R^d}^2 (\sigma_b^2 + \frac{\sigma_A^2}{N} M (1 + \norm{y}_{\R^N})^2)
    \]
    from which we easily get condition (ii). 
    
    For condition (i) note that 
    \[
     \norm{\sigma(t,y) - \sigma(t,y')}_{F}^2 = N \norm{\Dot{x}_t}_{\R^d}^2 \sigma_A^2\frac{\norm{\varphi(y) - \varphi(y')}_{\R^N}^2}{N}
    \]
    thus one just uses Lipschitz property of $\varphi$ with Lemma \ref{app:lipR_to_lipRn}.

    Finally for (iii) one computes just as before
    \[
    \norm{\sigma(t,y) - \sigma(s,y)}_{F}^2 = N \norm{\Dot{x}_t - \Dot{x}_s}_{\R^d}^2 (\sigma_b^2 + \sigma_A^2\frac{\norm{\varphi(y)}_{\R^N}^2}{N})
    \]
    and using H\"{o}lder property of $x$ and linear bound on $\varphi$ one has, for some $\Tilde{M} > 0$
    \[
    \norm{\sigma(t,y) - \sigma(s,y)}_{F}^2 \leq N(\sigma_b^2 + \frac{\sigma_A^2}{N} M (1 + \norm{y}_{\R^N})^2)\Tilde{M}^2|t-s|
    \]
    hence the concluding inequality
    \[
    \norm{\sigma(t,y) - \sigma(s,y)}_{F} \leq  (N\Tilde{M}(\sigma_b^2 + \frac{\sigma_A^2}{N} M)) (1 + \norm{y}_{\R^N})|t-s|^{\frac{1}{2}}
    \]

    Unfortunately we are not done since 
    \begin{equation*}
        \begin{gathered}
            Y^{\D_M,N}_{t^{\D_M}_l}(x) = Y^{\D_M,N}_{t^{\D_M}_{l-1}}(x) + \sum_{k=1}^d \frac{\Delta x^k_{t^{\D_M}_l}}{\Delta t^{\D_M}_l} (\frac{\sigma_A}{\sqrt{N}}\sqrt{\Delta t^{\D_M}_l} W_{k,l} \varphi(Y^{\D_M,N}_{t^{\D_M}_{l-1}}(x)) + \sigma_b\sqrt{\Delta t^M_l} B_{k,l} ) 
        \end{gathered}
    \end{equation*}
    is not the Euler discretization of the above SDE, in fact in general
    \[
        \frac{\Delta x^k_{t^{\D_M}_l}}{\Delta t^{\D_M}_l} \neq \Dot{x}^k_{t^{\D_M}_{l-1}}
    \]

    We have to prove that 
    \[
        \lim_{M \to \infty}\E[\sup\limits_{t\in [0,1]} |\Tilde{X}^{\D_M, N}_t(x) - X^{\D_M, N}_t(x)|] = 0
    \]
    where $\Tilde{X}^{\D_M, N}_t(x)$ is defined as ${X}^{\D_M, N}_t(x)$ but substituting the difference quotients with the actual derivatives.
    This follows from the fact that the piecewise constant, on partition intervals, approximations of $\Dot{x}^\kappa(t)$ given by finite difference quotients converge uniformly to it since for any $r \in [a,b]\subseteq[0,1]$ one has
    \[
     |\frac{x_b - x_a}{b-a}  -  \Dot{x}_r| = |\frac{1}{b-a}\int_a^b \Dot{x}_s ds -  \Dot{x}_r| = 
     \frac{1}{b-a}\int_a^b |\Dot{x}_s ds -  \Dot{x}_r| ds \leq |b-a|^{\frac{1}{2}}
    \] 
    by H\"{o}lder continuity. 

    \nico{More details?}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
We can extend this by considering multiple input paths at the same time to preserve the joint distribution: 
\begin{proposition}
    Assume to be under the assumptions of Proposition (\ref{prop:app-inf-dep-limit-hayou}).
    Fix $\X := \{x_1, \dots, x_n\} \subset \bX \cap C^{1,\frac{1}{2}}$.
    The process $\mathbf{X}^{\D_M,N}_t(\X) := [X^{\D_M,N}_t(x_i)]_{i=1,\dots,n} := [Y^{\D_M,N}_{\rho_M(t)}(x_i)]_{i=1,\dots,n} \in \R^{Nn}$ converges in distribution, as $M \to \infty$, to the solution of the following stochastic differential equation
    \begin{equation}
    \begin{gathered}
        d\Tilde{\mathbf{X}}^{N}_t(\X) =  \sigma_{\X}(t, \Tilde{\mathbf{X}}^{N}_t(\X))^{\frac{1}{2}} d\mathbf{Z}_t\\
        \Tilde{\mathbf{X}}^{N}_0(x_k) := [\Tilde{\mathbf{X}}^{N}_0(\X)]_{i = (k-1)N + 1, \dots, kN} = Y_0
    \end{gathered}
    \end{equation}
    with $\mathbf{Z}_t \in \R^{nN}$ standard Brownian motion independent from $Y_0$ and $\Sigma(t, \Tilde{X}^{N}_t(\X)) \in \R^{nN\times nN}$
    the matrix
    \begin{equation}
    \begin{gathered}
        [\Sigma(t, \Tilde{\mathbf{X}}^{N}_t(\X))]_{i = (k-1)N + 1, \dots, kN }^{j =(m-1)N + 1, \dots, mN } =  \frac{\sigma_A^2}{N}\sprod{\varphi(\Tilde{\mathbf{X}}^{N}_t(x_k))}{\varphi(\Tilde{\mathbf{X}}^{N}_t(x_m))}_{\R^N} + \sigma_b^2
    \end{gathered}
    \end{equation}
\end{proposition}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Similarly we prove that
\begin{proposition}\label{prop:app-joint-hayou-trick}
    Assume to be under the assumptions of Proposition (\ref{prop:app-inf-dep-limit-hayou}).
    Fix $\X := \{x_1, \dots, x_n\} \subset \bX \cap C^{1,\frac{1}{2}}$.
    The process $\mathbf{X}^{\D_M,N}_t(\X) := [X^{\D_M,N}_t(x_i)]_{i=1,\dots,n} := [Y^{\D_M,N}_{\rho_M(t)}(x_i)]_{i=1,\dots,n} \in \R^{Nn}$ converges in distribution, as $M \to \infty$, to the solution of the following stochastic differential equation
    \begin{equation}\label{eqn:app-joint-hayou-trick}
    \begin{gathered}
        d\Tilde{\mathbf{X}}^{N}_t(\X) =   \Sigma_{\X}(t, \Tilde{\mathbf{X}}^{N}_t(\X))^{\frac{1}{2}} d\mathbf{Z}_t\\
        \Tilde{\mathbf{X}}^{N}_0(x_k) := [\Tilde{\mathbf{X}}^{N}_0(\X)]_{i = (k-1)N + 1, \dots, kN} = Y_0
    \end{gathered}
    \end{equation}
    with $\mathbf{Z}_t \in \R^{nN}$ standard Brownian motion independent from $Y_0$ and $\Sigma_{\X}(t, \Tilde{X}^{N}_t(\X)) \in \R^{nN\times nN}$
    the matrix
    \begin{equation}
    \begin{gathered}
        [\Sigma_{\X}(t, \Tilde{\mathbf{X}}^{N}_t(\X))]_{i = (k-1)N + 1, \dots, kN }^{j =(m-1)N + 1, \dots, mN } =  \sprod{\Dot{x}_k}{\Dot{x}_m}_{\R^d} \big[ \frac{\sigma_A^2}{N}\sprod{\varphi(\Tilde{\mathbf{X}}^{N}_t(x_k))}{\varphi(\Tilde{\mathbf{X}}^{N}_t(x_m))}_{\R^N} + \sigma_b^2 \big] I_{N\times N}
    \end{gathered}
    \end{equation}
\end{proposition}

\begin{proof}
    The main idea of the proof is that of constructing, for every $M$, an Euler scheme $\Bar{\mathbf{X}}_t^{\D_M, N}(\X)$ having same distribution as $\mathbf{X}^{\D_M,N}_t(\X)$ but converging to the solution of Equation (\ref{eqn:app-joint-hayou-trick}). 
    The result will follow from the uniqueness of the limit in distribution.

    We have, with the obvious abuses of notation for readability,
    \begin{equation*}
        \begin{gathered}
            Y^{\D_M,N}_{l}(x_m) = Y^{\D_M,N}_{l-1}(x_m) + \sum_{k=1}^d \frac{\Delta (x_m)^k_{t^M_l}}{\Delta t^M_l} (\frac{\sigma_A}{\sqrt{N}}\sqrt{\Delta t^M_l} W_{k,l} \varphi(Y^{\D_M,N}_{l-1}(x_m)) + \sigma_b\sqrt{\Delta t^M_l} B_{k,l} ) 
        \end{gathered}
    \end{equation*}
    with $W_{k,l} \in \R^{N \times N}$ and $B_{k,l} \in \R^N$ independent standard normally distributed matrices and vectors.

    We can rewrite this as 
    \begin{equation*}
        \begin{gathered}
            Y^{\D_M,N}_{l}(x_m) = Y^{\D_M,N}_{l-1}(x_m) + \sqrt{\Delta t^M_l} \Lambda^{\D_M, N}_{l} \zeta^{\D_M, N}_l(x_m) 
        \end{gathered}
    \end{equation*}
    for $\Lambda^{\D_M, N}_{l} \in \R^{N \times d(N+1)}$ and $\zeta^{\D_M, N}_l(x_i) \in \R^{d(N+1)}$ defined as
    \begin{equation*}
        \begin{gathered}
           [\Lambda^{\D_M, N}_{l}]_{i = 1, \dots, N}^{j = (k-1)(N+1)+1, \dots, k(N+1) } =  [W_{k,l} | B_{k,l}]
           \\
           [\zeta^{\D_M, N}_l(x_m)]_{i = (k-1)(N+1)+1, \dots, k(N+1) } = \frac{\Delta (x_m)^k_{t^M_l}}{\Delta t^M_l} [ \frac{\sigma_A}{\sqrt{N}} (\varphi(Y^{\D_M,N}_{l-1}(x_m)))^T | \sigma_b ]^T
        \end{gathered}
    \end{equation*}
    Let $\Xi^{\D_M, N}_l(x_m) := \Lambda^{\D_M, N}_{l} \zeta^{\D_M, N}_l(x_m)$.
    Denote by $\textbf{Y}^{\D_M,N}_{l}(\X)$ the concatenation of the $Y^{\D_M,N}_{l}(x_m)$, and $\mathbf{\Xi}^{\D_M,N}_{l}(\X)$ similarly.
    Then
    \[
        \textbf{Y}^{\D_M,N}_{l}(\X) = \textbf{Y}^{\D_M,N}_{l-1}(\X) + \sqrt{\Delta t^M_l}\mathbf{\Xi}^{\D_M,N}_{l}(\X)
    \]
    
    Since the covariance matrix $\Sigma(\mathbf{\Xi}^{\D_M,N}_{l}(\X))$ of $\mathbf{\Xi}^{\D_M,N}_{l}(\X)$ has form 
    \[
        [\Sigma(\mathbf{\Xi}^{\D_M,N}_{l}(\X))]_{i = (k-1)N + 1, \dots, kN }^{j =(m-1)N + 1, \dots, mN } =  
        \sprod{\frac{\Delta (x_k)_{t^M_l}}{\Delta t^M_l}}{\frac{\Delta (x_m)_{t^M_l}}{\Delta t^M_l}}_{\R^d} 
        \big[ \frac{\sigma_A^2}{N}\sprod{\varphi(Y^{\D_M,N}_{l}(x_k))}{\varphi(Y^{\D_M,N}_{l}(x_m))}_{\R^N} + \sigma_b^2 \big] 
        I_{N\times N}
    \]
    and since $\Sigma(\mathbf{\Xi}^{\D_M,N}_{l}(\X))$ is distributed as $(\Sigma(\mathbf{\Xi}^{\D_M,N}_{l}(\X)))^{\frac{1}{2}}Z_l$ for some standard Gaussian $^{\D_M,N}Z_l \in \R^{nN}$ dependent only on the $\sigma$-algebra generated by $\Lambda^{\D_M, N}_{l}$, to conclude simply reason as in the proof of Proposition \ref{prop:app-inf-dep-limit-hayou}. 
    
\end{proof}


\subsubsection{Infinite-depth-then-width limit in the linear case}

We now prove 
\begin{proposition}
Let $\varphi = id$. For any subset $\X = \{x_1, \dots, x_n\} \subset \bX$.
Then for all integers $N\geq 1$ and for all $k,m = 1,\dots,d$ that the following convergence holds
\[
    \lim_{M \to \infty} \E[ \psi^{\D_M, N}_{in}(\X)\psi^{\D_M, N}_{in}(\X) ] 
    =
    \kappa_{id}^{in}(\X,\X)
\]
\end{proposition}

\begin{proof}
    To start notice that
    \[
    \E[ \psi^{\D_M, N}_{in}(x_k)\psi^{\D_M, N}_{in}(x_m) ]=
    \E[ \frac{\sprod{{Y^{\D_M,N}_{1}}(x_k)}{{Y^{\D_M,N}_{1}}(x_m)}}{N}]
    \]
    
    From \ref{prop:app-joint-hayou-trick} we have 
    \[
        \lim_{M \to \infty} \E[ \frac{\sprod{{Y^{\D_M,N}_{1}}(x_k)}{{Y^{\D_M,N}_{1}}(x_m)}}{N}] = 
        \E[ \frac{\sprod{\Tilde{\mathbf{X}}^{N}_1(x_k)}{\Tilde{\mathbf{X}}^{N}_1(x_m)}}{N}]
    \]
    and by It\^{o}'s lemma 
    \[
    \E[ \frac{\sprod{\Tilde{\mathbf{X}}^{N}_1(x_k)}{\Tilde{\mathbf{X}}^{N}_1(x_m)}}{N}] =
    \sigma_{Y_0}^2 + 
    \int_0^1
    \big( 
    \sigma_A^2 \E[\frac{\sprod{\Tilde{\mathbf{X}}^{N}_s(x_k)}{\Tilde{\mathbf{X}}^{N}_s(x_m)}}{N}] + \sigma_b^2 \big)
    \sprod{\Dot{x}_s}{\Dot{y}_s}_{\R^d} ds
    \]

    Defining $K^N_t(x_k,x_m) := \E[ \frac{\sprod{\Tilde{\mathbf{X}}^{N}_t(x_k)}{\Tilde{\mathbf{X}}^{N}_t(x_m)}}{N}]$ and noticing that we can repeat the previous arguments for all $t \in [0,1]$, not only for $t=1$, we see that
    \[
        K^N_t(x_k,x_m) = \sigma_{Y_0}^2 + 
    \int_0^t
    \big( 
    \sigma_A^2 K^N_s(x_k,x_m) + \sigma_b^2 \big)
    \sprod{\Dot{x}_s}{\Dot{y}_s}_{\R^d} ds
    \]
    meaning that $K^N_t(x_k,x_m)$ solves Equation (\ref{eqn:app_inhom_kernel}). 

    Since we showed in the proof of Theorem \ref{inhom_simple_conv} that the unique solution to the equation is $\kappa_{id}^{x_k,x_m}(1)$ we conclude.
    
\end{proof}

\section{Homogeneous Case}

In this section of the appendix we are going to prove all the results for the homogeneous case.

Recall that the \emph{homogeneous controlled ResNet}  model is defined as follows: fixed a partition $\D$, the \emph{hidden dimension} $N$ and the activation function $\varphi: \R \to \R$ we have defined the models as 
\[
    \psi^{\D, N}_{hom}(x) := \sprod{v^N}{S^{\D,N}_1(x)}_{\R^N}
\]
where $v^N \sim \mathcal{N}(0,\frac{1}{N})$ and $S^{\D,N} : \D \times \bX \to \R^N$ is the final value of:
\[
    S^{\D_M,N}_{t_m}(x) = S_0 + \sum_{l=1}^m \sum_{k=1}^d \big( A_{k} \varphi(S^{\D_M, N}_{t_{l-1}}(x)) + b_{k} \big) \Delta x^k_{t_l}
\]
with $\varphi$ applied componentwise and the components of $A_{k} \in \R^{N\times N}$,$b_{k} \in \R^N$ sampled according to
\begin{equation*}
\begin{gathered}
    [A_{k}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{\sigma_{A}^2}{N})     
    \hspace{15pt}
    [Y_0]_{\alpha}\sim \mathcal{N}(0,\sigma_{S_0}^2)
    \hspace{15pt}
    [b_{k}]_{\alpha} \sim \mathcal{N}(0,\sigma_b^2)
\end{gathered}
\end{equation*}
independently from each other and from $v^N$.



The section too will be subdivided in two main parts: in the first we consider the infinite-width-then-depth limit and in the second we reverse the order and consider the infinite-depth-then-width limit.


\subsection{The infinite-width-then-depth limit}\label{appendix:hom-WD-limit}
The main goal is that of proving Theorem \ref{thm:phi-SigKer}, which we restate here:
\begin{theorem}
Let the activation function $\varphi: \R \to \R$ be a linearly bounded, absolutely continuous map with exponentially bounded derivative.
Let $\{\D_M\}$ be any sequence of partitions of $[0,1]$ with $|\D_M| \to 0$.
For any subset $\X = \{x_1, \dots, x_n\} \subset \bX$ the following convergence in distribution holds
\[
    \lim_{M \to \infty} \lim_{N \to \infty} \psi^{\D_M, N}_{hom}(\X) 
    =
    \mathcal{N}(0,K^{hom}_{\varphi}(\X, \X))
\]
where the map $K^{hom}_{\varphi} : \bX \times \bX \to \R$ is given by the unique
final values $K_{\varphi}^{x,y}(1, 1)$ of the following integro-differential equation
\begin{equation}\label{eqn:hom_kernel}
%\resizebox{\hsize}{!}{$
\begin{gathered}
      K_{\varphi}^{x, y}(t, s) =  \sigma_{S_0 }^2  +  
      \int_{\tau = 0}^{t} \int_{\sigma = 0}^{s} 
      \Big[ 
      \sigma_A^2 \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}^{x, y}_{\tau, \sigma})} 
      [ \varphi(Z_1) \varphi(Z_2) ] 
      + 
      \sigma_b^2 
      \Big] 
     \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
\end{gathered}
%$}
\end{equation}

with 
\[ 
    {\Sigma}^{x, y}_{t,s} = 
     \left(\begin{array}{c}
       K_{\varphi}^{x, x}(t, t), K_{\varphi}^{x, y}(t, s)\\
       K_{\varphi}^{x, y}(t, s), K_{\varphi}^{y, y}(s, s)
     \end{array}\right) 
\]
\emph{i.e.} the finite dimensional distributions of the stochastic process $\psi^{\D_M,N}_{hom}(\cdot)$ indexed on $\bX$ 
    converge weakly to the corresponding ones of the Gaussian Process $\mathcal{GP}(0,K^{hom}_{\varphi})$.
\end{theorem}

Once again, it is clearer to subdivide the proof of this result in two parts:
\begin{enumerate}
    \item The infinite width-convergence of the finite dimensional distributions 
    \[
    \mathcal{L}(\psi^{\D_M, N}_{hom}(\X) ) \xrightarrow[]{N \to \infty} \mathcal{N}(0, K_{\D_M \times \D_M}(\X,\X))
    \]
    to those of a Gaussian process $\mathcal{GP}(0,K_{\D_M \times \D_M})$ defined by a Kernel computed as the final value of a difference equation on the "partition" $\D_M \times \D_M$ of $[0,1]\times[0,1]$. This will be done using Tensor Programs \cite{yang2019wide} in \ref{subsubsec:discrete-phi-SK}.
    
    \item The infinite-depth convergence of the \emph{discrete Kernels} $K_{\D_M \times \D_M}$ to a limiting Kernel $K_{\varphi}$ which solves the differential equation in Theorem \ref{thm:phi-SigKer}. This will be done in \ref{subsubsec:conv-phi-SK}.
\end{enumerate}


\subsubsection{Infinite-width limit with fixed-depth}\label{subsubsec:discrete-phi-SK}
With the notation of \ref{subsec:body-phi-infWDlimit} we will prove, using the formalism of \emph{Tensor Programs}, that

\begin{theorem}\label{thm:discrete-phi-SigKer}
Let the activation function $\varphi: \R \to \R$ be linearly bounded
\footnote{in the sense that $\exists C > 0.$ such that $|\phi(x)| \leq C(1+|x|)$.}.
For any subset $\X = \{x_1, \dots, x_n\} \subset \bX$ the following convergence in distribution holds
\[
    \lim_{N \to \infty} \psi^{\D_M, N}_{hom}(\X) 
    =
    \mathcal{N}(0,K_{\D_M \times \D_M}(\X, \X))
\]
where the map $K_{\D \times \D'} : \bX \times \bX \to \R$ is, given any two partitions $\D, \D'$ of $[0,1]$, by the unique final values $K_{\D \times \D'}^{x,y}(1, 1)$ of the following planar finite difference scheme on $\D \times \D'$
\begin{equation}\label{eqn:hom-discrete-kernel}
%\resizebox{0.8\hsize}{!}{$
\begin{gathered}
    K_{\D \times \D'}^{x,y}(t^{\D}_{m}, s^{\D'}_n) = K_{\D \times \D'}^{x, y}({t^{\D}_{m-1},s^{\D'}_{n}}) + K_{\D \times \D'}^{x, y}({t^{\D}_{m},s^{\D'}_{n-1}}) - K_{\D \times \D'}^{x, y}({t^{\D}_{m-1},s^{\D'}_{n-1}})
    \\
    + \Big( \sigma_A^2 
    \E_{Z \sim \mathcal{N}(0, \Sigma_{\D \times \D'}^{x, y}(t^{\D}_{m-1},s^{\D'}_{n-1})}[ \varphi(Z_1) \varphi(Z_2) ]
    + \sigma_b^2 \Big)  \sprod{\Delta x_{t^{\D}_m}}{\Delta y_{s^{\D'}_n} }_{\R^d}
    \\
    \vspace{5pt}
    K_{\D \times \D'}^{x, y}({0,0}) = K_{\D \times \D'}^{x, y}({0,s^{\D'}_{n}}) = K_{\D \times \D'}^{x, y}({t^{\D}_{m},0}) = \sigma_{S_0}^2
\end{gathered}
%$}
\end{equation}
where 
\[
    \Sigma_{\D \times \D'}^{x, y}(t,s) =  
    \begin{pmatrix}
        K_{\D \times \D'}^{x, x}({t,t}) & K_{\D \times \D'}^{x, y}({t,s}) \\
         K_{\D \times \D'}^{x, y}({t,s}) & K_{\D' \times \D'}^{y,y}(s,s)
    \end{pmatrix}
\]
\end{theorem}

\begin{proof}
    We use \cite{yang2019wide}[Corollary 5.5] applied to the Tensor Program of Algorithm \ref{Algo:TimeDep} where the input variables are independently sampled according to
    \[
    [A_{k}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{\sigma_{A}^2}{N}), 
    [v]_{\alpha}\sim \mathcal{N}(0,{1}),
    [S_0]_{\alpha}\sim \mathcal{N}(0,\sigma_{S_0}^2)
    \hspace{5pt} and \hspace{5pt} 
    [b_{k}]_{\alpha} \sim \mathcal{N}(0,\sigma_b^2)
\]
Note how the sampling scheme follows \cite{yang2019wide}[Assumption 5.1] and how linearly bounded functions are \emph{controlled} in the sense of \cite{yang2019wide}[Definition 5.3] since for all $x \in \R$ one has $|\phi(x)| \leq C(1+|x|) \leq e^{|x| + log(C)}$.
Thus we are under the needed assumptions to apply \cite{yang2019wide}[Corollary 5.5].

There are two things to notice, done in order to satisfy the required formalism: 
\begin{itemize}
    \item In the program the output projector $v$ is sampled according to $\mathcal{N}(0,1)$ while the original $v^N \sim \mathcal{N}(0,\frac{1}{N})$. This does not pose any problems since the output of the formal programs uses ${v}/{\sqrt{N}}\sim \mathcal{N}(0,\frac{1}{N})$.
    \item The input paths $x_i$ enter program \ref{Algo:TimeDep} not as \emph{Inputs} but as coefficients of \emph{LinComb}, this means that for any choice of input paths we must formally consider different algorithms. In any case, for any possible choice, the result has always the same functional form; hence \emph{a posteriori} it is legitimate to think about \emph{one} algorithm.
\end{itemize}

Note that $S^{x}_{m}$ stands for the formal variable in program \ref{Algo:TimeDep}, not for $S^{\D_M, N}_{t^{\D_M}_m}(x)$ even thogh this is the value which it "stores" for a fixed hidden dimension $N$.

The result in \cite{yang2019wide}[Corollary 5.5] tells us that the output vector converges in law, as $N \to \infty$, to a Gaussian distribution $\mathcal{N}(0, \Tilde{K}^M)$ where
\[
    [\Tilde{K}^M]_i^j = \E_{Z \sim \mathcal{N}(\mu^M, \Sigma^M)}
    \bigg[
    Z^{S^{x_i}_{\norm{\mathcal{D}_M}}} Z^{S^{x_j}_{\norm{\mathcal{D}_M}}}
    \bigg]
    =
    \Sigma^M(S^{x_i}_{\norm{\mathcal{D}_M}}, S^{x_j}_{\norm{\mathcal{D}_M}})
\]

with $\mu^M, \Sigma^M$ computed according to \cite{yang2019wide}[Definition 5.2] and defined on the set of all G-vars in the program \emph{i.e.}

\begin{equation*}
    \mu^M(g) = \begin{cases}
      \mu^{M, in}(g) & \text{if $g$ is \textbf{Input} G-var}\\
      \sum_k a_k \mu^M(g_k) & \text{if $g$ is introduced as $\sum_k a_k g_k$ via \textbf{LinComb}}\\
      0 & \text{otherwise}
    \end{cases}
\end{equation*}
\begin{equation*}
    \Sigma^M(g, g') =  \begin{cases}
      \Sigma^{M, in}(g, g') & \text{if both $g$ and $g'$ are \textbf{Input} G-var}\\
      \sum_k a_k \Sigma^M(g_k, g') & \text{if $g$ is introduced as $\sum_k a_k g_k$ via \textbf{LinComb}}\\
      \sum_k a_k \Sigma^M(g, g_k') & \text{if $g'$ is introduced as $\sum_k a_k g'_k$ via \textbf{LinComb}}\\
      \sigma_W^2 \E_{Z \sim \mathcal{N}(\mu^M, \Sigma^M)}[\phi(Z)\phi'(Z)]& \text{if $g = Wh$, $g' = Wh'$ via \textbf{MatMul} w/ same $W$}\\
      0 & \text{otherwise}
    \end{cases}
\end{equation*}

where $h = \phi((g_k)_{k=1}^{m})$ for some function $\phi$ and $\phi(Z) := \phi((Z^{g_k})_{k=1}^{m})$, similarly for $g'$.

In our setting $\mu^{M, in} \equiv 0$ since all \textbf{Input} variables are independent, from which $\mu^M \equiv 0$; furthermore $\Sigma^{M, in}(g, g') = 0$ except if $g = g'$ when it takes values in $\{ \sigma^2_{S_0}, \sigma^2_{b}, \sigma^2_{A}\}$ accordingly.

Following the rules of $\Sigma^M$, assuming $m_i, m_j \in \{1, \dots, \norm{\mathcal{D}_M} \}$, we obtain
\begin{eqnarray*}
  \Sigma^M (S^{x_i}_{m_i}, S^{x_j}_{m_j}) & = & \Sigma^M (S^{x_i}_{m_i - 1}, S^{x_j}_{m_j}) +
  \Sigma^M \left( \sum_{k = 1}^d \gamma_{m_i, k}^i \Delta (x_i)_{t_{m_i}}^k,
  S^{x_j}_{m_j} \right)\\
  & = & \Sigma^M (S^{x_i}_{m_i - 1}, S^{x_j}_{m_j}) + \Sigma^M \left( \sum_{k = 1}^d
  \gamma_{m_i, k}^i \Delta (x_i)_{t_{m_i}}^k, S^{x_j}_{m_j-1} \right)\\
  &  & + \Sigma^M \left( \sum_{k = 1}^d \gamma_{m_i, k}^i \Delta
  (x_i)_{t_{m_i}}^k, \sum_{l = 1}^d \gamma_{m_j, l}^j \Delta
  (x_j)_{t_{m_j}}^l \right)\\
  & = & \Sigma^M (S^{x_i}_{m_i - 1}, S^{x_j}_{m_j}) + \Sigma^M (S^{x_i}_{m_i}, S^{x_j}_{m_j-1})
  - \Sigma^M (S^{x_i}_{m_i - 1}, S^{x_j}_{m_j-1})\\
  &  & + \sum_{k, l = 1}^d \Sigma^M (\gamma_{m_i, k}^i, \gamma_{m_j, l}^j)
  \Delta (x_i)_{t_{m_i}}^k \Delta (x_j)_{t_{m_j}}^l
\end{eqnarray*}

Now
\[ 
    \Sigma^M (\gamma_{m_i, k}^i, \gamma_{m_j, l}^j) 
    = \delta_{k, l} \sigma_{A}^2
    \E[\varphi(Z_1)\varphi(Z_2)]
    +
    \Sigma^M(b_k, b_l)
    = \delta_{k l} \big[ 
    \sigma_{A}^2 
    \E[\varphi(Z_1)\varphi(Z_2)]
    + \sigma_b^2
    \big]
\]
   
where $[Z_{1,} Z_2]^{\top} \sim \mathcal{N} (0, \tilde{\Sigma}^M_{m_i - 1, m_j - 1}(x_i, x_j))$  with

\begin{eqnarray*}
  \tilde{\Sigma}^M_{m, m'}(x_i, x_j) & = 
  & \left(\begin{array}{c c}
    \Sigma^M (S^{x_i}_{m}, S^{x_i }_{m}) & 
    \Sigma^M (S^{x_i}_{m}, S^{x_j }_{m'})\\
    \Sigma^M (S^{x_i}_{m}, S^{x_j }_{m'}) & 
    \Sigma^M (S^{x_j }_{m'}, S^{x_j }_{m'})
  \end{array}\right)
\end{eqnarray*}

thus if we set, for $t_{m_i}, t_{m_j} \in \D_M$,  $K_{\D_M \times \D_M}^{x_i, x_j}(t_{m_i}, t_{m_j}) := \Sigma^M(S^{x_i}_{m_i}, S^{x_j}_{m_j})$ then we get
\begin{eqnarray*}
  K_{\D_M \times \D_M}^{x_i, x_j}(t_{m_i}, t_{m_j}) & = & K_{\D_M \times \D_M}^{x_i, x_j}({t_{m_i - 1}, t_{m_j}}) + K_{\D_M \times \D_M}^{x_i, x_j}(({t_{m_i}, t_{m_j - 1}}) - 
  K_{\D_M \times \D_M}^{x_i, x_j}(({t_{m_i - 1}, t_{m_j - 1}})\\
  &  &+ \sum_{k = 1}^d \big( \sigma_A^2 \mathbb{E}_{(Z_x, Z_y)
  \sim \mathcal{N} (0, \tilde{\Sigma}^M_{m_{i-1}, m_{j-1}}(x_i, x_j))} [\varphi (Z_x) \varphi
  (Z_y)]  + \sigma_b^2 \big) \Delta (x_i)_{t_{m_i}}^k \Delta (x_j)_{t_{m_j}}^k
\end{eqnarray*}
which is exactly what Equation \ref{eqn:hom-discrete-kernel} states. 
Then note how 
\[
\Sigma^M (S^{x_i}_{m_i}, S^{x_j}_{0}) = \Sigma^M (S^{x_i}_{m_i - 1}, S^{x_j}_{0}) = \dots = \Sigma^M (S^{x_i}_{0}, S^{x_j}_{0}) = \sigma_{S_0}^2
\]

Thus finally we can conclude and write the entries of the matrix $\Tilde{K}^M$ as
\[
    [\Tilde{K}^M]_i^j = K_{\D_M \times \D_M}^{x_i, x_j}(1,1)
\]

\end{proof}

\begin{algorithm}[tbh]
    \caption{$S^{\D_M, N}_1$ as Nestor program}
    \label{Algo:TimeDep}
    \begin{algorithmic}
       \STATE {\bfseries Input:} $S^0: \Gtype(N)$ \hfill  $\triangleright$ \textit{initial value}
       \STATE {\bfseries Input:} $b_1,\dots, b_d: \Gtype(N)$ \hfill $\triangleright$ \textit{biases}
       \STATE {\bfseries Input:} $A_1, \dots, A_d: \Atype(N, N)$ \hfill $\triangleright$ \textit{matrices}
       \STATE {\bfseries Input:} $v: \Gtype(N)$ \hfill $\triangleright$ \textit{readout layer weights}
      \\
      \FOR{$i = 1, \dots, n$}
          \STATE {\it // Compute $S^{\D_M, N}_1 (x_i)$  (here $ S_0^{x_i}$ is to be read as $S_0$)}
          \\
          \FOR{$m = 1,\dots,\norm{\mathcal{D}_M}$}
              \FOR{$k = 1,\dots,d$}
                \STATE $\alpha^i_{m,k} := \varphi(S^{x_i}_{m-1}): \Htype(N)$ \hfill  $\triangleright$ \textit{by Nonlin;}
                \STATE $\beta^i_{m,k} := A_k \alpha^i_{m,k} : \Gtype(N)$ \hfill  $\triangleright$ \textit{by Matmul;}
                \STATE $\gamma^i_{m,k} := \beta^i_{m,k} + b_k  : \Gtype(N)$ \hfill  $\triangleright$ \textit{by LinComb;}
              \ENDFOR
              \STATE $S^{x_i}_{m} := S^{x_i}_{m-1} + \sum_{k=1}^d \gamma^i_{m,k} [(x_i)^k_{t_m} - (x_i)^k_{t_{m-1}}]  : \Gtype(N)$ \hfill  $\triangleright$ \textit{by LinComb;}
          \ENDFOR
          \\
      \ENDFOR
      \\
      \ENSURE $(v^T S_{\norm{\mathcal{D}_M}}^{x_i} / \sqrt{N})_{i=1,\dots,n}$
    \end{algorithmic}
\end{algorithm}


Actually we have proved the even stronger statement that 
\begin{corollary}
    For all $t,s \in \D_M$ one has the following distributional limit
    \[
     \sprod{v^N}{S^{\D_M, N}_{t}(\X)}\sprod{v^N}{S^{\D_M, N}_{s}(\X)}
    \xrightarrow[N \to \infty]{} 
    \mathcal{N}(0,K_{\D_M \times \D_M}^{\X,\X}(t,s))
    \]
\end{corollary}

Moreover with the same proof but considering different partitions for different paths $x,y \in \bX$ in the algorithm we see that:
\begin{proposition}\label{app:prop:Sigma_in_PSD}
    For all $t \in \D$, for all $s \in \D'$ one has the following distributional limit
    \[
    \sprod{v^N}{S^{\D, N}_{t}(x)}\sprod{v^N}{S^{\D', N}_{s}(y)}
    \xrightarrow[N \to \infty]{} 
    \mathcal{N}(0,K_{\D \times \D'}^{x,y}({t,s}))
    \]
    and the matrices $\Sigma_{\D \times \D'}^{x,y}(t,s)$ are always in $PSD_2$.    
\end{proposition}


\subsubsection{Infinite-width-then-depth limit and convergence to $\varphi$-signature kernels}\label{subsubsec:conv-phi-SK}

\begin{definition}
  Fix $\D \assign \{ 0 = t_0 < \cdots < t_{\| \D \|} = 1 \}$
  and $\D' \assign \{ 0 = s_0 < \cdots < s_{\| \D' \|} = 1
  \}$ partitions of $[0, 1]$, the interval where the paths $x, y$ are defined.
  We define
  \[ K_{\D \times \D'}^{x \comma y} : \D \times
     \D' \rightarrow \mathbb{R} \]
  as the map satisfying
  \begin{eqnarray*}
    & K_{\D \times \D'}^{x \comma y} (t_m, s_n) =
    K_{\D \times \D'}^{x \comma y} (t_{m - 1}, s_n) +
    K_{\D \times \D'}^{x \comma y} (t_m, s_{n - 1}) -
    K_{\D \times \D'}^{x \comma y} (t_m, s_{n - 1}) + & \\
    & \sum_{k = 1}^d \left( \sigma_A^2 \mathbb{E}_{\tmscript{(Z_x, Z_y)
    \sim \mathcal{N} \left( 0,  \Sigma^{\tmscript{x, y}}_{\D \times \D'} (t_{m - 1}, s_{n -
    1}) \right)}} [\varphi (Z_x) \varphi (Z_y)] + \sigma_b^2 \right)
    \Delta^{\D} x_{{t_m} }^k \Delta^{\D'} y_{s_n}^k & \\
    & = K_{\D \times \D'}^{x \comma y} (t_{m - 1}, s_n) +
    K_{\D \times \D'}^{x \comma y} (t_m, s_{n - 1}) -
    K_{\D \times \D'}^{x \comma y} (t_m, s_{n - 1}) + & \\
    & + \sum_{k = 1}^d \left( \sigma_A^2 V_{\varphi} \left(
    \Sigma^{{x, y}}_{\D \times \D'} (t_{m - 1}, s_{n -
    1}) \right) + \sigma_b^2 \right) \Delta^{\D} x_{{t_m} }^k
    \Delta^{\D'} y_{s_n}^k & \\
    & = \sigma^2_{S_0} + \sum_{\tmscript{\begin{array}{c}
      0 \leq k_1 < m\\
      0 \leq k_2 < n
    \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 V_{\varphi} \left(
    \Sigma^{\tmscript{ x, y}}_{\D \times \D'} (t_{k_1}, s_{k_2})
    \right) + \sigma_b^2 \right) \Delta^{\D} x_{{t_{k_1 + 1}} }^k
    \Delta^{\D'} y_{s_{k_2 + 1}}^k & 
  \end{eqnarray*}
  where
  \[ \Delta^{\D} x_{{t_m} }^k = (x^k_{t_m} - x^k_{t_{m - 1}}),
     \Delta^{\D'} y_{s_n}^l = (y^l_{s_n} - y^l_{s_{n - 1}}),
     K_{\D \times \D'}^{x, y}(0, s_n) =  K_{\D \times \D'}^{x, y}({t_m, 0}) =
     \sigma^2_{S_0} \]
  and
  \[ \Sigma^{x,y}_{\D \times \D'} (t_m, s_n) =
     \left(\begin{array}{c}
       K_{\D \times \D}^{x, x} (t_m, t_m),  K_{\D \times \D'}^{x, y} (t_m, s_n)\\
       K_{\D \times \D'}^{x, y} (t_m, s_n), K_{\D' \times \D'}^{y, y} (s_n, s_n)
     \end{array}\right) \]
\end{definition}

\begin{definition}
  We extend
  \begin{eqnarray*}
    & K_{\D \times \D'}^{x \comma y} : \D \times
    \D' \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  to
  \begin{eqnarray*}
    & K_{\D \times \D'}^{x \comma y} : [0, 1] \times [0, 1]
    \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  as
  \begin{eqnarray*}
    & K_{\D \times \D'}^{x \comma y} (t, s) =
    K_{\D \times \D'}^{x \comma y} (t_{m - 1}, s_n) +
    K_{\D \times \D'}^{x \comma y} (t_m, s_{n - 1}) -
    K_{\D \times \D'}^{x \comma y} (t_m, s_{n - 1}) & \\
    & + \int^t_{\tau = t_{m - 1}} \int^s_{\sigma = s_{n - 1}}
    \left( \sigma_A^2 V_{\varphi} \left( \Sigma^{\tmscript{x, y}}_{\D \times \D'} (t_{m - 1}, s_{n -
    1}) \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
  \end{eqnarray*}
  where $(t, s) \in [t_m - 1, t_m] \times [s_{n - 1}, s_n]$ (note that this extension is continuous)
  and to
  \begin{eqnarray*}
    & \tilde{K}_{\D \times \D'}^{x \comma y} : [0, 1]
    \times [0, 1] \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  as
  \begin{eqnarray*}
    \tilde{K}_{\D \times \D'}^{x \comma y} (t, s) & = &
    \left\{\begin{array}{l}
      K_{\D \times \D'}^{x \comma y} (t_m, s_n) \quad
      \tmop{if} \quad (t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times
      [s_n, s_{n + 1})\\
      K_{\D \times \D'}^{x \comma y} (1, s_n) \quad
      \tmop{if} \quad (t, s) \in \{ 1 \} \times [s_n, s_{n + 1})\\
      K_{\D \times \D'}^{x \comma y} (t_{m}, 1) \quad
      \tmop{if} \quad (t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times \{ 1
      \}\\
      K_{\D \times \D'}^{x \comma y} (1, 1) \quad \tmop{if}
      \quad (t, s) = (1, 1)
    \end{array}\right.
  \end{eqnarray*}
and similarly for $\tilde{\Sigma}^{\tmscript{x, y}}_{\D \times \D'} (t, s)$
\end{definition}

\begin{remark}
  For ease of notation, if clear from the context, we will write 
  \[ K_{t, s} : = K_{\D \times \D'} (t, s) : = K^{x \comma
     y} (t, s) : = K_{\D \times \D'}^{x \comma y} (t, s) \]
  and similarly for $\tilde{K}_{\D \times \D'}^{x \comma y}
  (t, s)$ and the covariance matrices.
\end{remark}

\begin{remark}
  Note then how, for $(t, s) \in [t_m - 1, t_m] \times [s_{n - 1}, s_n]$,
  \begin{eqnarray*}
    & K_{\D \times \D'}^{x \comma y} (t, s) =
    K_{\D \times \D'}^{x \comma y} (t_{m - 1}, s_n) +
    K_{\D \times \D'}^{x \comma y} (t_m, s_{n - 1}) -
    K_{\D \times \D'}^{x \comma y} (t_m, s_{n - 1}) + & \\
    & + \int^t_{\tau = t_{m - 1}} \int^s_{\sigma = s_{n - 1}} \left(
    \sigma_A^2 V_{\varphi} \left( \tilde{\Sigma}^{\tmscript{ x, y}}_{\D \times \D'} (\tau, \sigma)
    \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma & \\
    & = \sigma^2_{S_0} + \int^t_{\tau = 0} \int^s_{\sigma = 0} \left(
    \sigma_A^2 V_{\varphi} \left( \tilde{\Sigma}^{\tmscript{ x, y}}_{\D \times \D'} (\tau, \sigma)
    \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma & 
  \end{eqnarray*}
  
\end{remark}

Our next goal is to prove the following result:

\begin{theorem} \label{simple_conv}
  Fix a sequence $\{\D_M \times \D'_M\}_{M \in \N}$ of partitions of $[0,1]\times [0,1]$ with $| \D_M | \vee | \D'_M | \rightarrow 0$.
  Then we have the following convergence in $(C^0([0,1]\times [0,1]; \R), \norm{\cdot}_{\infty})$
  \[ K_{\D_M \times \D'_M}^{x, y} (t, s) \rightarrow K^{x, y}
     (t, s) \]
  where $K^{x, y} (t, s)$ satisfies
  \begin{equation}\label{eqn:simple-conv-PDE}
   \begin{gathered}
    K^{x, y} (t, s) =  \sigma^2_{S_0} +  \int_{\tau = 0}^t
    \int_{\sigma = 0}^s \left( \sigma_A^2 \mathbb{E}_{(Z_x, Z_y) \sim
    \mathcal{N} (0,  \Sigma^{x, y}(t, s))} [\varphi (Z_x) \varphi (Z_y)] +
    \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma\\
     =  \sigma^2_{S_0} +  \int_{\tau = 0}^t \int_{\sigma =
    0}^s (\sigma_A^2 V_{\varphi} (\Sigma^{x, y}(t, s)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
   \end{gathered}  
  \end{equation}
  with
  \[ \Sigma^{x, y}(t, s) = \left(\begin{array}{c}
       K^{x, x} (t, t), K^{x, y} (t, s)\\
       K^{x, y} (t, s), K^{y, y} (s, s)
     \end{array}\right) \]

    The limit is independent of the chosen sequence and the convergence is, in $x,y$, uniform on bounded sets of $\bX$.
\end{theorem}

The proof will rely on classic arguments used to prove convergence of Euler schemes to CDE solutions (see \cite{FrizVictoir} and \cite{EulerGoursat}).
Our setting is more complex than the ones we found in the literature though, this is due to the presence of two "independent" driving signals and on the unique nature of the driving fields, which not only depend on the "present" but also on "past" and "future". 
This complex dependency structure of the driving fields makes them completely non-local and requires more involved arguments for the solution to be made sense of.

\subsubsection{Preliminary Bounds}

Note that due to their definition as limiting kernels the $\tilde{\Sigma}_{\D \times\D'}^{x \comma y}$ are always PSD as noted in Proposition \ref{app:prop:Sigma_in_PSD}. However we are going to need a more quantitative result, in the form of a uniform membership in some $PSD(R)$, in order to later leverage Lemma \ref{lemma:split_on_PSD_R}.

We first prove such a result for the case $x = y$ and $\D = \D'$, the general case will follow easily.

The first "ingredient" is a uniform, in $x \in \bX$, bound from below of the kernels for $t=s$.

\begin{lemma}
  $\forall x \in \bX. \forall t \in \D. \quad \Tilde{K}_{\D \times \D}^{x, x}
  (t, t) \geq \sigma_{S_0}^2 $\quad for any choiche of $\D$.
\end{lemma}

\begin{proof}
  We have
  \[ K_{\D \times \D}^{x, x} (t_m, t_m) = \sigma^2_{S_0} +
     \sum_{\tmscript{\begin{array}{c}
       0 \leq k_1 < m\\
       0 \leq k_2 < m
     \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 V_{\varphi} \left(
     \Sigma^{\tmscript{x, x}}_{\D \times \D} (t_{k_1}, t_{k_2})
     \right) + \sigma_b^2 \right) \Delta^{\D} x_{{t_{k_1 + 1}} }^k
     \Delta^{\D} x_{t_{k_2 + 1}}^k \]
  and by Tensor Programs we know that
\begin{equation*}
\resizebox{\hsize}{!}{$
\begin{gathered}
\sum_{\tmscript{\begin{array}{c}
       0 \leq k_1 < m\\
       0 \leq k_2 < m
     \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 V_{\varphi} \left(
     \Sigma^{\tmscript{x, x}}_{\D \times \D} (t_{k_1}, t_{k_2})
     \right) + \sigma_b^2 \right) \Delta^{\D} x_{{t_{k_1 + 1}} }^k
     \Delta^{\D} x_{t_{k_2 + 1}}^k = \lim_{N \rightarrow \infty}
     \mathbb{E} \left[ \frac{\langle S_{t_m}^{\D, N} (x) - S^N_0, S_{t_m}^{\D, N} (x) - S^N_0 \rangle}{N} \right] \geq 0 
\end{gathered}
$}
\end{equation*}
  
\end{proof}

The second step is another bound, this time from above, which will be uniform on bounded subsets of $\bX$.

\begin{lemma}
  There is a constant $C_x > 0$ independent of $\D$ such that
  \[ \| {K}_{\D \times \D}^{x \comma x} \|_{\infty,
     [0, 1] \times [0, 1]} \assign \sup\limits_{(t, s) \in [0, 1]^2} |
     {K}_{\D \times \D}^{x \comma x} (t, s) | \leq C_x
  \]
  Moreover $C_x$ only depends on $\norm{x}_{1-var}$ and is increasing in it, thus there is a uniform bound on bounded subsets of $\bX$.
\end{lemma}

\begin{proof}
    Let us prove this result for $\Tilde{\kappa}_{x,x}$ first.
  Wlog $(t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times [s_n, s_{n + 1})$. Remember how
  \begin{eqnarray*}
    \tilde{K}_{\D \times \D}^{x \comma x} (t, s) & = &
    K_{\D \times \D}^{x \comma x} (t_m, s_n)\\
    & = & \sigma^2_{S_0} +  \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma =
    0} \left( \sigma_A^2 V_{\varphi} \left(
    \tilde{\Sigma}^{\tmscript{x, x}}_{\D \times \D} (\tau, \sigma) \right)
    + \sigma_b^2 \right)
    \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
    d\tau d\sigma
  \end{eqnarray*}
  thus
  \begin{eqnarray*}
    | \tilde{K}_{t, s} | & \leq & 
    \sigma^2_{S_0} + 
    \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    | \sigma_A^2 V_{\varphi} (\tilde{\Sigma}_{ \tau, \sigma})| 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma
    + \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    | \sigma_b^2 | 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma \\
    & = & \sigma^2_{S_0} + 
    \sigma_b^2 \norm{x}_{1-var, [0,t_m]}\norm{x}_{1-var, [0,s_n]} +
    \sigma_A^2 \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    |V_{\varphi}(\tilde{\Sigma}_{ \tau, \sigma})|  
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma \\
    & \leq & \sigma^2_{S_0} + 
    \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    \tilde{M} 
    \tmscript{\left(
    1 + \sqrt{\tilde{K}_{\tau, \tau}} \right) \left( 1 +
    \sqrt{\tilde{K}_{\sigma, \sigma}} \right)} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma\\
    & = & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \tilde{M} 
    \tmscript{\left( \int^{t_m}_{\tau = 0} \left( 1 +
    \sqrt{\tilde{K}_{\tau, \tau}} \right) |\Dot{x}_{\tau}| d\tau \right) 
    \left(\int^{s_n}_{\sigma = 0} \left( 1 + \sqrt{\tilde{K}_{\sigma, \sigma}}
    \right)  |\Dot{x}_{\sigma}| d\sigma \right)}
  \end{eqnarray*}
  In particular
  \begin{eqnarray*}
    \tilde{K}_{t, t} = | \tilde{K}_{t, t} | & \leq & \sigma^2_{S_0} +
    \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} + \sigma_A^2 \tilde{M}
    \left| \int^{t_m}_{\tau = 0} \left( 1 +
    \sqrt{\tilde{K}_{\tau, \tau}} \right) |\Dot{x}_{\tau}| d\tau
    \right|^2\\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \tilde{M}  \| x \|_{1 - \tmop{var}, [0, t_m]}
    \tmscript{
    \left( \int^{t_m}_{\tau = 0} \left( 1 + \sqrt{\tilde{K}_{\tau, \tau}}
    \right)^2 |\Dot{x}_{\tau}| d\tau \right)}\\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    2 \sigma_A^2 \tilde{M} \| x \|_{1 - \tmop{var}, [0, 1]} 
    \int^{t_m}_{\tau = 0} (1 + \tilde{K}_{\tau, \tau}) 
    |\Dot{x}_{\tau}| d\tau \\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    2 \sigma_A^2 \tilde{M} \| x \|_{1 - \tmop{var}, [0, 1]}
    \int^t_{\tau = 0} (1 + \tilde{K}_{\tau, \tau}) 
    |\Dot{x}_{\tau}| d\tau
  \end{eqnarray*}
  
  
  and we can use Gronwall Inequality (\cite{FrizVictoir}, Lemma 3.2) to
  obtain
  \begin{eqnarray*}
    1 + \tilde{K}_{t, t} & \leq & (1 + \sigma^2_{S_0} + \sigma_b^2 \| x
    \|^2_{1 - \tmop{var}, [0, 1]}) \exp \{ 2 \sigma_A^2 \tilde{M} \| x \|^2_{1
    - \tmop{var}, [0, 1]} \}
  \end{eqnarray*}
  hence the thesis with
  \begin{eqnarray*}
    \Tilde{C}_x & = & (1 + \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0,
    1]}) {e^{2 \sigma_A^2 \tilde{M} \| x \|^2_{1 - \tmop{var}, [0, 1]}}}  - 1
  \end{eqnarray*}


  In order to extend the bound to $K_{x,x}$ notice that
  \begin{equation*}
      \begin{gathered}
          |K_{\D \times \D}^{x,x}(t,s)| =  |\sigma^2_{S_0} +  \int^{t}_{\tau = 0} \int^{s}_{\sigma =
          0} \left( \sigma_A^2 V_{\varphi} \left(
          \tilde{\Sigma}_{\tmscript{x, x}}^{\D \times \D} (\tau, \sigma) \right)
          + \sigma_b^2 \right)
          \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
          d\tau d\sigma |\\
          \leq \sigma^2_{S_0} +   \left( 2\sigma_A^2 \Tilde{M} (1 + \Tilde{C}_x) + \sigma_b^2 \right)
          \int^{t}_{\tau = 0} \int^{s}_{\sigma = 0} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}| d\tau d\sigma \\
          \leq \sigma^2_{S_0} +   \left( 2\sigma_A^2 \Tilde{M} (1 + \Tilde{C}_x) + \sigma_b^2 \right)
          \norm{x}_{1-var,[0,1]}^2 =: C_x \\
      \end{gathered}
  \end{equation*}
\end{proof}

Thus finally we can conclude, as promised, that

\begin{lemma}
  There is an $R = R_x \in \mathbb{R}$ such that $\tilde{\Sigma}_{\D \times\D}^{x \comma x} \in \tmop{PSD_2} (R)$ for every $\D$.
  Moreover, as before, this $R_x$ only depends on $\norm{x}_{1-var}$ and is increasing in it. 
\end{lemma}

\begin{proof}
  The diagonal elements $\Tilde{K}_{\D \times \D}^{x,x}(t , t)$ are
  bounded above by a common constant $C_x$ and below by $\sigma^2_{S_0}$
  We thus can simply choose $R_x = C_x \vee \sigma^{-2}_{S_0}$.
\end{proof}

We are ready to extend the result to the general case. 

\begin{proposition}\label{prop:bounded_set_bounds}
    Fix a $\alpha > 0$. There exist a constant $C_{\alpha}$ such that for all $x,y \in \bX$ with $\norm{x}_{1-var}, \norm{y}_{1-var} \leq \alpha$ and partitions $\D, \D'$ it holds
    \[
        \sup_{0 \leq t, s \leq 1} \nobracket | \nobracket K_{\D \times \D^{'}}^{x \comma y} (t, s) | \leq C_{\alpha} 
    \]
    Moreover for $R_{\alpha} := C_{\alpha} \vee \sigma^{-2}_{S_0}$ we get 
    \[
        \Tilde{\Sigma}_{\D \times \D'}^{x \comma y} (t, s) \in \tmop{PSD}(R_{\alpha}) 
    \]
\end{proposition}


\begin{proof}
Remember how the maps $\Tilde{\Sigma}_{\D \times \D'}^{x \comma y}$
are $PSD_2$ since they arise as such from Tensor limiting arguments, in particular by positive semidefinitiveness 
and the previous bounds
\begin{eqnarray*}
\nobracket | \nobracket \tilde{K}_{\D \times \D'}^{x
\comma y} (t, s) | \leq \sqrt{\tilde{K}_{\D \times
\D}^{x \comma x} (t, t) \tilde{K}_{\D' \times
\D'}^{y \comma y} (s, s)} \leq \sqrt{\Tilde{C}_x \Tilde{C}_y} \leq \Tilde{C}_x \vee \Tilde{C}_y 
&  & 
\end{eqnarray*}

For $K_{x,y}(t)$ we proceed similarly to before:
\begin{equation*}
      \begin{gathered}
          |K_{\D \times \D'}^{x,y}(t,s)| =  |\sigma^2_{S_0} +  \int^{t}_{\tau = 0} \int^{s}_{\sigma =
          0} \left( \sigma_A^2 V_{\varphi} \left(
          \tilde{\Sigma}^{\tmscript{x, y}}_{\D \times \D'} (\tau, \sigma) \right)
          + \sigma_b^2 \right)
          \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}   
          d\tau d\sigma |\\
          \leq \sigma^2_{S_0} +   \left( 2\sigma_A^2 \Tilde{M} (1 + \Tilde{C}_x \vee \Tilde{C}_y ) + \sigma_b^2 \right)
          \int^{t}_{\tau = 0} \int^{s}_{\sigma = 0} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}| d\tau d\sigma \\
          \leq \sigma^2_{S_0} +   \left( 2\sigma_A^2 \Tilde{M} (1 + \Tilde{C}_x \vee \Tilde{C}_y ) + \sigma_b^2 \right)
          \norm{x}_{1-var,[0,1]}\norm{y}_{1-var,[0,1]} \leq C_{\alpha} \\
      \end{gathered}
  \end{equation*}

The second part follows from the definition of $\tmop{PSD}(R_{\alpha})$.
\end{proof}

\subsubsection{Proof of Theorem \ref{simple_conv}}

\begin{proof} (Theorem \ref{simple_conv})
\vspace{5pt}
  \newline
  \textit{- Roadmap}
  
  The central idea will be proving that, given any sequence $\D_n \times \D'_n$ with $|\D_n| \vee |\D'_n| \downarrow 0$, the maps $\{ K_{\D_n \times \D'_n}^{x, y} \}_{n}$ form a Cauchy sequence in the Banach space $(C^0 ([0, 1] \times [0, 1] ; \mathbb{R}), \| \cdot \|_{\infty})$. By completeness of this space the sequence will admit a limit $K^{x, y}$, which we will prove to be independent from the chosen sequence. Finally we will prove that this limit is the sought after kernel. \cris{Wouldn't a similar argument based on Ascoli-Arzela work too?}

  Note that trivially the set $\{x,y\}$ is bounded in $\bX$, we can thus fix two constants $C_{x,y}, R_{x,y}$ with the properties given in Proposition \ref{prop:bounded_set_bounds}. We will often, for ease of notation, refer to them as $C$ and $R$.

  \textit{- Part I : how close are $K_{\D \times \D'}$ and $\tilde{K}_{\D \times \D'}$ ?}
  
  We have
  \begin{eqnarray*}
    | K_{\D \times \D'}^{x, y} (t, s) -
    \tilde{K}_{\D \times \D'}^{x, y} (t, s) | & = & |
    \nobracket \int^t_{\tau = 0} \int^s_{\sigma = 0} (\sigma_A^2 V_{\varphi}
    (\widetilde{\Sigma }_{\D \times \D'}^{x, y} (\tau,
    \sigma)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma\\
    &  & - \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} (\sigma_A^2 V_{\varphi}
    (\widetilde{\Sigma }_{\D \times \D'}^{ x, y} (\tau,
    \sigma)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma | \nobracket\\
    & = & \left| \int_{\Omega_{t, s}} (\sigma_A^2 V_{\varphi} (\widetilde{\Sigma
    }_{\D \times \D'}^{ x, y} (\tau, \sigma)) + \sigma_b^2)
    \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma \right|
  \end{eqnarray*}
  with
  \[ \Omega_{t, s} \assign [0, t] \times [0, s] \setminus [0, t_m] \times [0,
     s_n] \]
  Note that
  \[ \Omega_{t, s} \subseteq ([t_{m,} t_{m + 1}] \times [0, 1]) \cup ([0, 1]
     \times [s_n, s_{n + 1}]) \]
  thus
  \[ \mathcal{L}^2 (\Omega_{t, s}) \leq | \D | + | \D' |
     \leq 2 (| \D | \vee | \D' |) \]
  hence
  \begin{equation*} \begin{gathered}
    | K_{\D \times \D'}^{x, y} (t, s) -
    \tilde{K}_{\D \times \D'}^{x, y} (t, s) |  \leq 
    \int_{\Omega_{t, s}} | \sigma_A^2 V_{\varphi} (\widetilde{\Sigma }_{\D
    \times \D'}^{ x, y} (\tau, \sigma)) + \sigma_b^2 |  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma
    \\
     \leq  \sigma_A^2 \int_{\Omega_{t, s}} \tilde{M} 
    \tmscript{\left( 1 +
    \sqrt{K_{\D \times \D}^{x, x} (\tau \comma \tau)}
    \right) \left( 1 + \sqrt{K_{\D' \times \D'}^{y, y}
    (\sigma \comma \sigma)} \right)} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma
       + \sigma_b^2 \int_{\Omega_{t, s}} 
       |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
       d\tau d\sigma\\
     \leq  \sigma_A^2 \tilde{M} \left( 1 + \sqrt{C_{x, y}} \right)^2
    \int_{\Omega_{t, s}} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
    d\tau d\sigma 
    + \sigma_b^2
    \int_{\Omega_{t, s}} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|      
    d\tau d\sigma\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) \int_{[0, 1]
    \times [0, 1]} \mathbb{I}_{\Omega_{t, s}} (\tau, \sigma) 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
    d\tau d\sigma\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\int_{[0, 1] \times [0, 1]} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|^2       
    d\tau d\sigma}\\
    \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\int_{[0, 1] \times [0, 1]} 
    |\Dot{x}_{\tau}|^2 |\Dot{y}_{\sigma}|^2       
    d\tau d\sigma}\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}}\\
     \leq  2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\D | \vee | \D' |} 
     \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}}
  \end{gathered} \end{equation*}
  
  In particular as $(| \D | \vee | \D' |) \rightarrow 0$ we
  have
    \begin{equation*} \begin{gathered}
    \sup_{[0, 1] \times [0, 1]} | K_{\D \times \D'}^{x, y}
     (t, s) - \tilde{K}_{\D \times \D'}^{x, y} (t, s) | \leq
     2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)   
     \sqrt{|\D | \vee | \D' |} 
     \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}} \rightarrow 0
     \end{gathered} \end{equation*}
  
  
  Notice that, since we can repeat the argument for $K_{\D \times
  \D}^{x, x}$ and $K_{\D' \times \D'}^{y, y}$, we have
  \begin{equation*}  \begin{gathered}
  \sup_{[0, 1] \times [0, 1]} | \Sigma_{\D \times \D'}^{ 
     x, y} (t, s) - \tilde{\Sigma}_{\D \times \D'}^{  x, y}
     (t, s) |_{\infty} \leq 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) +
     \sigma_b^2) 
     \sqrt{|\D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
  \end{gathered} \end{equation*}

  \textit{- Part II : Cauchy Bounds}
  
  Consider now another partition $\check{\D} \times
  \check{\D}'$, we have
  \begin{equation*}  \begin{gathered}
    | K_{\check{\D} \times \check{\D}'}^{x, y} (t, s) -
    K_{\D \times \D'}^{x, y} (t, s) |  =  \left|
    \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} [V_{\varphi}
    (\tilde{\Sigma}_{\check{\D} \times \check{\D}'}^{  x, y}
    (\tau, \sigma)) - V_{\varphi} (\tilde{\Sigma}_{\D \times \D'}^{
    x, y} (\tau, \sigma))] \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma 
    \right|\\
     \leq  \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} | V_{\varphi}
    (\tilde{\Sigma}_{\check{\D} \times \check{\D}'}^{  x, y}
    (\tau, \sigma)) - V_{\varphi} (\tilde{\Sigma}_{\D \times \D'}^{x, y} (\tau, \sigma)) |  
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} k_R |
    \tilde{\Sigma}_{\check{\D} \times \check{\D}'}^{  x, y}
    (\tau, \sigma) - \tilde{\Sigma}_{\D \times \D'}^{  x, y}
    (\tau, \sigma) |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}_{\check{\D} \times \check{\D}'}({  \tau,
    \sigma}) - \Sigma_{\check{\D} \times \check{\D}'}({ 
    \tau, \sigma}) |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma_{\check{\D} \times \check{\D}'}({  \tau, \sigma})
    - \Sigma_{\D \times \D'}({  \tau, \sigma}) |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma_{\D \times \D'}({  \tau, \sigma}) -
    \tilde{\Sigma}_{\D \times \D'}({  \tau, \sigma})
    |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\check{\D} | \vee | \check{\D}'|}  
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    \int^t_{\tau = 0} \int^s_{\sigma = 0}  
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma_{\check{\D} \times \check{\D}'}({  \tau, \sigma})
    - \Sigma_{\D \times \D'}({  \tau, \sigma}) |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\D | \vee | \D' |}
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
     \int^t_{\tau = 0} \int^s_{\sigma = 0} 
     |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
     (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})
    \\
       + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma =
    0} | \Sigma_{\check{\D} \times \check{\D}'}^{  x, y}
    (\tau, \sigma) - \Sigma_{\D \times \D'}^{  x, y} (\tau,
    \sigma) |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{gathered} \end{equation*}


  \vspace{3pt}
  Assume to be in the case $x=y$, $\D = \D'$, $\check{\D} = \check{\D}'$ and define the following quantity:
  \[
  \Xi_t \assign 
  \sup_{0 \leq \tau, \sigma \leq t} | \Sigma_{\check{\D} \times \check{\D}}^{x,x}({\tau, \sigma}) - \Sigma_{\D \times \D}^{x,x}({\tau, \sigma}) |_{\infty} = 
  \sup_{0 \leq \tau, \sigma \leq t} |K_{\check{\D} \times \check{\D}}^{x,x}({\tau, \sigma}) - K_{\D \times \D}^{x,x}({\tau, \sigma})|
  \]

  One has, from the previous inequality, that
  \begin{eqnarray*}
    \Xi_t &
    \leq & 4 \sigma_A^2 \left( 2 \sigma_A^2 \tilde{M} \left( {1 + C_x} 
    \right) + \sigma_b^2 \right) 
    \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\D} | \vee |\D |}\\
    &  & + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^t_{\sigma =
    0} | \Sigma_{\check{\D} \times \check{\D}}({  \tau,
    \sigma}) - \Sigma_{\D \times \D}({  \tau, \sigma})
    |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{eqnarray*}
  and since
  \begin{eqnarray*}
    & \int^t_{\tau = 0} \int^t_{\sigma = 0} | \Sigma_{\check{\D}
    \times \check{\D}}({  \tau, \sigma}) - \Sigma_{\D \times
    \D}({  \tau, \sigma}) |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma
    \leq \int^t_{\tau = 0} \int^t_{\sigma = 0} \Xi_{\tau \vee
    \sigma} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma & \\
    & = \int^t_{\tau = 0} \int^{\tau}_{\sigma = 0} \Xi_{\tau} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma
    + \int^t_{\tau = 0} \int^t_{\sigma = \tau}
    \Xi_{\sigma} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}| d\tau d\sigma & \\
    & \leq  \int^t_{\tau = 0}  \| x \|_{1 - \tmop{var},
    [0, \tau]} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
    +  \int^t_{\sigma = 0} \int^{\sigma}_{\tau = 0} 
    \Xi_{\sigma} 
    |\Dot{x}_{\tau} | |\Dot{x}_{\sigma} | d\tau d\sigma 
    & \\
    & = \int^t_{\tau = 0}  \| x \|_{1 - \tmop{var},
    [0, \tau]} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
    + \int^t_{\sigma = 0}  \| x \|_{1 - \tmop{var},
    [0, \sigma]} \Xi_{\sigma} |\Dot{x}_{\sigma} | d\sigma  & \\
    & \leq 2 \| x \|_{1 - \tmop{var}, [0, 1]} 
     \int^t_{\tau = 0} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau & 
  \end{eqnarray*}
  we get
  \begin{eqnarray*}
    {\Xi_t}  & \leq & 4 \sigma_A^2 \left( 2 \sigma_A^2 \tilde{M} \left( {1 + C_x} 
    \right) + \sigma_b^2 \right) 
    \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\D} | \vee |\D |}\\
    &  & + 2 \sigma_A^2 k_R \| x \|_{1 - \tmop{var}, [0, 1]} 
    \int^t_{\tau = 0} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
  \end{eqnarray*}
  thus, by Gronwall,
  \[ \Xi_t \leq 4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2)
     \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\D} | \vee |\D |}
      \cdot e^{2 \sigma_A^2 k_R \| x \|_{1 - \tmop{var}, [0, 1]}^2 }
      \]

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \vspace{5pt}
  Coming back to the general case, we can now say that
  
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \Xi^{x, y}_t \assign \sup_{0 \leq \tau, \sigma \leq t} |
    \Sigma_{\check{\D} \times \check{\D}'}({  \tau, \sigma})
    - \Sigma_{\D \times \D'}({  \tau, \sigma}) |_{\infty} \\
    \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})
    (1 +  e^{2 \sigma_A^2 k_R (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]}) })\\
       + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^t_{\sigma =
    0} | \Sigma_{\check{\D} \times \check{\D}'}({  \tau,
    \sigma}) - \Sigma_{\D \times \D'}({  \tau, \sigma})|_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{gathered} $} \end{equation*}
  and since
  \begin{eqnarray*}
    & \int^t_{\tau = 0} \int^t_{\sigma = 0} 
    | \Sigma_{\check{\D} \times \check{\D}'}({  \tau, \sigma}) 
    - \Sigma_{\D \times \D'}({  \tau, \sigma}) |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma 
    \leq \int^t_{\tau = 0} \int^t_{\sigma = 0} {\Xi^{x, y}_{\tau
    \vee \sigma}}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma & \\
    & = \int^t_{\tau = 0} \int^{\tau}_{\sigma = 0} 
    \Xi^{x, y}_{\tau} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma 
    + \int^t_{\tau = 0} \int^t_{\sigma =\tau} 
    \Xi^{x, y}_{\sigma}
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma & \\
    & \leq 
    \int^t_{\tau = 0} \| y \|_{1 - \tmop{var}, [0, \tau]} 
    \Xi^{x, y}_{\tau} |\Dot{x}_{\tau}| d\tau 
    +  \int^t_{\sigma = 0} \int^{\sigma}_{\tau = 0} 
    \Xi^{x, y}_{\sigma} 
    |\Dot{x}_{\tau}| |\Dot{y}_{\sigma}| d\tau  d\sigma  & \\
    & = \int^t_{\tau = 0} \| y \|_{1 - \tmop{var}, [0, \tau]} 
    \Xi^{x, y}_{\tau} |\Dot{x}_{\tau}| d\tau 
    +  \int^t_{\sigma = 0} \| x \|_{1 - \tmop{var}, [0, \sigma]} 
    \Xi^{x,y}_{\sigma} |\Dot{y}_{\sigma}| d\sigma & \\
    & \leq (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1 - \tmop{var},[0, 1]}) 
    \int^t_{\tau = 0} \Xi^{x, y}_{\tau} (|\Dot{x}_{\tau}| +|\Dot{y}_{\tau}|) d\tau  & 
  \end{eqnarray*}
  we get
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \Xi^{x, y}_t  \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})
    (1 +  e^{2 \sigma_A^2 k_R (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]}) })\\
     + 2 \sigma_A^2 k_R (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1
    - \tmop{var}, [0, 1]}) \int^t_{\tau = 0} \Xi^{x, y}_{\tau} (|\Dot{x}_{\tau}| +|\Dot{y}_{\tau}|) d\tau
  \end{gathered} $} \end{equation*}
  thus, by Gronwall,
 \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \Xi_t  \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})
    (1 +  e^{2 \sigma_A^2 k_R (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]}) })\\
     \cdot e^{2 \sigma_A^2 k_R (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \|
    y \|_{1 - \tmop{var}, [0, 1]}) {(\| x \|_{1 - \tmop{var},
    [0, t]} + \| y \|_{1 - \tmop{var}, [0, t]})}}
  \end{gathered} $} \end{equation*}
  hence
  \begin{equation*} \begin{gathered}
     \| K_{\check{\D} \times \check{\D}'}^{x, y} (t, s) -
    K_{\D \times \D'}^{x, y} (t, s) \|_{\infty, [0, 1]^2} \leq
    \\
    4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    \norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})\\
    \cdot
    (1 +  e^{2 \sigma_A^2 k_R (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]}) })
    \cdot e^{{4 \sigma_A^2 k_R (\| x
    \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1 - \tmop{var}, [0, 1]})}} 
  \end{gathered} \end{equation*}

  \nico{Formatting....}

  \textit{- Part III : Existence and Uniqueness of limit}
  
  Given any sequence of partitions $\{ \D_n \times \D'_n \}$ with $| \D_n | \vee | \D_n' | \rightarrow 0$, due to the bounds we have just proven we have
  \[ 
     \{ K_{\D_n \times \D'_n}^{x , y} \} \text{is a Cauchy sequence in } (C^0 ([0, 1] \times [0, 1] ;
     \mathbb{R}), \| \cdot \|_{\infty}) 
  \]
  and the limit $K^{x, y}$ does not depend on the sequence (i.e. the limit
  exists and is unique). 

  The limit is indeed unique: assume $K^{x, y}$ and $G^{x, y}$ are limits along two different sequences of partitions $\{ \D_n \times \D'_n \}$ and $\{ \mathcal{G}_n \times \mathcal{G}'_n \}$; then the sequence $\{ \mathcal{P}_n \times \mathcal{P}'_n \}$ such that $\mathcal{P}_{2n} \times \mathcal{P}'_{2n} := \D_n \times \D'_n $ and $\mathcal{P}_{2n + 1} \times \mathcal{P}'_{2n + 1} := \mathcal{G}_n \times \mathcal{G}'_n$ is still such that $| \mathcal{P}_n | \vee | \mathcal{P}'_n | \rightarrow 0$ hence the associated kernels have a limit which must be equal to both $K^{x, y}$ and $G^{x, y}$.
  
  Since PSD matrices form a closed set we moreover have that the matrices $\Sigma_{x, y} (t, s)$
  obtained as limits using the previous result are all PSD. We can actually say more: they belong to $\tmop{PSD} (R)$.


  \textit{- Part IV : Limiti Kernel solves Equation (\ref{eqn:simple-conv-PDE})} 

  We can finally conclude by proving that  $K^{x, y}$ is, in fact,  a solution of the PDE:
 \begin{equation*} \begin{gathered}
     \left| K^{x, y} (t, s) - \sigma^2_{S_0} + \int_{\tau = 0}^t
    \int_{\sigma = 0}^s (\sigma_A^2 V_{\varphi} (\Sigma^{x, y}(\tau, \sigma)) +
    \sigma_b^2) 
    \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma   \right|  \\
    \leq  | K^{x, y} (t, s) - K_{\D \times \D'}^{x, y} (t,
    s) | + \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} | V_{\varphi}
    (\tilde{\Sigma}_{\D \times \D'}^{  x, y} (\tau, \sigma))
    - V_{\varphi} (\Sigma^{x, y}(\tau, \sigma)) |  
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma  \\
    \leq  o (1) + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}_{\D \times \D'}^{  x, y} (\tau, \sigma) -
    \Sigma^{x, y}(\tau, \sigma) |_{\infty} 
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma\\
    \leq  o (1) + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}_{\D \times \D'}^{  x, y} (\tau, \sigma) -
    \Sigma_{\D \times \D'}^{  x, y} (\tau, \sigma)
    |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma  \\
     + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma_{\D \times \D'}^{  x, y} (\tau, \sigma) -
    \Sigma^{x, y}(\tau, \sigma) |_{\infty}  
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma \\
    =  o (1) + o (1) + o (1) = o (1)  
   \end{gathered} \end{equation*}
  thus
  \[ \left| K^{x, y} (t, s) - \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma
     = 0}^s (\sigma_A^2 V_{\varphi} (\Sigma^{x, y}(\tau, \sigma)) + \sigma_b^2) 
     \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma\right| = 0 \]
  i.e
  \[ K^{x, y} (t, s) = \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma = 0}^s
     (\sigma_A^2 V_{\varphi} (\Sigma^{x, y}(\tau, \sigma)) + \sigma_b^2) 
     \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma\]

 \textit{- Part V : Uniformity in $x,y$ on bounded sets} 
 
Note that, once again, the bounds we have just proven only depend on  the norms $\norm{\cdot}_{1-var, [0,1]}$ and $\norm{\cdot}_{\bX}$ of the paths,and they do so in an increasing manner. 
Since $\norm{\cdot}_{1-var, [0,1]} \leq \norm{\cdot}_{\bX}$ this means that we have uniform convergence rates on bounded sets on $\bX$.
\end{proof}

\begin{remark}
    We could have stated this result for $x \in W^{1,1}([0,1];\R^d)$ thus requiring the derivative to only be in $L^1$, this is done in an analogous way to the proof of Theorem (\ref{thm:main-inhom-Kernels}). The cost to pay for the decreased regularity of the driving path is the loss of uniform convergence bounds.
\end{remark}

\begin{remark}
    Being careful one could maintain uniform bounds, at the cost of slower convergence, and state the result for $x \in W^{1,1+\epsilon}([0,1];\R^d)$ for any $\epsilon > 0$. More specifically the bound would be proportional to $|\D|^{\frac{\epsilon}{1+\epsilon}}$.
\end{remark}


\vspace{15pt}
\begin{proposition}[Uniqueness]\label{prop:hom_uniqueness}
    Under the previous assumptions on the activation function, fix $x,y \in \bX$. 
    Then any two triples $K({t,s}) := (K^{x,x}({t, s}),K^{x,y}({t, s}),K^{y,y}({t, s}))$ and $G({t,s}) :=(G^{x, x}(t,s),G^{x, y}(t,s),G^{y, y}(t,s))$ defined on $[0,1] \times [0,1]$,satisfying Equation (\ref{eqn:simple-conv-PDE}) and such that $K^{x,x}({t, t}),K^{y,y}({t, t}),G^{x,x}({t, t}),G^{y,y}({t, t})>0$ for all $t \in [0,1]$ must be equal. 
\end{proposition}
\begin{proof}
    We will write $|K|_{\infty} := |K^{x,x}|\vee|K^{x,y}|\vee|K^{y,y}|$.
    To satisfy equation (\ref{eqn:simple-conv-PDE}) the associated covariance matrices $\Sigma_K({\tau, \sigma}), \Sigma_G({\tau, \sigma})$ must be always $PSD_2$.
    Using the assumed bound from below the one from above given by continuity we can assume that they uniformly in time are contained in some $PSD_2(\Bar{R})$. This true for all choices $(x,x),(x,y),(y,y)$.
    
    \begin{equation*} \begin{gathered}
        |K^{x,y}({t, s}) - G^{x,y}({t, s})| = |\int_{\tau = 0}^t \int_{\sigma = 0}^s
     \sigma_A^2 (V_{\varphi} (\Sigma_K^{x,y}({\tau, \sigma})) - V_{\varphi} (\Sigma_G^{x,y}({\tau, \sigma}))) 
     \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}  d\tau d\sigma| \leq 
     \\
     \int_{\tau = 0}^t \int_{\sigma = 0}^s \sigma_A^2 
     |V_{\varphi} (\Sigma_K^{x,y}({\tau, \sigma})) - V_{\varphi} (\Sigma_G^{x,y}({\tau, \sigma}))|
     | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|  d\tau d\sigma \leq
     \\
     \int_{\tau = 0}^t \int_{\sigma = 0}^s \sigma_A^2 
     k_{\Bar{R}}|\Sigma_K^{x,y}({\tau, \sigma}) - \Sigma_G^{x,y}({\tau, \sigma})|_{\infty}
     | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|  d\tau d\sigma \leq
     \\
      \sigma_A^2 k_{\Bar{R}} \int_{\tau = 0}^t \int_{\sigma = 0}^s
    (\sup_{0\leq t_1, s_1 \leq \tau \vee \sigma }|K(t_1, s_1) - G(t_1, s_1)|_{\infty})
     | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|  d\tau d\sigma
    \end{gathered} \end{equation*}
    Moreover this holds substituting $(x,y)$ with $(x,x)$ and $(y,y)$.
    
    Let $\Xi_t := \sup_{0\leq t_1, s_1 \leq \tau t }|K({t_1, s_1}) - G({t_1, s_1})|_{\infty})$ then
    \begin{equation*} \begin{gathered}
        |K({t, s}) - G({t, s})|_{\infty} \leq \sigma_A^2 k_{\Bar{R}}
     \int_{\tau = 0}^t \int_{\sigma = 0}^s  \Xi_{\tau \vee \sigma}
     | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|  d\tau d\sigma \leq 
     \int_{\tau = 0}^t \int_{\sigma = 0}^s  \Xi_{\tau \vee \sigma}
     |\Dot{x}_{\tau}||\Dot{y}_{\sigma}|  d\tau d\sigma
    \end{gathered} \end{equation*}
    thus
    \begin{equation*} \begin{gathered}
        \Xi_t \leq
     \int_{\tau = 0}^t \int_{\sigma = 0}^t  \Xi_{\tau \vee \sigma}
     |\Dot{x}_{\tau}||\Dot{y}_{\sigma}|  d\tau d\sigma \leq
     \\
     \int_{\tau = 0}^t \int_{\sigma = 0}^\tau  \Xi_{\tau}
     |\Dot{x}_{\tau}||\Dot{y}_{\sigma}|  d\tau d\sigma +
     \int_{\tau = 0}^t \int_{\sigma = \tau}^t  \Xi_{\sigma}
     |\Dot{x}_{\tau}||\Dot{y}_{\sigma}|  d\tau d\sigma \leq
     \\
     \norm{y}_{1-var, [0,1]} \int_{\tau = 0}^t  \Xi_{\tau}
     |\Dot{x}_{\tau}|d\tau +
     \norm{x}_{1-var, [0,1]} \int_{\sigma = 0}^t  \Xi_{\sigma}
     |\Dot{y}_{\sigma}|  d\sigma \leq
     \\
     (\norm{x}_{1-var, [0,1]} \vee \norm{y}_{1-var, [0,1]}) \int_{\tau = 0}^t  \Xi_{\tau}
     (|\Dot{x}_{\tau}| + |\Dot{y}_{\tau}| ) d\tau 
    \end{gathered} \end{equation*}

    By Gronwall we finally conclude that $\Xi_t = 0$ for all $t$, which concludes the proof.z
\end{proof}



\subsubsection{Proof of Theorem \ref{thm:phi-SigKer}}

It is finally time to prove the main result of the paper, which we restate below for the reader's convenience.

Fix partitions $\{\D_M\}_{M \in \N}$ of $[0,1]$ with $|\D_M| \downarrow 0$.
Write $\psi^{\D_M, N}_{hom}(\cdot) = \sprod{v^N}{S^{\D_M,N}_1(\cdot)}$ for the ResNet initialized with the \emph{time-homogeneous} scheme.


\begin{theorem}\label{thm:phi-SigKer-appendix}
Let the activation function $\varphi: \R \to \R$ be a linearly bounded, absolutely continuous map with exponentially bounded derivative.
For any subset $\X = \{x_1, \dots, x_n\} \subset \bX$ the following convergence in distribution holds
\[
    \lim_{M \to \infty} \lim_{N \to \infty} \psi^{\D_M, N}_{hom}(\X) 
    =
    \mathcal{N}(0,K^{hom}_{\varphi}(\X, \X))
\]
where the map $K^{hom}_{\varphi} : \bX \times \bX \to \R$ is given by the unique final values $K_{\varphi}^{x,y}(1, 1)$ of the following integro-differential equation
\begin{equation}\label{eqn:hom_kernel-appendix}
\begin{gathered}
      K_{\varphi}^{x, y}(t, s) =  \sigma_{S_0 }^2  +  
      \int_{\tau = 0}^{t} \int_{\sigma = 0}^{s} 
      \Big[ 
      \sigma_A^2 \mathbb{E}_{Z \sim \mathcal{N} (0, {\Sigma}^{x, y}_{\tau, \sigma})} 
      [ \varphi(Z_1) \varphi(Z_2) ] 
      + 
      \sigma_b^2 
      \Big] 
     \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
\end{gathered}
\end{equation}

with 
\[ 
    {\Sigma}^{x, y}_{t,s} = 
     \left(\begin{array}{c}
       K_{\varphi}^{x, x}(t, t), K_{\varphi}^{x, y}(t, s)\\
       K_{\varphi}^{x, y}(t, s), K_{\varphi}^{y, y}(s, s)
     \end{array}\right) 
\]
\end{theorem}

\begin{proof}
    The proof is now just a matter of combining Theorem \ref{thm:discrete-phi-SigKer} and Theorem \ref{simple_conv}.

    Under our hypotheses Theorem \ref{thm:discrete-phi-SigKer} tells us that, for any subset $\X = \{x_1, \dots, x_n\} \subset \bX$, we have in distribution
\[
    \lim_{N \to \infty} \psi^{\D_M, N}_{hom}(\X) 
    =
    \mathcal{N}(0,K_{\D_M \times \D_M}(\X, \X))
\]
thus to conclude we just have to prove that, still in distribution, it holds
\[
    \lim_{M \to \infty} \mathcal{N}(0,K_{\D_M \times \D_M}(\X, \X))
    =
    \mathcal{N}(0,K^{hom}_{\varphi}(\X, \X))
\]
or, equivalently, that in $R^{n\times n}$ it holds $\lim_{M \to \infty} K_{\D_M \times \D_M}(\X, \X) = K^{hom}_{\varphi}(\X, \X)$.

This last needed limit follows from Theorem \ref{simple_conv} with the sequence $\{\D_M \times \D_M\}_{M \in \N}$.
The uniqueness follows from Proposition \ref{prop:hom_uniqueness}.
\end{proof}


Like in the inhomogeneous case we can explicitly write the Kernel for the simplest case:
\begin{corollary}
    If $\sigma = id$, then 
    \begin{equation}\label{eqn:app_hom_id_case}
    K_{id}^{x, y} (t, s) = \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big) SigKer^{\sigma_A x,\sigma_A y}(t,s) - \frac{\sigma_b^2}{\sigma_A^2}
    \end{equation}
\end{corollary}

\begin{proof}
    We readily see that
    \begin{equation}
    \begin{gathered}
         K_{id}^{x, y} (t, s) =  \sigma_{S_0 }^2  +  
          \int_{\tau = 0}^{t} \int_{\sigma = 0}^{s} 
          \Big[ 
          \sigma_A^2 K_{id}^{x, y} (\tau, \sigma)
          + 
          \sigma_b^2 
          \Big] 
         \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
    \end{gathered}
    \end{equation}

    By substituting (\ref{eqn:app_hom_id_case}) for $K_{id}^{x, y} (\tau, \sigma)$ in the integral and using \cite{salvi2021signature}[Theorem 2.5]
    \footnote{\nico{Actually this is for $C^1$ paths...}} 
    we have
    \begin{equation}
    \begin{gathered}
          \sigma_{S_0 }^2  +  
          \int_{\tau = 0}^{t} \int_{\sigma = 0}^{s} 
          \Big[ 
          \sigma_A^2 
          \big\{ \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big) SigKer^{\sigma_A x,\sigma_A y}({\tau,\sigma}) - \frac{\sigma_b^2}{\sigma_A^2} \big\}
          + 
          \sigma_b^2 
          \Big] 
         \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma = 
         \\
         \sigma_{S_0 }^2  +  
          \int_{\tau = 0}^{t} \int_{\sigma = 0}^{s} 
          \sigma_A^2 
           \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big) SigKer^{\sigma_A x,\sigma_A y}({\tau,\sigma}) 
         \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma = 
         \\
         \sigma_{S_0 }^2  +  \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)
          \int_{\tau = 0}^{t} \int_{\sigma = 0}^{s}  
            SigKer^{\sigma_A x,\sigma_A y}({\tau,\sigma}) 
         \sprod{\sigma_A\Dot{x}_{\tau}}{ \sigma_A\Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma = 
         \\
         \sigma_{S_0 }^2  +  \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)
          ( SigKer^{\sigma_A x,\sigma_A y}({t,s}) - 1) = 
          \\
          \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)
           SigKer^{\sigma_A x,\sigma_A y}({t,s})
          - \frac{\sigma_b^2}{\sigma_A^2}
    \end{gathered}
    \end{equation}
    which means, by {uniqueness of solutions} (Proposition \ref{prop:hom_uniqueness}), that the thesis holds.
\end{proof}

\begin{remark}
    A proof similar to that given in the inhomogeneous case for $\varphi = ReLU$ does not work now since the covariance matrix is not, in general, degenerate for $x=y$ as in that case.
\end{remark}

\begin{lemma}\label{app:lemma:hom_simpler_form}
For all choices $(\sigma_{Y_0}, \sigma_A, \sigma_b)$ and for all $\varphi$ as in Theorem \ref{thm:main-inhom-Kernels} we have, with abuse of notation and the obvious meaning, that
\[
    K_{\varphi}^{x,y}(t,s; \sigma_{Y_0}, \sigma_A, \sigma_b) = 
    K_{\varphi}^{\sigma_A x, \sigma_A y}(t,s; \sigma_{Y_0}, 1, \sigma_b \sigma_A^{-1})
\]
\end{lemma}
\begin{proof}
    Follow the exact same steps and arguments of \ref{app:lemma:ingom_simpler_form}.
\end{proof}

\subsection{The Infinite-Depth-then-Width limit}

\subsubsection{Going to Continuous Time}

\begin{proposition}
    Assume the activation function $\varphi$ to be Lipschitz. 
    Let $\rho_M(t) := \sup \{ s \in \D_M : s \leq t\}$ and $x \in \bX$.
    Then the process $Xs^{\D_M,N}_t(x) := S^{\D_M,N}_{\rho_M(t)}(x)$ converges uniformly, as $M \to \infty$, to the solution of the following controlled differential equation
    \begin{equation}
    \begin{gathered}
        S^{N}_t(x) = S_0 + \sum_{k=1}^d \int_0^t \big( A_k [ \varphi(S^{N}_{\tau}(x)) ] + b_k \big) dx_{\tau}^k
    \end{gathered}
    \end{equation}
    where $A_k \in \R^{N \times N}$ and $b_k \in \R^N$ are sampled according to the time-inhomogeneous scheme and for all $M$, given $N$. 
\end{proposition}

\begin{proof}
    The system has unique solution by \cite{FrizVictoir}[Theorems 3.7, 3.8] with 
    \[
        V_i(x) = A_i \varphi(x) + b_k
    \]
    noting that these are Lipschitz since composition of Lipschitz and linearly bounded.
    To conclude note that $S^{\D_M, N}$ is the Euler discretization on $\D_M$ which converges to the solution by the proofs of \cite{FrizVictoir}[Theorems 3.4, 3.7] and the usual subsubsequence argument.
\end{proof}

\begin{remark}
    Actually the same proof applies when the driving path $x$ is taken to be only continuous and of bounded variation \emph{i.e.} $x \in W^{1,1}([0,1];\R^d)$.
\end{remark}


\begin{definition}[Randomized Signatures]
    We call \emph{Randomized Signatures} the solutions to 
    \[
    S^{N}_t(x) = S_0 + \sum_{k=1}^d \int_0^t \big( A_k [ \varphi(S^{N}_{\tau}(x)) ] + b_k \big) dx_{\tau}^k
    \]
\end{definition}

These are the same objects defined in \cite{cuchiero2021expressive}.


\subsubsection{The Linear Case}

\begin{theorem}\label{thm:app_sig_id}
In the case $\varphi = id$ 
\[
    \frac{1}{N}\sprod{S^{id}_t(\X)}{S^{id}_s(\X)}_{\R^N} 
    \xrightarrow[N \to \infty]{\mathbb{L}^2}
    K_{id}^{\X,\X}(t,s)
\]
moreover the convergence is of order $\mathcal{O}(\frac{1}{N})$
\end{theorem}

\begin{proof}
    This is proved in Appendix \ref{app:conv_sigKer}.
\end{proof}

\input{conv_sigker_id.tex}

\newpage
\section{Experiments}

\subsection{Commutativity Conjecture: Experimental Evidence} \label{app:commut_conjecture}

Randomized Signatures have been seen as lower dimensional approximations of the Signature. 

This is indeed true for the linear case in which the activation function is the identity, as we proved in Theorem \ref{thm:sig_id}. 

We however believe that this is not the case in the general setting and conjecture that the limits in Theorem \ref{thm:phi-SigKer} can be exchanged.
In other words we conjecture that in the infinite width limit $\varphi$-RandomizedSignatures converge, in the sense of Proposition \ref{prop:hom-inf-D-W-limit}, to the corresponding $\varphi$-SignatureKernel.

In this section we show the empirical evidence we have to substantiate our claims. All the experiments are reproducible with the python code found at \nico{LINK ANONYMOUS REPO}.

We consider to be in the 
infinite width case since we compute the solutions to the Randomized Signature CDE via differential equation solvers \tocite.

\begin{figure}[h]
    \includegraphics[width=.5\textwidth]{Pictures/Hidden_50.png}\hfill
    \includegraphics[width=.5\textwidth]{Pictures/Hidden_100.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=.5\textwidth]{Pictures/Hidden_150.png}\hfill
    \includegraphics[width=.5\textwidth]{Pictures/Hidden_200.png}\hfill
    \caption{Histograms of $700$ independent realizations of $\sprod{\psi}{S_1(y)}_{\R^N}$ for \emph{ReLU}-RandomizedSignatures $S(y)$ at different values of the hidden dimension parameter $N \in \{50, 100, 250, 200\}$.
    The input path is fixed to be $y(t) := cos(15t) + 3e^t$.
    Gaussian density estimate and Kernel density estimates are shown.}
    \label{fig:conv_ReLU_vs_Id}
\end{figure}


==> B-Architecture.tex <==

\section{Architecture 1}

\begin{algorithm}[h!tb]
    \caption{rSig as Nestor program on Input Path $x$}
    \label{tp:MLP}
    \begin{algorithmic}
      \Require $S_0: \Gtype(n)$ \Comment{initial value}
      \Require $b_1,\dots, b_d: \Gtype(n)$ \Comment{biases}
      \Require $A_1, \dots, A_d: \Atype(n, n)$ \Comment{matrices}
      \Require $v: \Gtype(n)$ \Comment{readout layer weights}
      \\
      \For{$t = 1,\dots,m_x$}
          \For{$k = 1,\dots,d$}
            \State $\alpha^t_k := \sigma(S_{t-1}): \Htype(n)$ \Comment{by Nonlin;}
            \State $\beta^t_k := A_k \alpha^t_k : \Gtype(n)$ \Comment{by Matmul;}
            \State $\gamma^t_k := \beta^t_k + b_k  : \Gtype(n)$ \Comment{by LinComb;}
          \EndFor
          \State $S^x_{t} := S^x_{t-1} + \sum_{k=1}^d \gamma^t_k \Delta x^k_t  : \Gtype(n)$ \Comment{by LinComb;}
      \EndFor
     \\
      \Ensure $\frac{1}{\sqrt{n}}v^T S_{m_x}$
    \end{algorithmic}
\end{algorithm}


==> C-rSignatures.tex <==
\section{Signatures and rSignatures}



\subsection{Signatures}


\subsection{Randomized Signatures}

 Signature is difficult to work with due to its costly computation and infinite-dimensional nature.  \\
 A promising solution to these problems might come from representation theory (\cite{cuchiero2021expressive}): 
represent $\mathbb{A}_d$ as a family of vector fields and then consider the solution to the PDE representing 
\[
    dS(\omega)_t = \sum_{i=1}^d \big( S(\omega)_t \otimes e_i \big) \hspace*{3pt} d\omega^i_t
\]
i.e. the object corresponding to the signature.

\subsubsection{Definition and Properties}

Fix $\X := \{ \omega \in BV_c([0,1]; \R^d) : \omega(0) = 0\}$. Let $\mathbb{L}$ be the lie algebra of vector 
fields on $\mathbb{A}_d$ generated by $\{ a \to a\otimes e_i \}_{i=1}^d$.

\begin{definition}
A \emph{Stochastic Driving Basis} is the collection of a probability space
$(\Theta,\mathcal{A},\mu)$, a set $\{S^\theta_0\}_{\theta \in \Theta} \subseteq \R^n$ 
and a family of vector fields 
$\{ V_i^{\theta}\}_{\theta \in \Theta}^{i \in 1:d} \subseteq C^{\infty}(\R^n;\R^n)$
chosen such that the maps 
$$\Phi^{\theta} : \mathbb{L} \to C^{\infty}(\R^n;\R^n) \text{  s.t.  } \{ a \to a\otimes e_i \} \mapsto V^{\theta}_i$$
are \emph{faithful} $\mu$-a.s
\emph{i.e.} $\Phi^{\theta}$ is $\mu$-a.s. an injective Lie algebra homomorphism.

\end{definition}

Note that \emph{faithfulness} of $\Phi^{\theta}$ corresponds to asking all non-trivial Lie polynomials
in the vector fields $V_i^{\theta}$ to be non-zero. 



This may bee too complicated to prove, a partial result which is more attainable is that of 
having all non-trivial Lie polynomials in the $V_i^{\theta}$ \emph{up to order N} to be non-zero.

This motivates the following definition:
\begin{definition}
    A \emph{Stochastic Driving Basis of degree N} is the collection of a probability space
    $(\Theta,\mathcal{A},\mu)$, a set $\{S^\theta_0\}_{\theta \in \Theta} \subseteq \R^n$ 
    and a family of vector fields 
    $\{ V_i^{\theta}\}_{\theta \in \Theta}^{i \in 1:d} \subseteq C^{\infty}(\R^n;\R^n)$
    chosen such that $\mu$-a.s. all non-trivial Lie polynomials in the $V_i^{\theta}$ 
    \emph{up to order N} are non-zero.
    
    If $\Theta$ is endowed with a topology and $\mathcal{A}$ is its Borel $\sigma$-field 
    then we speak of \emph{Borel Driving Basis of degree N}.
\end{definition}

The bigger the degree $N$ the better we can mimic the non-linear dynamic of Signature,
in applications a big enough $N$ should therefore suffice in order to compute expressive enough feature maps.
    


\vspace*{5pt}
\begin{definition}[Randomized Signature]

The \emph{Randomized Signature} associated to a Stochastic Driving Basis %of any degree
is the functional $S: \X \times \Theta \to C^0([0,1];\R^n)$ mapping 
$(\omega,\theta)$ to the solution $S^{\omega,\theta}$ of 

\begin{equation}\label{RandSig}
    \begin{cases}
        dS^{\omega,\theta}_s = \sum_{i=1}^d V_i^{\theta}(S^{\omega,\theta}_s) \hspace*{3pt} d\omega_s^i\\
        S^{\omega,\theta}_0 = S^{\theta}_0
    \end{cases}
\end{equation}

\end{definition}    


\vspace*{10pt}
For a quantitative study of the expressive power of these object see \textcolor{red}{[Cite Muça Cirone - Teichann]}. 
Intuitively the bigger the dimension of the Randomized Signature and the more nonlinear the map $\sigma$ is, the more expressive these objects turn out to be.


==> conv_sigker_id.tex <==
\newpage
\section{Convergence to the SigKer}\label{app:conv_sigKer}


In this last section we prove Theorem \ref{thm:app_sig_id}.
between \emph{Randomized Signature Kernels} and the original \emph{Signature Kernel}.

We are going to consider words $I = (i_1, \cdots, i_k) \in \mathcal{A}_d^k$ in the alphabet $\mathcal{A}_d := \{1,\dots, d\}$; the space of all words will be denoted by $\mathbb{W}_d$, the length of a word by $|I| = k$ and the sum of its elements by $\norm{I} = \sum_{m=1}^k i_m$.

\vspace*{5pt}
Intuitively as the reservoir dimension increases 
randomized signature has more freedom to accurately mimic the dynamic behavior 
of Signature. The dynamics of Signature make it continuously move 
into orthogonal directions, the presence of more dimensions might allow its randomized counterpart to 
act similarly, at least on small time frames. 

\vspace*{5pt}
It is then natural to conjecture that Randomized Signature Kernels
behave like Signature Kernels when the reservoir dimension tends to infinity.


\vspace{5pt}
Recall we consider randomized Signatures of the type 
\[
   S^{N}_t(x) = S_0 + \sum_{k=1}^d \int_0^t \big( A_k S^{N}_{\tau}(x)  + b_k \big) dx_{\tau}^k
\]
where $x \in \bX$ and 
\[
    [A_{k}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{\sigma_{A}^2}{N}) 
    \hspace{15pt}
    [S_0]_{\alpha}\sim \mathcal{N}(0,\sigma_{S_0}^2)
    \hspace{15pt}
    [b_{k}]_{\alpha} \sim \mathcal{N}(0,\sigma_b^2)
\]

\vspace{10pt}
Our goal is that of proving the following result:
\begin{theorem}
    In the assumptions stated above
    \[
        \lim_{N \to \infty} \E\Big[
        \frac{1}{N}\langle S^N_t(x), S^N_s(y) \rangle_{\R^N}\Big] = 
        \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)  SigKer^{\sigma_A x,\sigma_A y}({t,s}) - \frac{\sigma_b^2}{\sigma_A^2}
    \]
    and the variance around the limit is of order $O(\frac{1}{N})$.
\end{theorem}


\vspace{15pt}
We know, see \cite{10.1214/EJP.v17-2136}[Remark 2.10], that it is possible to write a closed form for $S^N_t(x)$
which \emph{decouples} the effects of the vector fields 
and those of the driving control using the \emph{Signature}:

\begin{equation}\label{eqn:decoupling}
    S^N_t(x) = \sum_{I \in \mathbb{W}_d} V_{I}(S^N_0) \hspace{3pt} Sig^{I}_{0,t}(x)
\end{equation}


where $\mathbb{W}_d$ is the set of words in the alphabet $\{1,\dots,d\}$ and if $I = (i_1,\dots,i_k)$ then $[V_I(z)]_{\alpha} := V_{i_1} \cdots V_{i_k} \langle e_{\alpha}, \cdot \rangle (z)$ with $V_i(z) := A_i z + b_i$ and $Vf(z) = := df_z [V_j(z)]$ for $f \in C^{\infty}(\R^N; \R)$.
Notice that $V_{I}(S^N_0) \in \R^N$ and $Sig^{I}_{0,t}(x) \in \R$.

\vspace{5pt}
In fact the "Taylor expansion" with respect of the signature of $f(S^N_t(x))$ for $f \in C^{\infty}(\R^N; \R)$ is 

\[
    f(S^N_t(x)) = \sum_{I \in \mathbb{W}_d} V_{I}f(S^N_0) \hspace{3pt} Sig^{I}_{0,t}(x)
\]
where, with $I$ as above, $V_If(x) := V_{i_1} ( V_{i_2} \cdots  ( V_{i_k} f) \cdots )(x)$ with $$V_jf(x) := df_x [V_j(x)]$$

\vspace{15pt}

From Equation \ref{eqn:decoupling} we also get
\begin{align*}
    \langle S^N_t(x), S^N_s(y) \rangle_{\R^N} 
    &= \sum_{I \in \mathbb{W}_d} \sum_{J \in \mathbb{W}_d} 
    \langle V_{I}f(S^N_0) , V_{J}f(S^N_0)  \rangle_{\R^N} \hspace{3pt} Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y) 
\end{align*}

where $y$ is another control.
If we could exchange expectation with the series we would thus get

\begin{equation*}
    \mathbb{E}[\langle S^N_t(x), S^N_s(y) \rangle_{\R^N}]
    =
    \sum_{I \in \mathbb{W}_d} \sum_{J \in \mathbb{W}_d} 
    \E [ \langle V_{I}f(S^N_0) , V_{J}f(S^N_0)  \rangle_{\R^N} ]
    \hspace{3pt} Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)
\end{equation*}


Thus we have to study the expectations 
$\E [ \langle V_{I}f(S^N_0) , V_{J}f(S^N_0)  \rangle_{\R^N} ]$.

Note that if $I = ()$, the empty word, then $V_{I}f(S^N_0) = S^N_0$.

\vspace{20pt}
The most important result which will make our plan succeed is the following classical theorem:

\begin{theorem}[Isserlis]
 Let $(X_1, \dots, X_N)$ be a zero mean multivariate normal vector, then
 \[
    \E[X_1 \cdots X_N] = \sum_{p \in P^2_n} \prod_{\{i,j\} \in p} \E[X_i X_j]
 \]
 where the sum is over all distinct ways of partitioning $\{1,\ldots,N\}$ into pairs $\{i,j\}$, and the product is over the pairs contained in $p$.
\end{theorem}

\subsection{The coefficients}

\begin{proposition}\label{thm:randomized_sig_kernel}
 Assume $I,J \in \mathbb{W}_d$ such that $|I|+|J| > 0$.
 In the hypotheses stated above 
 \[
    \E [ \langle V_{I}f(S^N_0) , V_{J}f(S^N_0)  \rangle_{\R^N} ]
    =
    \delta^I_J + O(\frac{1}{N})
 \]
if the bias terms $b_i$ are set to $0$. 

While if the biases are sampled from the aforementioned normal distribution
\[
    \E [ \langle V_{I}f(S^N_0) , V_{J}f(S^N_0)  \rangle_{\R^N} ]
    =
    2\delta^I_J + O(\frac{1}{N})
\]

 
\end{proposition}

\begin{proof}

    Let us first consider the case $\sigma_b=0$.
    
    Taking $f(z) = \langle v, z \rangle_{\R^N}$ for some $v \in \R^N$ and $V_j(z) := A_jz $ we get
    \[
        V_jf(x) := d(\langle v, \cdot \rangle_{\R^N})_x [A_jx] = v^TA_jx = \langle A_j^Tv, x \rangle_{\R^N}
    \]
    hence by induction 
    \[
        V_If(x) = \langle A_{i_1}^T \cdots A_{i_k}^T v, x \rangle_{\R^N}
        = \langle v, A_{i_k} \cdots A_{i_1} x \rangle_{\R^N}
    \]
    and in our notation
    \[
    V_I(x) = A_Ix = A_{i_k} \cdots A_{i_1}x
    \]
    
    \vspace{5pt}
    We are thus interested in the quantities $\E [ (S^N_0)^T A_I^T A_J S^N_0 ]$.
    
    \vspace{15pt}
    
    Let $\alpha, \beta \in \{1, \dots, N\}$ and given a matrix $M \in \R^{N \times N}$ write $[M]_{\alpha}^{\beta}$ for its component in row $\alpha$ and column $\beta$. Remember how 
    \[
        [M_1 M_2]_{\alpha}^{\beta} = \sum_{\gamma = 1}^N \hspace{3pt} [M_1]_{\alpha}^{\gamma} [M_2]_{\gamma}^{\beta}
    \]
    
    Thus we have 
    \begin{equation*}
        \begin{gathered}
            \E\Big[ (S^N_0)^T A^T_I A_J S^N_0 \Big] 
            = \sum_{n=1}^N\sum_{m=1}^N \E\Big[ [S^N_0]_n [S^N_0]_m [A^T_I A_J]^m_n \Big]
            \\=
            \sum_{n=1}^N\sum_{m=1}^N \E\Big[ [S^N_0]_n [S^N_0]_m \Big] \E\Big[[A^T_I A_J]^m_n \Big]
        \end{gathered}
    \end{equation*}

    
    Moreover, for $I = (i_1, \dots, i_k)$, we obtain
    \begin{align*}
        [A_I]_{\alpha}^{\beta} 
        &= \sum_{\delta_1 = 1}^N \hspace{3pt} [A_{(i_2,\dots,i_{k})}]_{\alpha}^{\delta_1} [A_{i_1}]_{\delta_1}^{\beta}\\
        &= \sum_{\delta_{k-1} = 1}^N \dots \sum_{\delta_1 = 1}^N \hspace{3pt} [A_{i_k}]_{\alpha}^{\delta_{k-1}} [A_{i_{l-1}}]_{\delta_{k-1}}^{\delta_{k-2}} \cdots [A_{i_{2}}]_{\delta_{2}}^{\delta_1}[A_{i_1}]_{\delta_1}^{\beta}\\
        &= \sum_{\bar{\delta} \in \Lambda^{N,k}_{\alpha,\beta}} 
        \prod_{n=1}^k \hspace{3pt} [A_{i_n}]_{\delta_{n}}^{\delta_{n-1}}
    \end{align*}
    
    where $\Lambda^{N,k}_{\alpha,\beta} := \{ (\delta_0, \dots, \delta_{k}) \in \{1,\dots,N\}^{k+1} : \delta_k = \alpha \text{ and } \delta_{0} = \beta\}$. With this notation we can write 
    
    \begin{align*}
        [A_I^T A_J]_{\alpha}^{\beta} 
        &= \sum_{\gamma = 1}^N \hspace{3pt} [A_I^T]_{\alpha}^{\gamma} [A_J]_{\gamma}^{\beta}
        = \sum_{\gamma = 1}^N \hspace{3pt} [A_I]^{\alpha}_{\gamma} [A_J]_{\gamma}^{\beta}\\
        &= \sum_{\gamma = 1}^N \sum_{\bar{\delta} \in \Lambda^{N,|I|}_{\gamma,\alpha}} \sum_{\bar{\epsilon} \in \Lambda^{N,|J|}_{\gamma,\beta}} \prod_{n=1}^{|I|} \prod_{m=1}^{|J|}\hspace{3pt} [A_{i_n}]_{\delta_{n}}^{\delta_{n-1}} [A_{j_m}]_{\epsilon_{m}}^{\epsilon_{m-1}}\\
    \end{align*}
    
    thus 
    \begin{align}
        \E\Big[[A_I^T A_J]_{\alpha}^{\beta} \Big] &= 
        \sum_{\gamma = 1}^N \sum_{\bar{\delta} \in \Lambda^{N,|I|}_{\gamma,\alpha}} \sum_{\bar{\epsilon} \in \Lambda^{N,|J|}_{\gamma,\beta}} \E \Big[ \prod_{n=1}^{|I|} \prod_{m=1}^{|J|}\hspace{3pt} [A_{i_n}]_{\delta_{n}}^{\delta_{n-1}} [A_{j_m}]_{\epsilon_{m}}^{\epsilon_{m-1}} \Big]%\\ 
        %&= \sum_{\gamma = 1}^N \sum_{\bar{\zeta} \in x^{N,|I|,|J|}_{\gamma,(\alpha, \beta)}} \E \Big[ \prod_{o=1}^{|I*J|} \hspace{3pt} [A_{(i*j)_o}]_{\zeta_o}^{\zeta_{o+1}} \Big]
    \end{align}
    
    
    \vspace{5pt}
    The time is ripe for the application of \emph{Isserlis' Theorem}.
    
    
    \vspace{10pt}
    First of all notice how the sum in Isserlis runs over the possible pairings of the index set which in our case is the set of elements of the concatenation 
    $$I*J = (i*j_1, \dots, i*j_{|I|+|J|}) = (i_1, \dots, i_{|I|}, j_1, \dots, j_{|J|})$$ of $I$ and $J$. Then
    
    \begin{equation*}
        \begin{gathered}
            \E\Big[[A_I^T A_J]_{\alpha}^{\beta} \Big] \\ 
        =\sum_{\gamma = 1}^N \sum_{\bar{\delta} \in \Lambda^{N,|I|}_{\gamma,\alpha}} \sum_{\bar{\epsilon} \in \Lambda^{N,|J|}_{\gamma,\beta}} \sum_{p \in P^2_{|I|+|J|}} \prod_{\{a,b\} \in p} \E \Big[[A_{(i*j)_a}]_{(\delta*\epsilon)_{a}}^{(\delta*\epsilon)'_{a}} [A_{(i*j)_b}]_{(\delta*\epsilon)_{b}}^{(\delta*\epsilon)'_{b}} \Big]\\
        = \sum_{p \in P^2_{|I|+|J|}} \sum_{\gamma = 1}^N \sum_{\bar{\delta} \in \Lambda^{N,|I|}_{\gamma,\alpha}} \sum_{\bar{\epsilon} \in \Lambda^{N,|J|}_{\gamma,\beta}} \prod_{\{a,b\} \in p} \E \Big[[A_{(i*j)_a}]_{(\delta*\epsilon)_{a}}^{(\delta*\epsilon)'_{a}} [A_{(i*j)_b}]_{(\delta*\epsilon)_{b}}^{(\delta*\epsilon)'_{b}} \Big]
        \end{gathered}
    \end{equation*}

    where $$(\delta*\epsilon) = (\delta_1,\dots,\delta_{|I|},\epsilon_1,\dots,\epsilon_{|J|})$$
    and  
    $$(\delta*\epsilon)' = (\delta_0,\dots,\delta_{|I|-1},\epsilon_0,\dots,\epsilon_{|J|-1})$$
    
    \vspace{10pt}
    In particular this sum is $0$ by default if $I*J$ has an odd number of elements. This means that
    \[
         \E\Big[[A_I^T A_J]_{\alpha}^{\beta} \Big] = 0
    \]
    whenever $|I| + |J|$ is odd.
    
    Moreover, even if $|I| + |J|$ is even, the pairings must be in such a way that no factor of the product vanishes; since we are working with matrices with independent normal entries this is equivalent to requiring for each $\{a,b\} \in p \in P^2_{|I|+|J|}$ that $(i*j)_a = (i*j)_b$, $(\delta*\epsilon)_{a} = (\delta*\epsilon)_{b}$, and $(\delta*\epsilon)'_{a} = (\delta*\epsilon)'_{b}$. 
    
    \vspace{5pt}
    Evidently then $I*J$ must be at least "pairable" with pairs of identical indices! In this case we will say that $I*J$ is \emph{twinable} and we will get a factor $\sigma_A^2 N^{-1}$ out of every $\E \Big[[A_{(i*j)_a}]_{(\delta*\epsilon)_{a}}^{(\delta*\epsilon)'_{a}} [A_{(i*j)_b}]_{(\delta*\epsilon)_{b}}^{(\delta*\epsilon)'_{b}} \Big]$ thus
    
    \[
        \E\Big[[A_I^T A_J]_{\alpha}^{\beta} \Big] = \Big(\frac{\sigma_A^2}{N}\Big)^{\frac{|I|+|J|}{2}} \Xi(I,J,N,\alpha,\beta)
    \]
    
    where 
    \begin{equation*}
        \begin{gathered}
             \Xi(I,J,N,\alpha,\beta) 
             \\ =
            |\{(p,\gamma,\bar{\delta},\bar{\epsilon}) :  \forall \{a,b\} \in p. \hspace{3pt} \E \Big[[A_{(i*j)_a}]_{(\delta*\epsilon)_{a}}^{(\delta*\epsilon)'_{a}} [A_{(i*j)_b}]_{(\delta*\epsilon)_{b}}^{(\delta*\epsilon)'_{b}} \Big]\neq 0\}|
        \end{gathered}
    \end{equation*}

       
    
    \vspace{10pt}
    Define, given $p \in P^2_{|I|+|J|}$,
    \begin{equation*}
        \begin{gathered}
            \omega(p,I,J,N,\alpha,\beta) 
            \\ = 
            |\{(\gamma,\bar{\delta},\bar{\epsilon}) :  \forall \{a,b\} \in p. \hspace{3pt} \E \Big[[A_{(i*j)_a}]_{(\delta*\epsilon)_{a}}^{(\delta*\epsilon)'_{a}} [A_{(i*j)_b}]_{(\delta*\epsilon)_{b}}^{(\delta*\epsilon)'_{b}} \Big]\neq 0\}|
        \end{gathered}
    \end{equation*}
    
    so that
    \[
    \Xi(I,J,N,\alpha,\beta) = \sum_{p \in P^2_{|I|+|J|}} \omega(p,I,J,N,\alpha,\beta)
    \]
    
    \vspace{10pt}
    First of all notice how
    \[
        \omega(p,I,J,N,\alpha,\beta) \leq N^{\frac{|I|+|J|}{2}}
    \]
    
        in fact considering only the constraints given by $\alpha$ and $\beta$ we have $N^{|I|}$ ways to choose $\bar{\delta} \in \{1,\dots,N\}^{|I|+1}$ and $N^{|J|}$ ways to choose $\bar{\epsilon} \in \{1,\dots,N\}^{|J|+1}$, but since they must come in pairs as dictated by $p$ we actually have $N^{\frac{|I|+|J|}{2}}$ possible choices \emph{i.e.} $N$ per pair.
    
    \vspace{5pt}
    Notice however how we have equality if and only if $I=J$, $\alpha = \beta$ and the pairings are such that $p \ni \{a,b\} = \{a,|I|+a\}$ for $a \in \{1,\dots,|I|\}$
    \emph{i.e.} every element in $I$ is paired to the corresponding one in $J = I$.
    
    The \emph{if} part is easy to see: the full constraints are just
    $\delta_{|I|} = \epsilon_{|I|} = \gamma$, $\delta_a = \epsilon_a$ for every $1 < a \leq |I|$ and
    $\alpha = \delta_{0} = \epsilon_{0} = \beta$ thus there are $$N \times N^{|I| - 1} \times 1 = N^{|I|} = N^\frac{|I|+|J|}{2}$$ choices to make.
    
    The \emph{only if} is more complicated and follows from the constraint $\delta_{|I|} = \epsilon_{|J|}$. Fix $\gamma$ and assume $i_{|I|}$ is not paired with $j_{|J|}$, then the choices for $(\delta*\epsilon)_a = (\delta*\epsilon)_b$ for 2 out of the $\frac{|I|+|J|}{2}$ pairs are constrained to be $\gamma$, all in all we have $N$ choices for $\gamma$ and at most $N^{\frac{|I|+|J|}{2}-2}$ for the other entries, thus at most $N^{\frac{|I|+|J|}{2}-1}$ in total. But then we must require $i_{|I|}$ and $j_{|J|}$ to be paired. The same argument can now be repeated with $i_{|I|-1}$ and $j_{|I|-1}$ since we have established that $\{|I|,|I|+|J|\} \in p$, thus not only $\delta_{|I|} = (\delta*\epsilon)_{|I|} = (\delta*\epsilon)_{|I|+|J|} = \epsilon_{|J|}$ but also $\delta_{|I|-1} = (\delta*\epsilon)'_{|I|} = (\delta*\epsilon)'_{|I|+|J|} = \epsilon_{|J|-1}$. 
    This goes on until, without loss of generality, we run out of elements in $I$.
    If the same happens for $J$ (\emph{i.e.} $|I|=|J|$) we are done since we have proved that $\forall a \in 1, \dots, |I|$ we have $i_a = j_a$ and $\alpha = (\delta*\epsilon)'_{1} = (\delta*\epsilon)'_{|I| + 1} = \beta$.
    Otherwise $|J| \geq 2 + |I|$ and $(j_{|J|-|I|},\dots,j_{1})$ are paired between themselves. 
    But since $\{1,|I|+(|J|-|I|+1)\}\in p$ we have $\alpha = (\delta*\epsilon)'_{1} = (\delta*\epsilon)'_{|I|+(|J|-|I|+1)} = (\delta*\epsilon)_{|I|+(|J|-|I|+1) - 1} = (\delta*\epsilon)_{|I|+(|J|-|I|)} = \epsilon_{|J|-|I|}$. Which means that there is no free choice one of the remaining couples (\emph{i.e.} the one containing $|I|+(|J|-|I|)$ corresponding to $j_{|J|-|I|}$) thus, reasoning just as before, we cut the number of choices of at least a factor $N$.
    
    %Let $a$ be such that $\{a,|I|+|J|\} \in p$, we must have $2|I| < a < |I|+|J|$ and $\beta = (\delta*\epsilon)'_{|I|+|J|} = (\delta*\epsilon)'_{a} = (\delta*\epsilon)_{a+1}$ which means that there is no free choice one of the remaining couples thus, reasoning just as before, we cut the number of choices of at least a factor $N$.
    
    
    \vspace{10pt}
    We have just shown that, given a pairing $p$,
    $$\Big(\frac{\sigma_A^2}{N}\Big)^{\frac{|I|+|J|}{2}} \omega(p,I,J,N,\alpha,\beta) \leq  \\ \Big(\frac{\sigma_A^2}{N}\Big)^{\frac{|I|+|J|}{2}} N^{\frac{|I|+|J|}{2} - 1} = \frac{\sigma_A^{|I|+|J|}}{N} $$
    except when $I=J$, $\alpha = \beta$ and the pairings are such that $p \ni \{a,b\} = \{a,|I|+a\}$ for $a \in \{1,\dots,|I|\}$, in which case
    $$\Big(\frac{\sigma_A^2}{N}\Big)^{\frac{|I|+|J|}{2}} \omega(p,I,J,N,\alpha,\beta) =  \Big(\frac{\sigma_A^2}{N}\Big)^{\frac{|I|+|J|}{2}} N^{\frac{|I|+|J|}{2}} = \sigma_A^{|I|+|J|} $$
    
    This means that 
    \[
        \E\Big[[A_I^T A_J]_{\alpha}^{\beta} \Big] = \Big(\frac{\sigma_A^2}{N}\Big)^{^{\frac{|I|+|J|}{2}}} \hspace{3pt} \Xi(I,J,N,\alpha,\beta) = \sigma_A^{|I|+|J|}  \big[ \delta_{\alpha}^{\beta}\delta_{I}^{J} + \frac{1}{N}\psi(I,J,N,\alpha,\beta) \big]
    \]
    
    where $0 < \psi(I,J,N,\alpha,\beta) \leq (|I|+|J|)!!$ i.e.  $\psi(I,J,N)$ is a positive constant bounded above by the maximal number of pairings (which occur only when $I$ and $J$ are made up of the same one index). Notice how this bound depends only on $|I|$ and $|J|$ and not on $N$!
    
    \vspace{10pt}
    Finally, if $S^N_0$ is normally distributed then

    \begin{equation*}
        \begin{gathered}
            \E\Big[ (S^N_0)^T A^T_I A_J S^N_0 \Big] 
            =
            \sum_{n=1}^N\sum_{m=1}^N \E\Big[ [S^N_0]_n [S^N_0]_m \Big] \E\Big[[A^T_I A_J]^m_n \Big]
            \\=
            \sum_{n=1}^N {\sigma_{S_0}^2} \E\Big[[A^T_I A_J]^n_n \Big] 
            = N \sigma_{S_0}^2\sigma_A^{|I|+|J|} \big[ \delta_I^J + \frac{1}{N}\psi(I,J,N) \big] = N \sigma_{S_0}^2\sigma_A^{|I|+|J|} \big[ \delta_I^J + O(\frac{1}{N}) \big]
        \end{gathered}
    \end{equation*}
    
    with $0 \leq \psi(I,J,N) := \frac{1}{N} \sum_{n=1}^N \psi(I,J,N,n,n) \leq (|I|+|J|)!!$.
    
    \vspace{20pt}
    
    Let us now look at the case with $\sigma_b > 0$.  
    
    Let $V_j(x) := A_jx + b_j$ 
    \vspace{3pt}
    Take $f(x) = \langle v, x \rangle_{\R^N}$ for some $v \in \R^N$. Then 
    \[
        V_jf(x) = d(\langle v, \cdot \rangle_{\R^N})_x [A_jx + b_j] = v^T(A_jx + b_j) = \langle A_j^Tv, x \rangle_{\R^N}
        + \langle v, b_j \rangle_{\R^N}
    \]
    hence by induction 
    \[
        V_If(x) = \langle v, A_{i_k} \cdots A_{i_2} (A_{i_1} x + b_{i_1}) \rangle_{\R^N}
    \]
    now we have to study, with $\hat{I} := (i_2, \dots, i_{|I|})$, the terms
    \begin{equation*}
        \begin{gathered}
            \E\Big[ \langle A_I S^N_0 + A_{\hat{I}}b_{i_1}, A_J S^N_0 + A_{\hat{J}}b_{j_1} \rangle_{\R^N}  \Big]
            \\ =
            \E\Big[ \langle A_I S^N_0 , A_J S^N_0 \rangle_{\R^N}  \Big] 
            + 
            \E\Big[ \langle A_{\hat{I}} b_{i_{1}} , A_{\hat{J}} b_{j_{1}} \rangle_{\R^N}  \Big]
            \\ +
            \E\Big[ \langle A_{\hat{I}}b_{i_1} , A_J S^N_0 \rangle_{\R^N}  \Big]
            +
            \E\Big[ \langle A_I S^N_0 , A_{\hat{J}}b_{j_1} \rangle_{\R^N}  \Big]
            \\ = 
            \E\Big[ (S^N_0)^T A^T_I A_J S^N_0 \Big]
            + 
            \E\Big[b_{i_{1}}^T A^T_{\hat{I}} A_{\hat{J}} b_{j_{1}} \Big]
            \\ +
            \E\Big[ b^T_{i_1} A^T_{\hat{I}} A_J S^N_0 \Big]
            + 
            \E\Big[ (S^N_0)^T A^T_I A_{\hat{J}} b_{j_{1}} \Big]
            \\ =
            \E\Big[ (S^N_0)^T A^T_I A_J S^N_0 \Big]
            + 
            \E\Big[b_{i_{1}}^T A^T_{\hat{I}} A_{\hat{J}} b_{j_{1}} \Big]
        \end{gathered}
    \end{equation*}
    
    where in the last equality we have used the independence of the terms and their 0 mean.
    
    \vspace{5pt}
    We already know that the first term is
    \[
       \E\Big[ (S^N_0)^T A^T_I A_J S^N_0 \Big] = N \sigma_{S_0}^2\sigma_A^{|I|+|J|} \big[ \delta_I^J + O(\frac{1}{N}) \big]
    \]
    
    \vspace{5pt}
    Concerning the second term: using independence we readily see how we must have $i_{1} = j_{1}$, then 
    
    \begin{equation*}
        \begin{gathered}
            \E\Big[b_{i_{1}}^T A^T_{\hat{I}} A_{\hat{J}} b_{j_{1}} \Big] 
            = 
            \sigma_b^2 \delta_{i_1}^{j_1} \cdot \sum_{n=1}^N  
            \E\Big[[A^T_{\hat{I}} A_{\hat{J}}]^n_n \Big]
            \\ =
            \sigma_b^2\delta_{i_1}^{j_1} \cdot \sum_{n=1}^N  \sigma_A^{|\hat{I}|+|\hat{J}|}
            \big( 
                \delta_{\hat{I}}^{\hat{J}} + \frac{1}{N}\psi(I,J,N,n,n)
            \big) 
            =
            N \sigma_b^2 \sigma_A^{|\hat{I}|+|\hat{J}|} \big[ \delta_I^J + O(\frac{1}{N}) \big]
        \end{gathered}
    \end{equation*}
    
    
    
    Hence
    \[
        \E\Big[ \langle A_I S^N_0 + A_{\hat{I}}b_{i_1}, A_J S^N_0 + A_{\hat{J}}b_{j_1} \rangle_{\R^N}  \Big]
        =
        N(\sigma_{S_0}^2 + \frac{\sigma_{b}^2}{\sigma_A^2})\sigma_A^{|I|+|J|}  \big[ \delta_I^J + O(\frac{1}{N}) \big]
    \]
    
\end{proof}


Assume now that the exchange of series with limits and expectation are justified, which we will prove later, then we would like to study the variance of the \emph{expected signature kernels} around their limits.

\begin{proposition}
    The coefficients in the expansion of the variance 
    \[
        \E\Big[
        \Big(\frac{\langle S^N_t(x), S^N_s(y) \rangle_{\R^N}}{N} - 
        \sigma_{S_0}^2\langle Sig(\sigma_A x)_{0,t}, Sig(\sigma_A y)_{0,s} \rangle_{T((\R^d))}\Big)^2
        \Big]
    \]
    
    are all $O(\frac{1}{N})$ when $\sigma_b = 0$.
\end{proposition}

\begin{proof}

We have
\begin{equation*}
    \begin{gathered}
        \frac{\langle S^N_t(x), S^N_s(y) \rangle_{\R^N}}{N} - 
        \sigma_{S_0}^2\langle Sig(\sigma_A x)_{0,t}, Sig(\sigma_A y)_{0,s} \rangle_{T((\R^d))}
        \\
        = \sum_{I, J \in \mathbb{W}_d} 
        \big[ \frac{1}{N}(S^N_0)^T A^T_{I}A_{J} S^N_0 - \sigma_{S_0}^2\sigma_{A}^{|I|+|J|}\delta_I^J \big]\hspace{3pt} Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)
    \end{gathered}
\end{equation*}
thus 
\begin{equation*}
    %\resizebox{\hsize}{!}{$
    \begin{gathered}
        \Big(
        \frac{\langle S^N_t(x), S^N_s(y) \rangle_{\R^N}}{N} - 
        \sigma_{S_0}^2\langle Sig(\sigma_A x)_{0,t}, Sig(\sigma_A y)_{0,s} \rangle_{T((\R^d))}
        \Big)^2
        = 
        \\
        \sum_{I, J, K, L \in \mathbb{W}_d} 
        \big[ \frac{1}{N} (S^N_0)^T A^T_{I}A_{J} S^N_0 - \sigma_{S_0}^2\sigma_{A}^{|I|+|J|}\delta_I^J \big]
        \big[ \frac{1}{N} (S^N_0)^T A^T_{K}A_{L} S^N_0 - \sigma_{S_0}^2\sigma_{A}^{|L|+|K|}\delta_K^L \big] 
        \hspace{3pt} Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)Sig^{K}_{0,t}(x) Sig^{L}_{0,s}(y)
    \end{gathered}
    %$}
\end{equation*}

\vspace{5pt}
Let us study
\begin{equation*}
\begin{gathered}
    \E\Big[ 
    \big[ \frac{1}{N} (S^N_0)^T A^T_{I}A_{J} S^N_0 - \sigma_{S_0}^2\sigma_{A}^{|I|+|J|}\delta_I^J \big]
    \big[ \frac{1}{N} (S^N_0)^T A^T_{K}A_{L} S^N_0 - \sigma_{S_0}^2\sigma_{A}^{|L|+|K|}\delta_K^L \big] 
    \Big] 
    \\
    = \frac{1}{N^2} \E\Big[ (S^N_0)^T A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0 \Big]\\
    - \frac{\sigma_{S_0}^2\sigma_{A}^{2|I|}}{N} \delta_I^J \E\Big[ (S^N_0)^T A^T_{K}A_{L}S^N_0 \Big]
    - \frac{\sigma_{S_0}^2\sigma_{A}^{2|L|}}{N} \delta_K^L \E\Big[ (S^N_0)^T A^T_{I}A_{J}S^N_0 \Big]
    + (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2\delta_I^J\delta_K^L 
    \\
    = \frac{1}{N^2}\E\Big[ (S^N_0)^T A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0 \Big]\\
    - \frac{\sigma_{S_0}^2\sigma_{A}^{2|I|}}{N}\delta_I^J N \sigma_{S_0}^2\sigma_A^{|K|+|L|} \big[ \delta_K^L + O(\frac{1}{N}) \big]
    - \frac{\sigma_{S_0}^2\sigma_{A}^{2|L|}}{N}\delta_J^K N \sigma_{S_0}^2\sigma_A^{|I|+|J|} \big[ \delta_I^J + O(\frac{1}{N}) \big]
    + (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2\delta_I^J\delta_K^L\\
    = \frac{1}{N^2} \E\Big[ (S^N_0)^T A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0 \Big] 
    - (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2 \delta_I^J\delta_K^L + O(\frac{1}{N})\\
\end{gathered}
\end{equation*}

from our previous results.

\vspace{5pt}
We have 
\begin{equation*}
\begin{gathered}
    (S^N_0)^T A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0 =\\
    \sum_{\alpha = 1}^N [S^N_0]_{\alpha} [A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0]_{\alpha} =\\
    \sum_{\alpha, \delta = 1}^N [S^N_0]_{\alpha} [A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}]_{\alpha}^{\delta}[S^N_0]_{\delta} =\\
    \sum_{\alpha, \beta, \gamma, \delta = 1}^N [S^N_0]_{\alpha} [A^T_{I}A_{J}]_{\alpha}^{\beta}[S^N_0  (S^N_0)^T]_{\beta}^{\gamma}[ A^T_{K}A_{L}]_{\gamma}^{\delta}[S^N_0]_{\delta} =\\
    \sum_{\alpha, \beta, \gamma, \delta = 1}^N [S^N_0]_{\alpha} [A^T_{I}A_{J}]_{\alpha}^{\beta}[S^N_0]_{\beta}[S^N_0]_{\gamma}[ A^T_{K}A_{L}]_{\gamma}^{\delta}[S^N_0]_{\delta} =\\
    \sum_{\alpha, \beta, \gamma, \delta = 1}^N [S^N_0]_{\alpha}[S^N_0]_{\beta}[S^N_0]_{\gamma}[S^N_0]_{\delta} [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\gamma}^{\delta}\\
\end{gathered}
\end{equation*}
hence by independence
\begin{equation*}
\begin{gathered}
    \E\Big[(S^N_0)^T A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0\Big] =\\
    \sum_{\alpha, \beta, \gamma, \delta = 1}^N \E\Big[[S^N_0]_{\alpha}[S^N_0]_{\beta}[S^N_0]_{\gamma}[S^N_0]_{\delta}\Big] \E\Big[[A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\gamma}^{\delta}\Big]\\
\end{gathered}
\end{equation*}

\vspace{10pt}
If $S_0^N$ is sampled from a Normal distribution as before then
\[
    \E\Big[[S^N_0]_{\alpha}[S^N_0]_{\beta}[S^N_0]_{\gamma}[S^N_0]_{\delta}\Big]
\]
is equal to $\sigma_{S_0}^4$ if $|\{\alpha, \beta, \gamma, \delta\}| = 2$, to
$3\sigma_{S_0}^4$ if $|\{\alpha, \beta, \gamma, \delta\}| = 1$ and to $0$ otherwise.

\vspace{10pt}
Remember how
\[
[A_I^T A_J]_{\alpha}^{\beta} = \sum_{\gamma = 1}^N \sum_{\bar{\delta} \in \Lambda^{N,|I|}_{\gamma,\alpha}} \sum_{\bar{\epsilon} \in \Lambda^{N,|J|}_{\gamma,\beta}} \prod_{i=1}^{|I|} \prod_{j=1}^{|J|}\hspace{3pt} [A_{I_i}]_{\delta_{i}}^{\delta_{i-1}} [A_{J_j}]_{\epsilon_{j}}^{\epsilon_{j-1}}
\]
thus 
\begin{equation*}
\begin{gathered}
    [A^T_{I}A_{J}]_{\alpha}^{\beta}
    [A^T_{K}A_{L}]_{\gamma}^{\delta}
    = \\
    \sum_{\epsilon, \phi = 1}^N 
    \sum_{\bar{\iota} \in \Lambda^{N,|I|}_{\epsilon,\alpha}} 
    \sum_{\bar{\zeta} \in \Lambda^{N,|J|}_{\epsilon,\beta}}
    \sum_{\bar{\kappa} \in \Lambda^{N,|K|}_{\phi,\gamma}}
    \sum_{\bar{\lambda} \in \Lambda^{N,|L|}_{\phi,\delta}}
    \prod_{i=1}^{|I|} \prod_{j=1}^{|J|}
    \prod_{k=1}^{|K|} \prod_{l=1}^{|L|}
    [A_{I_i}]_{\iota_{i}}^{\iota_{i-1}}
    [A_{J_j}]_{\zeta_{j}}^{\zeta_{j-1}}
    [A_{K_k}]_{\kappa_{k}}^{\kappa_{k-1}}
    [A_{L_l}]_{\lambda_{l}}^{\lambda_{l-1}}
\end{gathered}
\end{equation*}

Let us then define $T = I*J*K*L$, $\theta = (\iota*\zeta*\kappa*\lambda)$
and $\theta' = (\iota*\zeta*\kappa*\lambda)'$ just like before, setting $\mathcal{P} := P^2_{|I|+|J|+|K|+|L|}$ we get

\begin{equation*}
\begin{gathered}
    \E\Big[
    [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\gamma}^{\delta}
    \Big]=\\
    \sum_{p \in \mathcal{P}}
    \sum_{\epsilon, \phi = 1}^N 
    \sum_{\bar{\iota} \in \Lambda^{N,|I|}_{\epsilon,\alpha}} 
    \sum_{\bar{\zeta} \in \Lambda^{N,|J|}_{\epsilon,\beta}}
    \sum_{\bar{\kappa} \in \Lambda^{N,|K|}_{\phi,\gamma}}
    \sum_{\bar{\lambda} \in \Lambda^{N,|L|}_{\phi,\delta}}
    \prod_{a,b \in p}
    \E\Big[
    [A_{T_a}]_{\theta_{a}}^{\theta'_{a}}
    [A_{T_b}]_{\theta_{b}}^{\theta'_{b}}
    \Big]\\
    = \big( \frac{\sigma_A^2}{N} \big)^\frac{|I|+|J|+|K|+|L|}{2}\sum_{p \in \mathcal{P}} \omega(p,I,J,K,L,\alpha,\beta,\gamma,\delta)
\end{gathered}
\end{equation*}

and once again we need to analyze these $\omega$s which, just as before, must satisfy the constraint
\[
    \omega(p,I,J,K,L,\alpha,\beta,\gamma,\delta) 
    \leq N^\frac{|I|+|J|+|K|+|L|}{2}
\]

Since we are interested in the behavior for 
$N \to \infty$ and $|\mathcal{P}|$ is independent from $N$ we just need to discover when the previous inequality is an equality.
This happens, as we have previously discovered, when we the pairing does not add to the possible choices of $\bar{\iota}, \bar{\zeta}, \bar{\kappa}, \bar{\lambda}$ any more constraints than the unavoidable ones \emph{i.e.} 
$\theta_{|I|} = \theta_{|I|+|J|}$, $\theta_{|I|+ |J| + |K|} = \theta_{|I| + |J| + |K| + |L|}$, $\theta'_{1} = \alpha$,
$\theta'_{|I| + 1} = \beta$, $\theta'_{|I| + |J| + 1} = \gamma $ and $\theta'_{|I| + |J| + |K| + 1} = \delta $.

\vspace{5pt}
Reasoning exactly as before this can happen if and only if 
$I = J$, $\alpha = \beta$, $K = L$, $\gamma = \delta$, 
$\theta_a = \theta_{|I| + a}$ for $a = 1, \dots, |I|$ and 
$\theta_{2|I| + a} = \theta_{2|I| + |K| + a}$ for $a = 1, \dots, |K|$.

\vspace{5pt}
This means that 
\begin{equation*}
    \begin{gathered}
        \E\Big[
    [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\gamma}^{\delta}
    \Big]
    =
    (\sigma_A)^{|I|+|J|+|K|+|L|} \big[ \delta_I^J\delta_{\alpha}^{\beta}\delta_K^L\delta_{\gamma}^{\delta} + O(\frac{1}{N}) \big] \leq  
    \\ 
    (\sigma_A)^{|I|+|J|+|K|+|L|} \big[ \delta_I^J\delta_{\alpha}^{\beta}\delta_K^L\delta_{\gamma}^{\delta} + \frac{1}{N} \sigma(I,J,K,L) \big]
    \end{gathered}
\end{equation*} 
where $\sigma(I,J,K,L)$ is a positive constant corresponding to the maximal number of non zero pairings.

Since 
\begin{equation*}
\begin{gathered}
    \E\Big[(S^N_0)^T A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0\Big] \\
    = \sum_{\alpha, \beta, \gamma, \delta = 1}^N \E\Big[
    [S^N_0]_{\alpha}[S^N_0]_{\beta}[S^N_0]_{\gamma}[S^N_0]_{\delta}
    \Big] 
    \E\Big[
    [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\gamma}^{\delta}
    \Big]\\
    = \sum_{\alpha= 1}^N 3 \sigma_{S_0}^4
    \E\Big[
    [A^T_{I}A_{J}]_{\alpha}^{\alpha}[A^T_{K}A_{L}]_{\alpha}^{\alpha}
    \Big]
    + \sum_{\substack{\alpha, \beta=1 \\ \alpha \neq \beta}}^N \sigma_{S_0}^4
    \E\Big[
    [A^T_{I}A_{J}]_{\alpha}^{\alpha}[A^T_{K}A_{L}]_{\beta}^{\beta}
    \Big]\\
    + \sum_{\substack{\alpha, \beta=1 \\ \alpha \neq \beta}}^N \sigma_{S_0}^4
    \E\Big[
    [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\alpha}^{\beta}
    \Big]
    + \sum_{\substack{\alpha, \beta=1 \\ \alpha \neq \beta}}^N \sigma_{S_0}^4
    \E\Big[
    [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\beta}^{\alpha}
    \Big]\\
\end{gathered}
\end{equation*}

we end up with 
\begin{equation*}
\begin{gathered}
    \E\Big[(S^N_0)^T A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0\Big] = \\
     \sigma_{S_0}^4(\sigma_A)^{|I|+|J|+|K|+|L|} \big\{ N 3  (\delta_I^J\delta_K^L + O(\frac{1}{N}))
    + (N^2 - N)(\delta_I^J\delta_K^L +  O(\frac{1}{N}))
    + (N^2 - N)O(\frac{1}{N}) + (N^2 - N) O(\frac{1}{N}) \big\}\\
    = \sigma_{S_0}^4 (\sigma_A)^{|I|+|J|+|K|+|L|} N^2 \big[ \delta_I^J\delta_K^L +  O(\frac{1}{N}) \big]
    = (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2 N^2 \big[ \delta_I^J\delta_K^L +  O(\frac{1}{N}) \big]
\end{gathered}
\end{equation*}

In the end 
\begin{equation*}
    \begin{gathered}
        \E\Big[ 
        \big[ \frac{1}{N} (S^N_0)^T A^T_{I}A_{J} S^N_0 - \sigma_{S_0}^2\sigma_{A}^{|I|+|J|}\delta_I^J \big]
        \big[ \frac{1}{N} (S^N_0)^T A^T_{K}A_{L} S^N_0 - \sigma_{S_0}^2\sigma_{A}^{|L|+|K|}\delta_K^L \big] 
        \Big] =
        \\
        \frac{1}{N^2} \E\Big[ (S^N_0)^T A^T_{I}A_{J} S^N_0  (S^N_0)^T A^T_{K}A_{L}S^N_0 \Big] 
        - (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2 \delta_I^J\delta_K^L + O(\frac{1}{N}) =
        \\
        (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2 \big[ \delta_I^J\delta_K^L +  O(\frac{1}{N}) \big] - (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2 \delta_I^J\delta_K^L + O(\frac{1}{N}) = O(\frac{1}{N})
    \end{gathered}
\end{equation*}

\end{proof}

\begin{proposition}
        The coefficients in the expansion of the variance 
    \[
        \E\Big[
        \Big(\frac{\langle S^N_t(x), S^N_s(y) \rangle_{\R^N}}{N} - 
        \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\langle Sig(\sigma_A x)_{0,t}, Sig(\sigma_A y)_{0,s} \rangle_{T((\R^d))} + \frac{\sigma_b^2}{\sigma_A^2}\Big)^2
        \Big]
    \]
    
    are all $O(\frac{1}{N})$ with $\sigma_b > 0$.
\end{proposition}

\begin{proof}
Now 
\begin{equation*}
\begin{gathered}
    \langle S^N_t(x), S^N_s(y) \rangle_{\R^N} 
    = \\
    \sum_{I, J \in \mathbb{W}_d} 
        \big[ 
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        + (b_{I_{1}})^T A^T_{\hat{I}}A_{J} S^N_0
        + (S^N_0)^T A^T_{{I}}A_{\hat{J}} b_{J_{1}}
        + (b_{I_{1}})^T A^T_{\hat{I}}A_{\hat{J}} b_{J_{1}}
        \big] \hspace{3pt} 
        Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)
\end{gathered}
\end{equation*}

\vspace{10pt}
Thus to study 
\[
        \E\Big[
        \Big(\frac{\langle S^N_t(x), S^N_s(y) \rangle_{\R^N}}{N} - 
        \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\langle Sig(\sigma_A x)_{0,t}, Sig(\sigma_A y)_{0,s} \rangle_{T((\R^d))} + 
        \frac{\sigma_b^2}{\sigma_A^2}\Big)^2
        \Big]
    \]
we need to study the terms 
\begin{equation*}
\begin{gathered}
        \frac{1}{N^2} \E\Big[
        \big[ 
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        + (b_{I_{1}})^T A^T_{\hat{I}}A_{J} S^N_0
        + (S^N_0)^T A^T_{{I}}A_{\hat{J}} b_{J_{1}}
        + (b_{I_{1}})^T A^T_{\hat{I}}A_{\hat{J}} b_{J_{1}}
        - N\big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|I|+|J|}\delta_I^J
        \big] \cdot\\
        \cdot \big[ 
        (S^N_0)^T A^T_{K}A_{L} S^N_0
        + (b_{K_{1}})^T A^T_{\hat{K}}A_{L} S^N_0
        + (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{L_{1}}
        + (b_{K_{1}})^T A^T_{\hat{K}}A_{\hat{L}} b_{L_{1}}
        - N\big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|}\delta_K^L
        \big]
        \Big]
\end{gathered}
\end{equation*}

To ease the notation let us write $i, j, k$ and $l$ instead of, respectively, $I_{1}, J_{1}, K_{1}$ and $L_{1}$.

\vspace{10pt}
We have 
\begin{equation*}
\begin{gathered}
        \E\Big[
        \big[ 
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        \big]
        \cdot 
        \big[ 
        (S^N_0)^T A^T_{K}A_{L} S^N_0
        + (b_{k})^T A^T_{\hat{K}}A_{L} S^N_0
        + (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
        + (b_{k})^T A^T_{\hat{K}}A_{\hat{L}} b_{l}
        - N \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|} \delta_K^L
        \big]
        \Big]
        \\
        = 
        \E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        (S^N_0)^T A^T_{K}A_{L} S^N_0
        \Big]\\
        +\E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        (b_{k})^T A^T_{\hat{K}}A_{L} S^N_0
        \Big]\\
        +\E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
        \Big]\\
        +\E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        (b_{k})^T A^T_{\hat{K}}A_{\hat{L}} b_{l}
        \Big]\\
         - N \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|}\delta_K^L\E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        \Big]
\end{gathered}
\end{equation*}
which by previous results is equal to 
\begin{equation*}
\begin{gathered}
        (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2 N^2 \big[ \delta_I^J\delta_K^L +  O(\frac{1}{N}) \big]\\
        +\E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        (b_{k})^T A^T_{\hat{K}}A_{L} S^N_0
        \Big]\\
        +\E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
        \Big]\\
        +\E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        (b_{k})^T A^T_{\hat{K}}A_{\hat{L}} b_{l}
        \Big]\\
         - \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|}\delta_K^L \sigma_{S_0}^2\sigma_A^{|I|+|J|} 
         N^2 \big[ \delta_I^J + O(\frac{1}{N}) \big]
\end{gathered}
\end{equation*}

Note then how 
\begin{equation*}
\begin{gathered}
        \E\Big[
        (S^N_0)^T 
        A^T_{I}A_{J} 
        S^N_0
        (b_{k})^T 
        A^T_{\hat{K}}A_{L} 
        S^N_0
        \Big]
        \\
        = \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \E\Big[
        [S^N_0]_{\alpha}
        [S^N_0]_{\beta}
        [b_{k}]_{\gamma}
        [S^N_0]_{\delta}
        \Big] 
        \E\Big[
        [A^T_{I}A_{J}]_{\alpha}^{\beta}
        [A^T_{K}A_{L}]_{\gamma}^{\delta}
        \Big]
        \\
        = \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \E\Big[
        [S^N_0]_{\alpha}
        [S^N_0]_{\beta}
        [S^N_0]_{\delta}
        \Big]
        \E\Big[
        [b_{k}]_{\gamma}
        \Big]
        \E\Big[
        [A^T_{I}A_{J}]_{\alpha}^{\beta}
        [A^T_{K}A_{L}]_{\gamma}^{\delta}
        \Big]
        = 0
        \\
\end{gathered}
\end{equation*}
given that 
$\E\Big[[b_{k}]_{\gamma}\Big] = 0$.
Analogously we have
\begin{equation*}
\begin{gathered}
        \E\Big[
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
        \Big]
        = 0
\end{gathered}
\end{equation*}

Finally
\begin{equation*}
\begin{gathered}
        \E\Big[
        (S^N_0)^T 
        A^T_{I}A_{J} 
        S^N_0
        (b_{k})^T 
        A^T_{\hat{K}}A_{\hat{L}} 
        b_{l}
        \Big]
        \\
        = \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \E\Big[
        [S^N_0]_{\alpha}
        [S^N_0]_{\beta}
        [b_{k}]_{\gamma}
        [b_{l}]_{\delta}
        \Big] 
        \E\Big[
        [A^T_{I}A_{J}]_{\alpha}^{\beta}
        [A^T_{\hat{K}}A_{\hat{L}}]_{\gamma}^{\delta}
        \Big]
        \\
        = \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \E\Big[
        [S^N_0]_{\alpha}
        [S^N_0]_{\beta}
        \Big]
        \E\Big[
        [b_{k}]_{\gamma}
        [b_{l}]_{\delta}
        \Big]
        \E\Big[
        [A^T_{I}A_{J}]_{\alpha}^{\beta}
        [A^T_{\hat{K}}A_{\hat{L}}]_{\gamma}^{\delta}
        \Big]
        \\
        = \sigma_{S_0}^2 \sigma_{b}^2 \sigma_A^{|I|+|J|+|\hat{K}|+|\hat{L}| } \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        {\delta_{\alpha}^{\beta}}
        {\delta_{\gamma}^{\delta}\delta_{k}^{l}}
        (\delta_{I}^{J}\delta_{\hat{K}}^{\hat{L}}\delta_{\alpha}^{\beta}\delta_{\gamma}^{\delta} + O(\frac{1}{N}) )
        \\ 
        = \sigma_{S_0}^2 \sigma_{b}^2 \sigma_A^{|I|+|J|+|\hat{K}|+|\hat{L}| }
        \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \delta_{\alpha}^{\beta}
        \delta_{\gamma}^{\delta}
        \big(
        \delta_{k}^{l}
        \delta_{I}^{J}
        \delta_{\hat{K}}^{\hat{L}}
        + O(\frac{1}{N})
        \big)
        \\
        = \sigma_{S_0}^2 \sigma_{b}^2 \sigma_A^{|I|+|J|+|\hat{K}|+|\hat{L}| } 
        \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \delta_{\alpha}^{\beta}
        \delta_{\gamma}^{\delta}
        \big(
        \delta_{I}^{J}
        \delta_{K}^{L}
        + O(\frac{1}{N})
        \big)
        \\
        = \sigma_{S_0}^2 \sigma_{b}^2 \sigma_A^{|I|+|J|+|\hat{K}|+|\hat{L}| }
        \sum_{\alpha, \gamma = 1}^N 
        \big(
        \delta_{I}^{J}
        \delta_{K}^{L}
        + O(\frac{1}{N})
        \big)
        = \sigma_{S_0}^2 \sigma_{b}^2 \sigma_A^{|I|+|J|+|\hat{K}|+|\hat{L}| } N^2 
        \big[ \delta_{I}^{J} \delta_{K}^{L} + O(\frac{1}{N}) \big]
\end{gathered}
\end{equation*}
where once again we use the fact that all the $O(\frac{1}{N})$ are uniformly bounded above by some $O(\frac{1}{N})$.

Putting everything together 
\begin{equation*}
\begin{gathered}
        \E\Big[
        \big[ 
        (S^N_0)^T A^T_{I}A_{J} S^N_0
        \big]
        \cdot 
        \big[ 
        (S^N_0)^T A^T_{K}A_{L} S^N_0
        + (b_{k})^T A^T_{\hat{K}}A_{L} S^N_0
        + (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
        + (b_{k})^T A^T_{\hat{K}}A_{\hat{L}} b_{l}
        - N \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|} \delta_K^L
        \big]
        \Big]\\
        = 
        (\sigma_{S_0}^2\sigma_{A}^{|L|+|I|})^2 N^2 \big[ \delta_I^J\delta_K^L +  O(\frac{1}{N}) \big]
        + 0
        + 0
        +\sigma_{S_0}^2 \sigma_{b}^2 \sigma_A^{|I|+|J|+|\hat{K}|+|\hat{L}| } N^2 
        \big[ \delta_{I}^{J} \delta_{K}^{L} + O(\frac{1}{N}) \big] \\
         -  \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|}\delta_K^L \sigma_{S_0}^2\sigma_A^{|I|+|J|} 
         N^2 \big[ \delta_I^J + O(\frac{1}{N}) \big] = N^2{O(\frac{1}{N})}
\end{gathered}
\end{equation*}

\vspace{10pt}
With analogous arguments we obtain 
\begin{equation*}
    \resizebox{\hsize}{!}{$
\begin{gathered}
        \E\Big[
        \big[ 
        (b_i)^T A^T_{\hat{I}}A_{J} S^N_0
        \big]
        \cdot 
        \big[ 
        (S^N_0)^T A^T_{K}A_{L} S^N_0
        + (b_{k})^T A^T_{\hat{K}}A_{L} S^N_0
        + (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
        + (b_{k})^T A^T_{\hat{K}}A_{\hat{L}} b_{l}
        - N \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|}\delta_K^L
        \big]
        \Big]\\
        = 0 
        + \E\Big[
        ((b_i)^T A^T_{\hat{I}}A_{J} S^N_0
        (b_{k})^T A^T_{\hat{K}}A_{L} S^N_0
        \Big]
        +\E\Big[
        (b_i)^T A^T_{\hat{I}}A_{J} S^N_0
        (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
        \Big]
        + 0  - N \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|}\delta_K^L \cdot 0
\end{gathered}
$}
\end{equation*}
and since 
\begin{equation*}
\begin{gathered}
        \E\Big[
        (b_i)^T 
        A^T_{\hat{I}}A_{J} 
        S^N_0
        (b_{k})^T 
        A^T_{\hat{K}}A_{L} 
        S^N_0
        \Big]
        \\
        = \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \E\Big[
        [S^N_0]_{\beta}
        [S^N_0]_{\delta}
        \Big] 
        \E\Big[
        [b_{i}]_{\alpha}
        [b_{k}]_{\gamma}
        \Big] 
        \E\Big[
        [A^T_{\hat{I}}A_{J}]_{\alpha}^{\beta}
        [A^T_{\hat{K}}A_{{L}}]_{\gamma}^{\delta}
        \Big]
        \\
        = \sigma_{S_0}^2 \sigma_b^2  \sigma_A^{|\hat{I}|+|J|+|\hat{K}|+|{L}| }
        \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        {\delta_{\beta}^{\delta}}
        {\delta_{\alpha}^{\gamma}\delta_{i}^{k}}
        (
        \delta_{\hat{I}}^{J}
        \delta_{\hat{K}}^{L}
        \delta_{\alpha}^{\beta}
        \delta_{\gamma}^{\delta}
        +
        O(\frac{1}{N})
        )
        \\
        =  \sigma_{S_0}^2 \sigma_b^2  \sigma_A^{|\hat{I}|+|J|+|\hat{K}|+|{L}|}
        \big[
        \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \delta_{\beta}^{\delta}
        \delta_{\alpha}^{\gamma}
        \delta_{i}^{k}
        \delta_{\hat{I}}^{J}
        \delta_{\hat{K}}^{L}
        \delta_{\alpha}^{\beta}
        \delta_{\gamma}^{\delta}
        + 
        \sum_{\alpha, \beta, \gamma, \delta = 1}^N 
        \delta_{\beta}^{\delta}
        \delta_{\alpha}^{\gamma}\delta_{i}^{k}
        O(\frac{1}{N})
        \big]
        \\
        = \sigma_{S_0}^2 \sigma_b^2  \sigma_A^{|\hat{I}|+|J|+|\hat{K}|+|{L}|}
        \big[
        \sum_{\alpha = 1}^N 
        \delta_{i}^{k}
        \delta_{\hat{I}}^{J}
        \delta_{\hat{K}}^{L}
        + \sum_{\alpha, \beta = 1}^N 
        \delta_{i}^{k}
        O(\frac{1}{N}) 
        \big]
        \\ 
       \sigma_{S_0}^2 \sigma_b^2  \sigma_A^{|\hat{I}|+|J|+|\hat{K}|+|{L}|}
        \big[
         N 
        \delta_{i}^{k}
        \delta_{\hat{I}}^{J}
        \delta_{\hat{K}}^{L}
        +
        N^2 
        \delta_{i}^{k}
        O(\frac{1}{N})
        \big]
        =
        N^2O(\frac{1}{N})
\end{gathered}
\end{equation*}

and similarly 
\[
    \E\Big[
    (b_i)^T A^T_{\hat{I}}A_{J} S^N_0
    (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
    \Big]
    = N^2O(\frac{1}{N})
\]
we finally obtain 
\begin{equation*}
    \resizebox{\hsize}{!}{$
\begin{gathered}
        \E\Big[
        \big[ 
        (b_i)^T A^T_{\hat{I}}A_{J} S^N_0
        \big]
        \cdot 
        \big[ 
        (S^N_0)^T A^T_{K}A_{L} S^N_0
        + (b_{k})^T A^T_{\hat{K}}A_{L} S^N_0
        + (S^N_0)^T A^T_{{K}}A_{\hat{L}} b_{l}
        + (b_{k})^T A^T_{\hat{K}}A_{\hat{L}} b_{l}
        - N \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)\sigma_A^{|K|+|L|}\delta_K^L
        \big]
        \Big]\\
        = N^2O(\frac{1}{N})
\end{gathered}
$}
\end{equation*}

Using the same arguments developed up to here all other terms in the product end up as being $N^2O(\frac{1}{N})$ thus dividing finally by $N^2$ we have the thesis.
\end{proof}

\subsection{On the question of convergence}

We will just do the case $(\sigma_{S_0},\sigma_A,\sigma_B) = (1,1,0)$.
The arguments for the general case are the same.

\begin{proposition}
    \begin{equation*}
        \begin{gathered}
            \lim_{N \to \infty} 
            \sum_{I \in \mathbb{W}_d}\sum_{J \in \mathbb{W}_d}
            \frac{1}{N}\E[(S_0^N)^T A^T_I A_J S^N_0]
            Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)
            \\ =
            \sum_{I \in \mathbb{W}_d}\sum_{J \in \mathbb{W}_d}
            \lim_{N \to \infty} 
            \frac{1}{N}\E[(S_0^N)^T A^T_I A_J S^N_0]
            Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)
        \end{gathered}
    \end{equation*}
\end{proposition}

\begin{proof}
First of all, to be thoroughly rigorous, we need to define a probability space over which we take all the expectations, everything is numerable thus there is no issues with this.

\vspace{5pt}
To justify the exchange of sum and limit we want to use Lebesgue dominated convergence, we thus need to bound the 
$$|\frac{1}{N}\E[(S_0^N)^T A^T_I A_J S^N_0]Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)|$$
from above.

We know, from previous considerations, that 
\[
    \frac{1}{N}\E[(S_0^N)^T A^T_I A_J S^N_0] =
    \sum_{n=1}^N \frac{1}{N} \E\Big[[A^T_I A_J]^n_n \Big]
\]

and that
\[
    \E\Big[[A^T_I A_J]^n_n \Big]
    =
    \Big(\frac{1}{N}\Big)^{\frac{|I|+|J|}{2}} \sum_{p \in P^2_{|I|+|J|}} \omega(p,I,J,N,n,n) 
\]
thus, since $\omega(p,I,J,N,\alpha,\beta)  \leq N^{\frac{|I|+|J|}{2}}$, we obtain
\[
    \E\Big[[A^T_I A_J]^n_n \Big] \leq |P^2_{|I|+|J|}| \leq (|I|+|J|)!! 
\]

We have also seen that 
$\E\Big[[A^T_I A_J]^n_n \Big] = 0$ if $|I|+|J|$ is odd, thus we can consider $|I|+|J|$ to be even; then, writing $i,j$ instead of $|I|,|J|$ for ease of reading, we get
\[
    (|I|+|J|)!! = \bigl( 2 (\frac{i+j}{2}) \bigr) !!
    = 2^{\frac{i+j}{2}} \bigl( \frac{i+j}{2} \bigr)!
\]

Putting everything together we have found 
\[
    |\frac{1}{N}\E[(S_0^N)^T A^T_I A_J S^N_0]| \leq 2^{\frac{i+j}{2}} \bigl( \frac{i+j}{2} \bigr)!
\]
and 
\[
    2 \nmid i+j \implies \frac{1}{N}\E[(S_0^N)^T A^T_I A_J S^N_0] = 0
\]

\vspace{5pt}
Finally remember how, by factorial decay,
\[
    |Sig^{I}_{0,t}(x)| \leq \frac{\norm{x}^{|I|}_{1-var}}{|I|!}
\]

\vspace{5pt}
We have now to prove, by \cite{tao2016analysis}[8.2.1 and 8.2.2], that 
\begin{align*}
    &\sum_{I \in \mathbb{W}_d}\sum_{J \in \mathbb{W}_d}
     2^{\frac{|I|+|J|}{2}} \bigl( \frac{|I|+|J|}{2} \bigr)! 
     \hspace{5pt} 
     \mathbb{I}_{2 | |I|+|J|} 
     \hspace{5pt}
     \frac{\norm{x}^{|I|}}{|I|!}\frac{\norm{y}^{|J|}}{|J|!}
    \\ =
    &\sum_{i \in \N}\sum_{j \in \N} 
    d^i d^j
     2^{\frac{i+j}{2}} \bigl( \frac{i+j}{2} \bigr)! 
     \hspace{5pt} 
     \mathbb{I}_{2 | i+j} 
     \hspace{5pt}
     \frac{\norm{x}^i}{i!}\frac{\norm{y}^j}{j!}
    <
    \infty
\end{align*}


Once again by \cite{tao2016analysis}[8.2.1 and 8.2.2] we have to find a bijection 
$\phi : \N  \to \N \times \N$ such that, if 
\[
    f(i,j) = 
    d^i d^j
    2^{\frac{i+j}{2}} \bigl( \frac{i+j}{2} \bigr)! 
    \hspace{5pt} 
    \mathbb{I}_{2 | i+j} 
    \hspace{5pt}
    \frac{\norm{x}^i}{i!}\frac{\norm{y}^j}{j!}
\]
then 
\[
    \sum_{k \in \N} f(\phi(k)) < \infty
\]

\vspace{5pt}
As a first step assume $2 | i+j$ and, writing 
$i \wedge j := \min\{i,j\}$ and $i \vee j := \max\{i,j\}$, note how 
\begin{equation*}
    \resizebox{\hsize}{!}{$
    \begin{gathered}
        f(i,j) = f(i \wedge j , i \vee j)
        \\ \leq
        \frac{
        (d\norm{x})^i(d\norm{y})^j 2^{\frac{i+j}{2}} \bigl( \frac{i+j}{2} \bigr)!
        }{
        (i \wedge j)! (i \vee j)!
        }
        =
        \frac{
        (d\norm{x})^i(d\norm{y})^j 2^{\frac{i+j}{2}} \bigl( \frac{i+j}{2} \bigr) \cdots (i \wedge j +1)
        }{
        (i \vee j)!
        }
        =
        \frac{
        (d\norm{x})^i(d\norm{y})^j 2^{\frac{i+j}{2}} 
        }{
        (i \vee j) \cdots \bigl( \frac{i+j}{2}  + 1\bigr) \cdot (i \wedge j)!
        }
        \\ \leq 
        \frac{
        d^{i+j}\norm{x}^i\norm{y}^j 2^{\frac{i+j}{2}} 
        }{
        \bigl( \frac{i+j}{2}\bigr)! 
        }
        \leq 
        \frac{
        d^{i+j}\bigr[(1+\norm{x})(1+\norm{y})\bigr]^{i+j} 2^{\frac{i+j}{2}} 
        }{
        \bigl( \frac{i+j}{2}\bigr)! 
        }
    \end{gathered}
    $}
\end{equation*}

Consider then $\phi$ as the inverse of the map $(i,j) \mapsto \frac{1}{2}(i+j)(i+j+1) + j$ 
\emph{i.e.} $\phi$ is the map enumerating pairs $(i,j)$ starting from $(0,0)$ and proceeding
with diagonal motions of the form 
$$(m,0) \to (m-1,1) \to \dots \to (0,m)$$
and then $(0,m) \to (m+1,0)$.
Notice that such diagonal strides have length $m+1$ and comprise all couples
$(i,j)$ such that $i+j = m$.

\vspace*{5pt}
Since there are exactly $2k + 1$ choices of $(i,j)$ such that $\frac{i+j}{2} = k$,
corresponding to the couples $(i,2k - i)$ for $i = 0, \dots, 2k$, using the above $\phi$
it suffices to prove
\[
    \sum_{k \in \N} (2k + 1)
    \frac{\bigr[d(1+\norm{x})(1+\norm{y})\bigr]^{2k} 2^{k} }{k}
    =
    \sum_{k \in \N} (2k + 1)
    \frac{\bigr[2d^2(1+\norm{x})^2(1+\norm{y})^2\bigr]^k}{k!} 
    <
    \infty
\]

Since 
\begin{equation*}
    \begin{gathered}
        \sum_{k \in \N} (2k + 1)
        \frac{\bigr[2d^2(1+\norm{x})^2(1+\norm{y})^2\bigr]^k}{k!} 
        \\\leq
        \sum_{k \in \N} 2^{k+1}
        \frac{\bigr[2d^2(1+\norm{x})^2(1+\norm{y})^2\bigr]^k}{k!} 
        =
        2e^{\bigl[2d(1+\norm{x})(1+\norm{y})\bigr]^2} 
        <
        \infty
    \end{gathered}
\end{equation*}

we are done.

\end{proof}


\begin{proposition}
    The exchange of sums and expectations has always been justified.
\end{proposition}

\begin{proof}
    For the case with just two indices $I,J$ we need to use Fubini-Tonelli and prove that 
    \begin{equation*}
        \begin{gathered}
            \E \Biggl[ 
            \sum_{I \in \mathbb{W}_d}\sum_{J \in \mathbb{W}_d}
            \frac{1}{N}|(S_0^N)^T A^T_I A_J S^N_0
            Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)|
            \Biggr]
            \\=
            \sum_{I \in \mathbb{W}_d}\sum_{J \in \mathbb{W}_d}
            \E[ \frac{1}{N}|(S_0^N)^T A^T_I A_J S^N_0 |]
            |Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)|
            <
            \infty  
        \end{gathered}  
    \end{equation*}
    
    
    
    \vspace{5pt}
    We have 
    \begin{equation*}
        \begin{gathered}
            \frac{1}{N} \E[ |(S_0^N)^T A^T_I A_J S^N_0 |] 
            \leq 
            \sqrt{\frac{1}{N^2}\E[ ((S_0^N)^T A^T_I A_J S^N_0)^2] }
        \end{gathered}
    \end{equation*}
    
    
    Remember how 
    \begin{equation*}
        \begin{gathered}
            \frac{1}{N^2}\E[ (S_0^N)^T A^T_I A_J S^N_0 (S_0^N)^T A^T_I A_J S^N_0] \\
            = \sum_{\alpha= 1}^N \frac{3}{N^2}
            \E\Big[
            [A^T_{I}A_{J}]_{\alpha}^{\alpha}[A^T_{I}A_{J}]_{\alpha}^{\alpha}
            \Big]
            + \sum_{\substack{\alpha, \beta=1 \\ \alpha \neq \beta}}^N \frac{1}{N^2}
            \E\Big[
            [A^T_{I}A_{J}]_{\alpha}^{\alpha}[A^T_{I}A_{J}]_{\beta}^{\beta}
            \Big]\\
            + \sum_{\substack{\alpha, \beta=1 \\ \alpha \neq \beta}}^N \frac{1}{N^2}
            \E\Big[
            [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{I}A_{J}]_{\alpha}^{\beta}
            \Big]
            + \sum_{\substack{\alpha, \beta=1 \\ \alpha \neq \beta}}^N \frac{1}{N^2}
            \E\Big[
            [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{I}A_{J}]_{\beta}^{\alpha}
            \Big]\\
        \end{gathered}
    \end{equation*}
    
    and how 
    \begin{equation*}
        \begin{gathered}
            \E\Big[
            [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\gamma}^{\delta}
            \Big]=\\
            = \frac{1}{N^\frac{|I|+|J|+|K|+|L|}{2}}\sum_{p \in \mathcal{P}} \omega(p,I,J,K,L,\alpha,\beta,\gamma,\delta)
        \end{gathered}
    \end{equation*}
    where
    \[
        \omega(p,I,J,K,L,\alpha,\beta,\gamma,\delta) 
        \leq N^\frac{|I|+|J|+|K|+|L|}{2}
    \]
    thus 
    \begin{equation*}
        \begin{gathered}
            \E\Big[
            [A^T_{I}A_{J}]_{\alpha}^{\beta}[A^T_{K}A_{L}]_{\gamma}^{\delta}
            \Big]
            \leq
            |P^2_{|I|+|J|+|K|+|L|}| 
            \leq
            (|I|+|J|+|K|+|L|)!!
        \end{gathered}
    \end{equation*}
    
    \vspace{5pt}
    In our case $K = I$ and $J = L$, hence 
    \[
    (|I|+|J|+|K|+|L|)!! = (2|I|+2|J|)!! \leq 2^{|I|+|J|}(|I|+|J|)!
    \]
    
    
    \vspace{5pt}
    Putting all together
    \begin{equation*}
        \begin{gathered}
            \frac{1}{N} \E[ |(S_0^N)^T A^T_I A_J S^N_0 |] 
            \leq 
            \sqrt{\frac{1}{N^2}\E[ ((S_0^N)^T A^T_I A_J S^N_0)^2] }
            \\ \leq
            \sqrt{6 \cdot 2^{|I|+|J|}(|I|+|J|)!}
            \leq
            \sqrt{6} \cdot  2^{\frac{|I|+|J|}{2}}(|I|+|J|)!!
        \end{gathered}
    \end{equation*}
       
     where we have used
     \[
        (|I|+|J|)! = (|I|+|J|)!! (|I|+|J| - 1)!! \leq [(|I|+|J|)!!]^2
     \]
     
     \vspace{5pt}
     Finally
     
     \begin{equation*}
        \begin{gathered}
            \sum_{I \in \mathbb{W}_d}\sum_{J \in \mathbb{W}_d}
            \frac{1}{N} \E[ |(S_0^N)^T A^T_I A_J S^N_0 |]
            |Sig^{I}_{0,t}(x) Sig^{J}_{0,s}(y)|
            \\ \leq
            \sum_{I \in \mathbb{W}_d}\sum_{J \in \mathbb{W}_d}
             \sqrt{6} \cdot  2^{\frac{|I|+|J|}{2}}(|I|+|J|)!! 
             \frac{\norm{x}^{|I|}}{|I|!}\frac{\norm{y}^{|J|}}{|J|!}
        \end{gathered}  
    \end{equation*}
    
    which is proved to be $<\infty$ exactly as in the previous proof, this time taking care to consider also the case $|I|+|J|$ \emph{not} even.
    
    
    \vspace{10pt}
    The case with 4 words, \emph{i.e.} the variance case, goes similarly. 
\end{proof}


Putting all of this together we have finally proved the theorem:

\begin{theorem}
    Consider randomized Signatures of the type 
\[
   S^{N}_t(x) = S_0 + \sum_{k=1}^d \int_0^t \big( A_k S^{N}_{\tau}(x)  + b_k \big) dx_{\tau}^k
\]
where $x \in \bX$ and 
\[
    [A_{k}]_{\alpha}^{\beta} \sim \mathcal{N}(0,\frac{\sigma_{A}^2}{N}) 
    \hspace{15pt}
    [Y_0]_{\alpha}\sim \mathcal{N}(0,\sigma_{S_0}^2)
    \hspace{15pt}
    [b_{k}]_{\alpha} \sim \mathcal{N}(0,\sigma_b^2)
\]

Then
    \[
        \lim_{N \to \infty} \E\Big[
        \frac{1}{N}\langle S^N_t(x), S^N_s(y) \rangle_{\R^N}\Big] = 
        \big( \sigma_{S_0}^2 + \frac{\sigma_b^2}{\sigma_A^2}\big)  SigKer^{\sigma_A x,\sigma_A y}({t,s}) - \frac{\sigma_b^2}{\sigma_A^2}
    \]
    and the variance around the limit is of order $O(\frac{1}{N})$.
\end{theorem}





\section{Convergence to a Gaussian process}

Fix $\X := \{x_1, \dots, x_m\} \subseteq \bX$.
Let moreover $v^N \in \R^N$ be sampled from $\mathcal{N}(0,I)$. 
Define the vectors
\[
    X^N_{\X} := [
    \sprod{v^N}{S^N(x_j)_1}_{\R^N}
    ]_{j=1,\dots,m}
\]


\begin{proposition}
    $X^N_{\X}$ converge in distribution to a $\mathcal{N}(0,K^{id}_{1,1}(\X,\X))$.
\end{proposition}

\begin{proof}
    By \emph{Lévy's continuity theorem} it suffices to study the limiting behavior of the characteristic functions
    
    \begin{equation*}
        \begin{gathered}
            \varphi_N(u) 
            := 
            \E[\exp{\big\{ i u^T X^N_{\X} \big\} }] 
            \\ =
            \E[\exp{\big\{ i \sum_{j=1}^m u_j [X^N_{\X}]_j \big\} }]
            = 
            \E[\exp{\big\{ i \sum_{j=1}^m u_j \sprod{v^N}{S^N(x_j)_1} \big\} }]
            \\ =
            \E[\exp{\big\{ i  \sprod{\sum_{j=1}^m u_j S^N(x_j)_1}{v^N} \big\} }]
            \\ =
            \E[\E[\exp{\big\{ i  \sprod{\sum_{j=1}^m u_j S^N(x_j)_1}{v^N} \big\} }| V_1, \dots, V_d, S_0]]
        \end{gathered}
    \end{equation*}
    
    But if we know $V_1, \dots, V_d, S_0$ the randomized signatures are deterministic objects, and $v^N$ is normally distributed; thus
    
    \begin{equation*}
        \begin{gathered}
            \varphi_N(u) 
            =
            \E[\E[\exp{\big\{ i  \sprod{\sum_{j=1}^m u_j S^N(x_j)_1}{v^N} \big\} }| V_1, \dots, V_d, S_0]]
            \\ =
            \E[\exp{\big\{ 
                -\frac{1}{2} \sprod{\sum_{j=1}^m u_j S^N(x_j)_1}{\sum_{j=1}^m u_j S^N(x_j)_1}
            \big\}}]
            \\ =
            \E[\exp{\big\{ 
                -\frac{1}{2} \sum_{i,j=1}^m u_i u_j \sprod{ S^N(x_i)_1}{S^N(x_j)_1}
            \big\}}]
            \\ = 
            E[\exp{\big\{ 
                -\frac{1}{2} \sprod{u}{G^N_{x} u}
            \big\}}]
        \end{gathered}
    \end{equation*}
    where 
    \[
        [G^N_{x}]_i^j := \sprod{ S^N(x_i)_1}{S^N(x_j)_1}
    \]
    

\vspace{5pt}
    Now, since we have proven that
    \[
        \sprod{ S^N(x_i)_1}{S^N(x_j)_1}
        \xrightarrow[N \to \infty]{\mathbb{L}^2} \sprod{Sig_{0,1}(x_i)}{Sig_{0,1}(x_j)}_{T((\R^d))}
        =
        [K^{id}_{1,1}(\X,\X)]_i^j 
    \]
    we have 
    \[
        G^N_{\X}
        \xrightarrow[N \to \infty]{\mathbb{L}^2}
        K^{id}_{1,1}(\X,\X) := \Sigma
    \]

    \vspace{5pt}
    Thus, since $\mathbb{L}^2$ convergence implies convergence in distribution, by the classical \emph{Portmanteau theorem} we must have 
    \[
        \E[h(G^N_{x})] 
        \xrightarrow[N \to \infty]{}  
        \E[h(\Sigma)] = h(\Sigma)
    \]
    for every continuous and bounded $h : \R^{m \times m} \to \R$

    \vspace{5pt}
    Fix $ u \in \R^m$ and consider 
    \[
        f_u : \R^{m \times m} \to \R 
        \hspace{3pt} \text{s.t.} \hspace{3pt}
        A \mapsto \exp\bigl\{ - \frac{1}{2} \sprod{u}{Au} \bigr\}
    \]
    
    We would like to take $h = f_u$, unfortunately if $u \neq 0$ then $f_u$ is \emph{not} bounded: taking $A = - \mathbb{I}_{m\times m}$ we have 
    \[
        f(kA) = \exp \{ \frac{k}{2} \norm{u}_2^2 \} \xrightarrow[k \to \infty]{} + \infty
    \]
    
    Fortunately we are only interested in evaluating $f_u$ on the $G^N_{x}$ which are all positive semidefinite matrices:
    \[
        G^N_{x} = (W^N_{x})^T W^N_{x}
    \]
    where $W^N_{x} \in \R^{N \times m}$ is defined by
    \[
        [W^N_{x}]_i^j := [S^N(x_j)]_i
    \]
    thus for any $u \in \R^m$ it holds that
    \[
        u^T G^N_{x} u = u^T (W^N_{x})^T W^N_{x} u
        = 
        (W^N_{x} u)^T W^N_{x} u = \norm{W^N_{x} u}_2^2 \geq 0
    \]

    Since the $G^N_{x}$ are semidefinite we have 
    $$0 < f_u(G^N_{x}) \leq 1 $$
    for any $u$, hence we always have
    \[
        f_u(G^N_{x}) = \psi \circ f_u(G^N_{x})
    \]
    
    where $\psi: \R \to \R$ is defined by $\psi(x) := \min\{x,2\}$.
    
    To end notice how $\psi \circ f_u : \R^{m \times m} \to \R$
    is continuous, being composition of continuous functions, and bounded, since 
    \[
     0 < \psi \circ f_u(A) \leq 2
    \]
    
    Then we have, for every $u \in \R^m$, that 
    \[
        \E[f_u(G^N_{x})]  
        =
        \E[(\psi \circ f_u)(G^N_{x})] 
        \xrightarrow[N \to \infty]{}  
        (\psi \circ f_u)(\Sigma)
        =
        f_u(\Sigma)
    \]
    
    where we have used the semidefinitiveness of $\Sigma$.
    With this we finally conclude that
    \[
    \varphi_N(u) 
    \xrightarrow[N \to \infty]{} 
    \exp \bigl\{-\frac{1}{2} \sprod{u}{\Sigma u} \bigr\}
    \]

\end{proof}

We have just proved
\begin{proposition}
Let $\varphi = id$. For any subset $\X = \{x_1, \dots, x_n\} \subset \bX$ the following convergence holds
\[
    \lim_{N \to \infty} \lim_{M \to \infty} \E[ \sprod{\psi^{\D_M, N}_{hom}(\X)}{\psi^{\D_M, N}_{hom}(\X)} ] 
    =
    K^{id}_{1,1}(\X, \X)
\]
\end{proposition}



==> convergence.tex <==

\subsection{Convergence to $\varphi$-Signature Kernel}

\subsubsection{Preliminary Assumptions}

\begin{assumption}\label{assumption_linear_bound}
  Henceforth we are going to assume the nonlinearity $\varphi$ to be s.t.
  \[ | \varphi (x) | \leq M (1 + | x |) \]
\end{assumption}

\begin{assumption}\label{assumption:split_on_PSD_R}
  Henceforth we are going to assume the nonlinearity $\varphi$ to be such that
  the maps
  \begin{eqnarray*}
    & \Phi : \tmop{PSD}_2 (R) \rightarrow \R & \\
    & \Sigma \mapsto \mathbb{E}_{(Z_x, Z_y) \sim \mathcal{N} (0,
    \Sigma)} [\varphi (Z_x) \varphi (Z_y)] & 
  \end{eqnarray*}
  are, respectively, $\kappa_R$-Lipschitz i.e.
  \[
  |\Phi (\Sigma) - \Phi (\tilde{\Sigma})|  \leq  \kappa_R \| \Sigma -
    \tilde{\Sigma} \|_{\infty} 
  \]
\end{assumption}

\textcolor{orange}{TO DO: Explain under which circumstances this holds}

\begin{lemma}
  Under {\tmstrong{Assumption \ref{assumption_linear_bound}}} we have
  \[ | \Phi (\Sigma) | \leq \tilde{M} \left( 1 + \sqrt{[\Sigma]_1^1} \right)
     \left( 1 + \sqrt{[\Sigma]_2^2} \right) \]
\end{lemma}

\begin{proof}
  In fact given a PSD matrix $\Sigma \in \mathbb{R}^{2 \times 2}$ we have
  \[ \Sigma = A A^T \]
  where
  \[ A = \left(\begin{array}{c}
       \alpha, 0\\
       \beta \gamma, \beta \sqrt{1 - \gamma^2}
     \end{array}\right) \]
  with
  \[ \alpha = \sqrt{[\Sigma]_1^1}, \beta = \sqrt{[\Sigma]_2^2} \infixand
     \gamma = \frac{[\Sigma]_1^2}{\sqrt{[\Sigma]_1^1 [\Sigma]_2^2}} \]
  Then
  \begin{eqnarray*}
    \mathbb{E}_{(Z_x, Z_y) \sim \mathcal{N} (0, \Sigma)} [\varphi (Z_x)
    \varphi (Z_y)] & = & \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})}
    \left[ \varphi (\alpha Z_1) \varphi \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right]
  \end{eqnarray*}
  so that
\begin{equation*}
\resizebox{\hsize}{!}{$
\begin{gathered}
    | \Phi (\Sigma) |  =  \left| \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} \left[ \varphi (\alpha Z_1) \varphi \left( \beta \left( \gamma
    Z_1 + \sqrt{1 - \gamma^2} Z_2 \right) \right) \right] \right|
    \\
     \leq  \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} \left[ |
    \varphi (\alpha Z_1) | \left| \varphi \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right| \right]
    \\
     \leq  M^2 \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} \left[
    (1 + | (\alpha Z_1) |) \left( 1 + \left| \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right| \right) \right]
    \\
     =  M^2 \left[ 1 + \alpha \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} [| Z_1 |] + \beta \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} \left[ \left| \gamma Z_1 + \sqrt{1 - \gamma^2} Z_2 \right|
    \right]+ \alpha \beta \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})}
    \left[ | Z_1 | \left| \gamma Z_1 + \sqrt{1 - \gamma^2} Z_2 \right| \right]
    \right]
    \\
     \leq  M^2 \left[ 1 + (\alpha + \beta | \gamma |) \mathbb{E}_{Z
    \sim \mathcal{N} (0, \tmop{Id})} [| Z_1 |] + \beta \sqrt{1 -
    \gamma^2} \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} [| Z_2 |] +
    \alpha \beta | \gamma | \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} [| Z_1 |^2] + \alpha \beta \sqrt{1 - \gamma^2} \mathbb{E}_{Z
    \sim \mathcal{N} (0, \tmop{Id})} [| Z_1 Z_2 |] \right]
    \\
     \leq  \bar{M} \left( 1 + \alpha + \beta | \gamma | + \beta \sqrt{1 -
    \gamma^2} + \alpha \beta | \gamma | + \alpha \beta \sqrt{1 - \gamma^2}
    \right)
\end{gathered}
$}
\end{equation*}
  and using \tmcolor{orange}{$\tmcolor{black}{\gamma^2 \leq 1}$}
  \begin{eqnarray*}
    | \Phi (\Sigma) | & \leq & \tilde{M} (1 + \alpha + \beta + \alpha \beta) =
    \tilde{M} (1 + \alpha) (1 + \beta)
  \end{eqnarray*}
  
\end{proof}

\subsubsection{Fixing the Notation}

\begin{definition}
  Fix $\D \assign \{ 0 = t_0 < \cdots < t_{\| \D \|} = 1 \}$
  and $\D' \assign \{ 0 = s_0 < \cdots < s_{\| \D' \|} = 1
  \}$ partitions of $[0, 1]$, the interval where the paths $x, y$ are defined.
  We define
  \[ K^{\D \times \D'}_{x \comma y} : \D \times
     \D' \rightarrow \mathbb{R} \]
  as the map satisfying
  \begin{eqnarray*}
    & K^{\D \times \D'}_{x \comma y} (t_m, s_n) =
    K^{\D \times \D'}_{x \comma y} (t_{m - 1}, s_n) +
    K^{\D \times \D'}_{x \comma y} (t_m, s_{n - 1}) -
    K^{\D \times \D'}_{x \comma y} (t_m, s_{n - 1}) + & \\
    & \sum_{k = 1}^d \left( \sigma_A^2 \mathbb{E}_{\tmscript{(Z_x, Z_y)
    \sim \mathcal{N} \left( 0,  \Sigma_{\tmscript{x, y}}^{\D \times \D'} (t_{m - 1}, s_{n -
    1}) \right)}} [\varphi (Z_x) \varphi (Z_y)] + \sigma_b^2 \right)
    \Delta^{\D} x_{{t_m} }^k \Delta^{\D'} y_{s_n}^k & \\
    & = K^{\D \times \D'}_{x \comma y} (t_{m - 1}, s_n) +
    K^{\D \times \D'}_{x \comma y} (t_m, s_{n - 1}) -
    K^{\D \times \D'}_{x \comma y} (t_m, s_{n - 1}) + & \\
    & + \sum_{k = 1}^d \left( \sigma_A^2 \Phi \left(
    \Sigma_{{x, y}}^{\D \times \D'} (t_{m - 1}, s_{n -
    1}) \right) + \sigma_b^2 \right) \Delta^{\D} x_{{t_m} }^k
    \Delta^{\D'} y_{s_n}^k & \\
    & = \sigma^2_{S_0} + \sum_{\tmscript{\begin{array}{c}
      0 \leq k_1 < m\\
      0 \leq k_2 < n
    \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 \Phi \left(
    \Sigma_{\tmscript{ x, y}}^{\D \times \D'} (t_{k_1}, s_{k_2})
    \right) + \sigma_b^2 \right) \Delta^{\D} x_{{t_{k_1 + 1}} }^k
    \Delta^{\D'} y_{s_{k_2 + 1}}^k & 
  \end{eqnarray*}
  where
  \[ \Delta^{\D} x_{{t_m} }^k = (x^k_{t_m} - x^k_{t_{m - 1}}),
     \Delta^{\D'} y_{s_n}^l = (y^l_{s_n} - y^l_{s_{n - 1}}),
     K^{\D}_{0, s_n} (x, y) = K^{\D}_{t_m, 0} (x, y) =
     \sigma^2_{S_0} \]
  and
  \[ \Sigma_{\tmscript{\begin{array}{c}
       x, y
     \end{array}}}^{\D \times \D'} (t_m, s_n) =
     \left(\begin{array}{c}
       K^{\D \times \D}_{x, x} (t_m, t_m), K^{\D
       \times \D'}_{x, y} (t_m, s_n)\\
       K^{\D \times \D'}_{x, y} (t_m, s_n), K^{\D'
       \times \D'}_{y, y} (s_n, s_n)
     \end{array}\right) \]
\end{definition}

\begin{definition}
  $| \D | \assign \max  \{ t_{m + 1} - t_m : 0 \leq m < \|
  \D \| \}$ is the \emph{mesh size} of the partition.
\end{definition}

\begin{definition}
  We extend
  \begin{eqnarray*}
    & K^{\D \times \D'}_{x \comma y} : \D \times
    \D' \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  to
  \begin{eqnarray*}
    & K^{\D \times \D'}_{x \comma y} : [0, 1] \times [0, 1]
    \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  as
  \begin{eqnarray*}
    & K^{\D \times \D'}_{x \comma y} (t, s) =
    K^{\D \times \D'}_{x \comma y} (t_{m - 1}, s_n) +
    K^{\D \times \D'}_{x \comma y} (t_m, s_{n - 1}) -
    K^{\D \times \D'}_{x \comma y} (t_m, s_{n - 1}) & \\
    & + \int^t_{\tau = t_{m - 1}} \int^s_{\sigma = s_{n - 1}}
    \left( \sigma_A^2 \Phi \left( \Sigma_{\tmscript{x, y}}^{\D \times \D'} (t_{m - 1}, s_{n -
    1}) \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
  \end{eqnarray*}
  where $(t, s) \in [t_m - 1, t_m] \times [s_{n - 1}, s_n]$
  
  and to
  \begin{eqnarray*}
    & \tilde{K}^{\D \times \D'}_{x \comma y} : [0, 1]
    \times [0, 1] \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  as
  \begin{eqnarray*}
    \tilde{K}^{\D \times \D'}_{x \comma y} (t, s) & = &
    \left\{\begin{array}{l}
      K^{\D \times \D'}_{x \comma y} (t_m, s_n) \quad
      \tmop{if} \quad (t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times
      [s_n, s_{n + 1})\\
      K^{\D \times \D'}_{x \comma y} (1, s_n) \quad
      \tmop{if} \quad (t, s) \in \{ 1 \} \times [s_n, s_{n + 1})\\
      K^{\D \times \D'}_{x \comma y} (t_{m - 1}, 1) \quad
      \tmop{if} \quad (t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times \{ 1
      \}\\
      K^{\D \times \D'}_{x \comma y} (1, 1) \quad \tmop{if}
      \quad (t, s) = (1, 1)
    \end{array}\right.
  \end{eqnarray*}
  and similarly for $\tilde{\Sigma}_{\tmscript{x, y}}^{\D \times \D'} (t, s)$
\end{definition}

\begin{notation}
  For ease of notation, if clear from the context, we will write 
  \[ K_{t, s} : = K^{\D \times \D'} (t, s) : = K_{x \comma
     y} (t, s) : = K^{\D \times \D'}_{x \comma y} (t, s) \]
  and similarly for $\tilde{K}^{\D \times \D'}_{x \comma y}
  (t, s)$ and the covariance matrices.
\end{notation}

\begin{remark}
  Note then how, for $(t, s) \in [t_m - 1, t_m] \times [s_{n - 1}, s_n]$,
  \begin{eqnarray*}
    & K^{\D \times \D'}_{x \comma y} (t, s) =
    K^{\D \times \D'}_{x \comma y} (t_{m - 1}, s_n) +
    K^{\D \times \D'}_{x \comma y} (t_m, s_{n - 1}) -
    K^{\D \times \D'}_{x \comma y} (t_m, s_{n - 1}) + & \\
    & + \int^t_{\tau = t_{m - 1}} \int^s_{\sigma = s_{n - 1}} \left(
    \sigma_A^2 \Phi \left( \tilde{\Sigma}_{\tmscript{ x, y}}^{\D \times \D'} (\tau, \sigma)
    \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma & \\
    & = \sigma^2_{S_0} + \int^t_{\tau = 0} \int^s_{\sigma = 0} \left(
    \sigma_A^2 \Phi \left( \tilde{\Sigma}_{\tmscript{ x, y}}^{\D \times \D'} (\tau, \sigma)
    \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma & 
  \end{eqnarray*}
  
\end{remark}

Our goal is to prove the following result:

\begin{theorem} \label{simple_conv}
  As $| \D | \vee | \D' | \rightarrow 0$
  \ we have
  \[ K^{\D \times \D'}_{x, y} (t, s) \rightarrow K_{x, y}
     (t, s) \]
  where $K_{x, y} (t, s)$ satisfies
  \begin{eqnarray*}
    K_{x, y} (t, s) & = & \sigma^2_{S_0} +  \int_{\tau = 0}^t
    \int_{\sigma = 0}^s \left( \sigma_A^2 \mathbb{E}_{(Z_x, Z_y) \sim
    \mathcal{N} (0,  \Sigma_{x, y}^{} (t, s))} [\varphi (Z_x) \varphi (Z_y)] +
    \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma\\
    & = & \sigma^2_{S_0} +  \int_{\tau = 0}^t \int_{\sigma =
    0}^s (\sigma_A^2 \Phi (\Sigma_{x, y}^{} (t, s)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
  \end{eqnarray*}
  with
  \[ \Sigma_{x, y}^{} (t, s) = \left(\begin{array}{c}
       K_{x, x} (t, t), K_{x, y} (t, s)\\
       K_{x, y} (t, s), K_{y, y} (s, s)
     \end{array}\right) \]
\end{theorem}

The proof will rely on classic arguments used to prove convergence of Euler schemes to CDE solutions (see \cite{FrizVictoir} and \cite{EulerGoursat}).
Our setting is more complex than the ones we found in the literature though, this is due to the presence of two "independent" driving signals and on the unique nature of the driving fields, which not only depend on the "present" but also on "past" and "future". 
This complex dependency structure of the driving fields makes them completely non-local and requires more involved arguments for the solution to be made sense of.

\subsubsection{Preliminary Bounds}

Note that due to their definition as limiting kernels the $\tilde{\Sigma}^{\D \times
\D'}_{x \comma y}$ are always PSD. We are going to need a more quantitative result, in the form of a uniform membership in some $PSD(R)$, in order to later leverage Assumption \ref{assumption:split_on_PSD_R}.

We first prove such a result for the case $x = y$ and $\D = \D'$, the general case will follow easily.

The first "ingredient" is a uniform, in $x \in \bX$, bound from below of the kernels for $t=s$.

\begin{lemma}
  $\forall t \in \D. \quad \Tilde{K}^{\D \times \D}_{x, x}
  (t, t) \geq \sigma_{S_0}^2 $\quad for any choiche of $\D$.
\end{lemma}

\begin{proof}
  We have
  \[ K^{\D \times \D}_{x, x} (t_m, t_m) = \sigma^2_{S_0} +
     \sum_{\tmscript{\begin{array}{c}
       0 \leq k_1 < m\\
       0 \leq k_2 < m
     \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 \Phi \left(
     \Sigma_{\tmscript{x, x}}^{\D \times \D} (t_{k_1}, t_{k_2})
     \right) + \sigma_b^2 \right) \Delta^{\D} x_{{t_{k_1 + 1}} }^k
     \Delta^{\D} x_{t_{k_2 + 1}}^k \]
  and by Tensor Programs we know that
\begin{equation*}
\resizebox{\hsize}{!}{$
\begin{gathered}
\sum_{\tmscript{\begin{array}{c}
       0 \leq k_1 < m\\
       0 \leq k_2 < m
     \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 \Phi \left(
     \Sigma_{\tmscript{x, x}}^{\D \times \D} (t_{k_1}, t_{k_2})
     \right) + \sigma_b^2 \right) \Delta^{\D} x_{{t_{k_1 + 1}} }^k
     \Delta^{\D} x_{t_{k_2 + 1}}^k = \lim_{N \rightarrow \infty}
     \mathbb{E} \left[ \frac{\langle S_x^{N, \D} (x) - S^N_0, S_x^{N,
     \D} (x) - S^N_0 \rangle}{N} \right] \geq 0 
\end{gathered}
$}
\end{equation*}
  
\end{proof}

The second step is another bound, this time from above, which will be uniform on bounded subsets of $\bX$.

\begin{lemma}
  There is a constant $C_x > 0$ independent of $\D$ such that
  \[ \| \tilde{K}^{\D \times \D}_{x \comma x} \|_{\infty,
     [0, 1] \times [0, 1]} \assign \sup\limits_{(t, s) \in [0, 1]^2} |
     \tilde{K}^{\D \times \D}_{x \comma x} (t, s) | \leq C_x
  \]
  Moreover $C_x$ only depends on $\norm{x}_{1-var}$ and is increasing in it, thus there is a uniform bound on bounded subsets of $\bX$.
\end{lemma}

\begin{proof}
  Wlog $(t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times [s_n, s_{n + 1})$. Remember how
  \begin{eqnarray*}
    \tilde{K}^{\D \times \D}_{x \comma x} (t, s) & = &
    K^{\D \times \D}_{x \comma x} (t_m, s_n)\\
    & = & \sigma^2_{S_0} +  \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma =
    0} \left( \sigma_A^2 \Phi \left(
    \tilde{\Sigma}_{\tmscript{x, x}}^{\D \times \D} (\tau, \sigma) \right)
    + \sigma_b^2 \right)
    \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}   
    d\tau d\sigma
  \end{eqnarray*}
  thus
  \begin{eqnarray*}
    | \tilde{K}_{t, s} | & \leq & 
    \sigma^2_{S_0} + 
    \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    | \sigma_A^2 \Phi (\tilde{\Sigma}_{ \tau, \sigma})| 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma
    + \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    | \sigma_b^2 | 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma \\
    & = & \sigma^2_{S_0} + 
    \sigma_b^2 \norm{x}_{1-var, [0,t_m]}\norm{x}_{1-var, [0,s_n]} +
    \sigma_A^2 \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    |\Phi(\tilde{\Sigma}_{ \tau, \sigma})|  
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma \\
    & \leq & \sigma^2_{S_0} + 
    \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    \tilde{M} 
    \tmscript{\left(
    1 + \sqrt{\tilde{K}_{\tau, \tau}} \right) \left( 1 +
    \sqrt{\tilde{K}_{\sigma, \sigma}} \right)} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma\\
    & = & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \tilde{M} 
    \tmscript{\left( \int^{t_m}_{\tau = 0} \left( 1 +
    \sqrt{\tilde{K}_{\tau, \tau}} \right) |\Dot{x}_{\tau}| d\tau \right) 
    \left(\int^{s_n}_{\sigma = 0} \left( 1 + \sqrt{\tilde{K}_{\sigma, \sigma}}
    \right)  |\Dot{x}_{\sigma}| d\sigma \right)}
  \end{eqnarray*}
  In particular
  \begin{eqnarray*}
    \tilde{K}_{t, t} = | \tilde{K}_{t, t} | & \leq & \sigma^2_{S_0} +
    \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} + \sigma_A^2 \tilde{M}
    \left| \int^{t_m}_{\tau = 0} \left( 1 +
    \sqrt{\tilde{K}_{\tau, \tau}} \right) |\Dot{x}_{\tau}| d\tau
    \right|^2\\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \tilde{M}  \| x \|_{1 - \tmop{var}, [0, t_m]}
    \tmscript{
    \left( \int^{t_m}_{\tau = 0} \left( 1 + \sqrt{\tilde{K}_{\tau, \tau}}
    \right)^2 |\Dot{x}_{\tau}| d\tau \right)}\\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    2 \sigma_A^2 \tilde{M} \| x \|_{1 - \tmop{var}, [0, 1]} 
    \int^{t_m}_{\tau = 0} (1 + \tilde{K}_{\tau, \tau}) 
    |\Dot{x}_{\tau}| d\tau \\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    2 \sigma_A^2 \tilde{M} \| x \|_{1 - \tmop{var}, [0, 1]}
    \int^t_{\tau = 0} (1 + \tilde{K}_{\tau, \tau}) 
    |\Dot{x}_{\tau}| d\tau
  \end{eqnarray*}
  
  
  and we can use Gronwall Inequality (\cite{FrizVictoir}, Lemma 3.2) to
  obtain
  \begin{eqnarray*}
    1 + \tilde{K}_{t, t} & \leq & (1 + \sigma^2_{S_0} + \sigma_b^2 \| x
    \|^2_{1 - \tmop{var}, [0, 1]}) \exp \{ 2 \sigma_A^2 \tilde{M} \| x \|^2_{1
    - \tmop{var}, [0, 1]} \}
  \end{eqnarray*}
  hence the thesis with
  \begin{eqnarray*}
    C_x & = & (1 + \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0,
    1]}) {e^{2 \sigma_A^2 \tilde{M} \| x \|^2_{1 - \tmop{var}, [0, 1]}}}  - 1
  \end{eqnarray*}
  
\end{proof}

Thus finally we can conclude, as promised, that

\begin{lemma}
  There is an $R = R_x \in \mathbb{R}$ such that $\tilde{\Sigma}^{\D \times
  \D}_{x \comma x}, \Sigma^{\D \times \D}_{x \comma
  x} \in \tmop{PSD} (R)$ for every $\D$.
  Moreover, as before, this $R_x$ only depends on $\norm{x}_{1-var}$ and is increasing in it. 
\end{lemma}

\begin{proof}
  The diagonal elements $K^{\D \times \D}_{x,x}(t , t)$ are
  bounded above by a common constant $C_x$ and below by $\sigma^2_{S_0}$. 
  We thus can simply choose $R_x = C_x \vee \sigma^{-2}_{S_0}$.
\end{proof}

We are ready to extend the result to the general case.

\begin{proposition}\label{prop:bounded_set_bounds}
    Fix a $\alpha > 0$. There exist a constant $C_{\alpha}$ such that for all $x,y \in \bX$ with $\norm{x}_{1-var}, \norm{y}_{1-var} \leq \alpha$ and partitions $\D, \D'$ it holds
    \[
        \sup_{0 \leq t, s \leq 1} \nobracket | \nobracket K^{\D \times
        \D^{'}}_{x \comma y} (t, s) | \leq C_{\alpha} 
    \]
    Moreover for $R_{\alpha} := C_{\alpha} \vee \sigma^{-2}_{S_0}$ we get 
    \[
        \Sigma^{\D \times \D'}_{x \comma y} (t, s) \in \tmop{PSD}(R_{\alpha}) 
    \]
\end{proposition}


\begin{proof}
Remember how the maps $\Sigma^{\D \times \D'}_{x \comma y}$
are  PSD since they arise as such from Tensor limiting arguments, in particular by positive semidefinitiveness 
and the previous bounds
\begin{eqnarray*}
\nobracket | \nobracket \tilde{K}^{\D \times \D'}_{x
\comma y} (t, s) | \leq \sqrt{\tilde{K}^{\D \times
\D}_{x \comma x} (t, t) \tilde{K}^{\D' \times
\D'}_{y \comma y} (s, s)} \leq \sqrt{C_x C_y} \leq C_x \vee C_y \leq C_{\alpha}
&  & 
\end{eqnarray*}

The second part follows from the definition of $\tmop{PSD}(R_{\alpha})$.
\end{proof}

\subsubsection{Main body of the proof}

We are now ready to prove Theorem \ref{simple_conv}.

\begin{proof} (Theorem \ref{simple_conv})
\vspace{5pt}
  \newline
  \textit{- Roadmap}
  
  The central idea will be proving that, given any sequence $\D_n \times \D'_n$ with $|\D_n| \vee |\D'_n| \downarrow 0$, the maps $\{ K^{\D_n \times \D'_n}_{x, y} \}_{n}$ form a Cauchy sequence in the Banch space $(C^0 ([0, 1] \times [0, 1] ; \mathbb{R}), \| \cdot \|_{\infty})$. By completeness of this space the sequence will admit a limit $K_{x, y}$, which we will prove to be independent from the chosen sequence. Finally we will prove that this limit is the sought after kernel.

  Note that trivially the set $\{x,y\}$ is bounded in $\bX$, we can thus fix two constants $C_{x,y}, R_{x,y}$ with the properties given in Proposition \ref{prop:bounded_set_bounds}. We will often, for ease of notation, refer to them as $C$ and $R$.

  \textit{- Part I : how close are $K^{\D \times \D'}$ and $\tilde{K}^{\D \times \D'}$ ?}
  
  We have
  \begin{eqnarray*}
    | K^{\D \times \D'}_{x, y} (t, s) -
    \tilde{K}^{\D \times \D'}_{x, y} (t, s) | & = & |
    \nobracket \int^t_{\tau = 0} \int^s_{\sigma = 0} (\sigma_A^2 \Phi
    (\widetilde{\Sigma }^{\D \times \D'}_{ x, y} (\tau,
    \sigma)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma\\
    &  & - \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} (\sigma_A^2 \Phi
    (\widetilde{\Sigma }^{\D \times \D'}_{ x, y} (\tau,
    \sigma)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma | \nobracket\\
    & = & \left| \int_{\Omega_{t, s}} (\sigma_A^2 \Phi (\widetilde{\Sigma
    }^{\D \times \D'}_{ x, y} (\tau, \sigma)) + \sigma_b^2)
    \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma \right|
  \end{eqnarray*}
  with
  \[ \Omega_{t, s} \assign [0, t] \times [0, s] \setminus [0, t_m] \times [0,
     s_n] \]
  Note that
  \[ \Omega_{t, s} \subseteq ([t_{m,} t_{m + 1}] \times [0, 1]) \cup ([0, 1]
     \times [s_n, s_{n + 1}]) \]
  thus
  \[ \mathcal{L}^2 (\Omega_{t, s}) \leq | \D | + | \D' |
     \leq 2 (| \D | \vee | \D' |) \]
  hence
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    | K^{\D \times \D'}_{x, y} (t, s) -
    \tilde{K}^{\D \times \D'}_{x, y} (t, s) |  \leq 
    \int_{\Omega_{t, s}} | \sigma_A^2 \Phi (\widetilde{\Sigma }^{\D
    \times \D'}_{ x, y} (\tau, \sigma)) + \sigma_b^2 |  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma
    \\
     \leq  \sigma_A^2 \int_{\Omega_{t, s}} \tilde{M} 
    \tmscript{\left( 1 +
    \sqrt{K^{\D \times \D}_{x, x} (\tau \comma \tau)}
    \right) \left( 1 + \sqrt{K^{\D' \times \D'}_{y, y}
    (\sigma \comma \sigma)} \right)} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma
       + \sigma_b^2 \int_{\Omega_{t, s}} 
       |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
       d\tau d\sigma\\
     \leq  \sigma_A^2 \tilde{M} \left( 1 + \sqrt{C_{x, y}} \right)^2
    \int_{\Omega_{t, s}} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
    d\tau d\sigma 
    + \sigma_b^2
    \int_{\Omega_{t, s}} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|      
    d\tau d\sigma\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) \int_{[0, 1]
    \times [0, 1]} \mathbb{I}_{\Omega_{t, s}} (\tau, \sigma) 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
    d\tau d\sigma\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\int_{[0, 1] \times [0, 1]} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|^2       
    d\tau d\sigma}\\
    \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\int_{[0, 1] \times [0, 1]} 
    |\Dot{x}_{\tau}|^2 |\Dot{y}_{\sigma}|^2       
    d\tau d\sigma}\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}}\\
     \leq  2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\D | \vee | \D' |} 
     \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}}
  \end{gathered} $} \end{equation*}
  
  In particular as $(| \D | \vee | \D' |) \rightarrow 0$ we
  have
    \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \sup_{[0, 1] \times [0, 1]} | K^{\D \times \D'}_{x, y}
     (t, s) - \tilde{K}^{\D \times \D'}_{x, y} (t, s) | \leq
     2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)   
     \sqrt{|\D | \vee | \D' |} 
     \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}} \rightarrow 0
     \end{gathered} $} \end{equation*}
  
  
  Notice that, since we can repeat the argument for $K^{\D \times
  \D}_{x, x}$ and $K^{\D' \times \D'}_{y, y}$, we have
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
  \sup_{[0, 1] \times [0, 1]} | \Sigma^{\D \times \D'}_{ 
     x, y} (t, s) - \tilde{\Sigma}^{\D \times \D'}_{  x, y}
     (t, s) |_{\infty} \leq 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) +
     \sigma_b^2) 
     \sqrt{|\D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
  \end{gathered} $} \end{equation*}

  \textit{- Part II : Cauchy Bounds}
  
  Consider now another partition $\check{\D} \times
  \check{\D}'$, we have
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    | K^{\check{\D} \times \check{\D}'}_{x, y} (t, s) -
    K^{\D \times \D'}_{x, y} (t, s) |  =  \left|
    \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} [\Phi
    (\tilde{\Sigma}^{\check{\D} \times \check{\D}'}_{  x, y}
    (\tau, \sigma)) - \Phi (\tilde{\Sigma}^{\D \times \D'}_{
    x, y} (\tau, \sigma))] \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma 
    \right|\\
     \leq  \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} | \Phi
    (\tilde{\Sigma}^{\check{\D} \times \check{\D}'}_{  x, y}
    (\tau, \sigma)) - \Phi (\tilde{\Sigma}^{\D \times \D'}_{
    x, y} (\tau, \sigma)) |  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} k_R |
    \tilde{\Sigma}^{\check{\D} \times \check{\D}'}_{  x, y}
    (\tau, \sigma) - \tilde{\Sigma}^{\D \times \D'}_{  x, y}
    (\tau, \sigma) |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\check{\D} \times \check{\D}'}_{  \tau,
    \sigma} - \Sigma^{\check{\D} \times \check{\D}'}_{ 
    \tau, \sigma} |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\check{\D} \times \check{\D}'}_{  \tau, \sigma}
    - \Sigma^{\D \times \D'}_{  \tau, \sigma} |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\D \times \D'}_{  \tau, \sigma} -
    \tilde{\Sigma}^{\D \times \D'}_{  \tau, \sigma}
    |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\check{\D} | \vee | \check{\D}'|}  
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    \int^t_{\tau = 0} \int^s_{\sigma = 0}  
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\check{\D} \times \check{\D}'}_{  \tau, \sigma}
    - \Sigma^{\D \times \D'}_{  \tau, \sigma} |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\D | \vee | \D' |}
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
     \int^t_{\tau = 0} \int^s_{\sigma = 0} 
     |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
     (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})
    \\
       + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma =
    0} | \Sigma^{\check{\D} \times \check{\D}'}_{  x, y}
    (\tau, \sigma) - \Sigma^{\D \times \D'}_{  x, y} (\tau,
    \sigma) |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{gathered} $} \end{equation*}


  \vspace{3pt}
  Assume to be in the case $x=y$, $\D = \D'$, $\check{\D} = \check{\D}'$ and define the following quantity:
  \[
  \Xi_t \assign 
  \sup_{0 \leq \tau, \sigma \leq t} | \Sigma^{\check{\D} \times \check{\D}}_{x,x}({\tau, \sigma}) - \Sigma^{\D \times \D}_{x,x}({\tau, \sigma}) |_{\infty} = 
  \sup_{0 \leq \tau, \sigma \leq t} |K^{\check{\D} \times \check{\D}}_{x,x}({\tau, \sigma}) - K^{\D \times \D}_{x,x}({\tau, \sigma})|
  \]

  One has, from the previous inequality, that
  \begin{eqnarray*}
    \Xi_t &
    \leq & 4 \sigma_A^2 \left( 2 \sigma_A^2 \tilde{M} \left( {1 + C_x} 
    \right) + \sigma_b^2 \right) 
    \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\D} | \vee |\D |}\\
    &  & + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^t_{\sigma =
    0} | \Sigma^{\check{\D} \times \check{\D}}_{  \tau,
    \sigma} - \Sigma^{\D \times \D}_{  \tau, \sigma}
    |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{eqnarray*}
  and since
  \begin{eqnarray*}
    & \int^t_{\tau = 0} \int^t_{\sigma = 0} | \Sigma^{\check{\D}
    \times \check{\D}}_{  \tau, \sigma} - \Sigma^{\D \times
    \D}_{  \tau, \sigma} |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma
    \leq \int^t_{\tau = 0} \int^t_{\sigma = 0} \Xi_{\tau \vee
    \sigma} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma & \\
    & = \int^t_{\tau = 0} \int^{\tau}_{\sigma = 0} \Xi_{\tau} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma
    + \int^t_{\tau = 0} \int^t_{\sigma = \tau}
    \Xi_{\sigma} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}| d\tau d\sigma & \\
    & \leq  \int^t_{\tau = 0}  \| x \|_{1 - \tmop{var},
    [0, \tau]} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
    +  \int^t_{\sigma = 0} \int^{\sigma}_{\tau = 0} 
    \Xi_{\sigma} 
    |\Dot{x}_{\tau} | |\Dot{x}_{\sigma} | d\tau d\sigma 
    & \\
    & = \int^t_{\tau = 0}  \| x \|_{1 - \tmop{var},
    [0, \tau]} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
    + \int^t_{\sigma = 0}  \| x \|_{1 - \tmop{var},
    [0, \sigma]} \Xi_{\sigma} |\Dot{x}_{\sigma} | d\sigma  & \\
    & \leq 2 \| x \|_{1 - \tmop{var}, [0, 1]} 
     \int^t_{\tau = 0} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau & 
  \end{eqnarray*}
  we get
  \begin{eqnarray*}
    {\Xi_t}  & \leq & 4 \sigma_A^2 \left( 2 \sigma_A^2 \tilde{M} \left( {1 + C_x} 
    \right) + \sigma_b^2 \right) 
    \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\D} | \vee |\D |}\\
    &  & + 2 \sigma_A^2 k_R \| x \|_{1 - \tmop{var}, [0, 1]} 
    \int^t_{\tau = 0} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
  \end{eqnarray*}
  thus, by Gronwall,
  \[ \Xi_t \leq 4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2)
     \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\D} | \vee |\D |}
      \cdot e^{2 \sigma_A^2 k_R \| x \|_{1 - \tmop{var}, [0, 1]}^2 }
      \]

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \vspace{5pt}
  Coming back to the general case, we can now say that
  
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \Xi^{x, y}_t \assign \sup_{0 \leq \tau, \sigma \leq t} |
    \Sigma^{\check{\D} \times \check{\D}'}_{  \tau, \sigma}
    - \Sigma^{\D \times \D'}_{  \tau, \sigma} |_{\infty} \\
    \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})
    (1 +  e^{2 \sigma_A^2 k_R (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]}) })\\
       + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^t_{\sigma =
    0} | \Sigma^{\check{\D} \times \check{\D}'}_{  \tau,
    \sigma} - \Sigma^{\D \times \D'}_{  \tau, \sigma}|_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{gathered} $} \end{equation*}
  and since
  \begin{eqnarray*}
    & \int^t_{\tau = 0} \int^t_{\sigma = 0} 
    | \Sigma^{\check{\D} \times \check{\D}'}_{  \tau, \sigma} 
    - \Sigma^{\D \times \D'}_{  \tau, \sigma} |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma 
    \leq \int^t_{\tau = 0} \int^t_{\sigma = 0} {\Xi^{x, y}_{\tau
    \vee \sigma}}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma & \\
    & = \int^t_{\tau = 0} \int^{\tau}_{\sigma = 0} 
    \Xi^{x, y}_{\tau} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma 
    + \int^t_{\tau = 0} \int^t_{\sigma =\tau} 
    \Xi^{x, y}_{\sigma}
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma & \\
    & \leq 
    \int^t_{\tau = 0} \| y \|_{1 - \tmop{var}, [0, \tau]} 
    \Xi^{x, y}_{\tau} |\Dot{x}_{\tau}| d\tau 
    +  \int^t_{\sigma = 0} \int^{\sigma}_{\tau = 0} 
    \Xi^{x, y}_{\sigma} 
    |\Dot{x}_{\tau}| |\Dot{y}_{\sigma}| d\tau  d\sigma  & \\
    & = \int^t_{\tau = 0} \| y \|_{1 - \tmop{var}, [0, \tau]} 
    \Xi^{x, y}_{\tau} |\Dot{x}_{\tau}| d\tau 
    +  \int^t_{\sigma = 0} \| x \|_{1 - \tmop{var}, [0, \sigma]} 
    \Xi^{x,y}_{\sigma} |\Dot{y}_{\sigma}| d\sigma & \\
    & \leq (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1 - \tmop{var},[0, 1]}) 
    \int^t_{\tau = 0} \Xi^{x, y}_{\tau} (|\Dot{x}_{\tau}| +|\Dot{y}_{\tau}|) d\tau  & 
  \end{eqnarray*}
  we get
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \Xi^{x, y}_t  \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})
    (1 +  e^{2 \sigma_A^2 k_R (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]}) })\\
     + 2 \sigma_A^2 k_R (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1
    - \tmop{var}, [0, 1]}) \int^t_{\tau = 0} \Xi^{x, y}_{\tau} (|\Dot{x}_{\tau}| +|\Dot{y}_{\tau}|) d\tau
  \end{gathered} $} \end{equation*}
  thus, by Gronwall,
 \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \Xi_t  \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})
    (1 +  e^{2 \sigma_A^2 k_R (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]}) })\\
     \cdot e^{2 \sigma_A^2 k_R (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \|
    y \|_{1 - \tmop{var}, [0, 1]}) {(\| x \|_{1 - \tmop{var},
    [0, t]} + \| y \|_{1 - \tmop{var}, [0, t]})}}
  \end{gathered} $} \end{equation*}
  hence
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
     \| K^{\check{\D} \times \check{\D}'}_{x, y} (t, s) -
    K^{\D \times \D'}_{x, y} (t, s) \|_{\infty, [0, 1]^2} \leq
    \\
    4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\D} | \vee | \check{\D}'| \vee | \D | \vee | \D' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    \norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]})\\
    \cdot
    (1 +  e^{2 \sigma_A^2 k_R (\norm{x}^2_{1 - \tmop{var}, [0, 1]} \vee \norm{y}^2_{1 - \tmop{var}, [0, 1]}) })
    \cdot e^{{4 \sigma_A^2 k_R (\| x
    \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1 - \tmop{var}, [0, 1]})}} 
  \end{gathered} $} \end{equation*}

  \textit{- Part III : Existence and Uniqueness of limit}
  
  Given any sequence of partitions $\{ \D_n \times \D'_n \}$ with $| \D_n | \vee | \D_n' | \rightarrow 0$, due to the bounds we have just proven we have
  \[ 
     \{ K^{\D_n \times \D'_n}_{x , y} \} \tmop{is} a
     \tmop{Cauchy} \tmop{sequence} \tmop{in} (C^0 ([0, 1] \times [0, 1] ;
     \mathbb{R}), \| \cdot \|_{\infty}) 
  \]
  and the limit $K_{x, y}$ does not depend on the sequence (i.e. the limit
  exists and is unique). 

  The limit is indeed unique: assume $K_{x, y}$ and $G_{x, y}$ are limits along two different sequences of partitions $\{ \D_n \times \D'_n \}$ and $\{ \mathcal{G}_n \times \mathcal{G}'_n \}$; then the sequence $\{ \mathcal{P}_n \times \mathcal{P}'_n \}$ such that $\mathcal{P}_{2n} \times \mathcal{P}'_{2n} := \D_n \times \D'_n $ and $\mathcal{P}_{2n + 1} \times \mathcal{P}'_{2n + 1} := \mathcal{G}_n \times \mathcal{G}'_n$ is still such that $| \mathcal{P}_n | \vee | \mathcal{P}'_n | \rightarrow 0$ hence the associated kernels have a limit which must be equal to both $K_{x, y}$ and $G_{x, y}$.
  
  Since PSD matrices form a closed set we moreover have that the matrices $\Sigma_{x, y} (t, s)$
  obtained as limits using the previous result are all PSD. We can actually say more: they belong to $\tmop{PSD} (R)$.


  \textit{- Part IV : Existence and Uniqueness of limit} 

  We can finally conclude by proving that  $K_{x, y}$ is, in fact,  a solution of the PDE:
 \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
     \left| K_{x, y} (t, s) - \sigma^2_{S_0} + \int_{\tau = 0}^t
    \int_{\sigma = 0}^s (\sigma_A^2 \Phi (\Sigma_{x, y}^{} (\tau, \sigma)) +
    \sigma_b^2) 
    \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma   \right|  \\
    \leq  | K_{x, y} (t, s) - K^{\D \times \D'}_{x, y} (t,
    s) | + \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} | \Phi
    (\tilde{\Sigma}^{\D \times \D'}_{  x, y} (\tau, \sigma))
    - \Phi (\Sigma_{x, y}^{} (\tau, \sigma)) |  
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma  \\
    \leq  o (1) + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\D \times \D'}_{  x, y} (\tau, \sigma) -
    \Sigma_{x, y}^{} (\tau, \sigma) |_{\infty} 
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma\\
    \leq  o (1) + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\D \times \D'}_{  x, y} (\tau, \sigma) -
    \Sigma^{\D \times \D'}_{  x, y} (\tau, \sigma)
    |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma  \\
     + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\D \times \D'}_{  x, y} (\tau, \sigma) -
    \Sigma_{x, y}^{} (\tau, \sigma) |_{\infty}  
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma \\
    =  o (1) + o (1) + o (1) = o (1)  
   \end{gathered} $} \end{equation*}
  thus
  \[ \left| K_{x, y} (t, s) - \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma
     = 0}^s (\sigma_A^2 \Phi (\Sigma_{x, y}^{} (\tau, \sigma)) + \sigma_b^2) 
     \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma\right| = 0 \]
  i.e
  \[ K_{x, y} (t, s) = \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma = 0}^s
     (\sigma_A^2 \Phi (\Sigma_{x, y}^{} (\tau, \sigma)) + \sigma_b^2) 
     \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma\]
\end{proof}


\begin{remark}
    Note that, once again, the bounds we have just proven only depend on the norms of the paths, this time both the 1-var norm and the $W^{1,2}$ norm, and they do so in an increasing manner. This means that we have uniform convergence rates on bounded sets.
\end{remark}



==> old_convergence.tex <==

\subsection{Convergence to $\varphi$-Signature Kernel}

\begin{assumption}\label{assumption_linear_bound}
  Henceforth we are going to assume the nonlinearity $\varphi$ to be s.t.
  \[ | \varphi (x) | \leq M (1 + | x |) \]
\end{assumption}

\begin{assumption}
  Henceforth we are going to assume the nonlinearity $\varphi$ to be such that
  the maps
  \begin{eqnarray*}
    & \Phi : \tmop{PSD}_2 (R) \rightarrow \R & \\
    & \Sigma \mapsto \mathbb{E}_{(Z_x, Z_y) \sim \mathcal{N} (0,
    \Sigma)} [\varphi (Z_x) \varphi (Z_y)] & 
  \end{eqnarray*}
  are, respectively, $\kappa_R$-Lipschitz i.e.
  \[
  |\Phi (\Sigma) - \Phi (\tilde{\Sigma})|  \leq  \kappa_R \| \Sigma -
    \tilde{\Sigma} \|_{\infty} 
  \]
\end{assumption}

\begin{lemma}
  Under {\tmstrong{Assumption \ref{assumption_linear_bound}}} we have
  \[ | \Phi (\Sigma) | \leq \tilde{M} \left( 1 + \sqrt{[\Sigma]_1^1} \right)
     \left( 1 + \sqrt{[\Sigma]_2^2} \right) \]
\end{lemma}

\begin{proof}
  In fact given a PSD matrix $\Sigma \in \mathbb{R}^{2 \times 2}$ we have
  \[ \Sigma = A A^T \]
  where
  \[ A = \left(\begin{array}{c}
       \alpha, 0\\
       \beta \gamma, \beta \sqrt{1 - \gamma^2}
     \end{array}\right) \]
  with
  \[ \alpha = \sqrt{[\Sigma]_1^1}, \beta = \sqrt{[\Sigma]_2^2} \infixand
     \gamma = \frac{[\Sigma]_1^2}{\sqrt{[\Sigma]_1^1 [\Sigma]_2^2}} \]
  Then
  \begin{eqnarray*}
    \mathbb{E}_{(Z_x, Z_y) \sim \mathcal{N} (0, \Sigma)} [\varphi (Z_x)
    \varphi (Z_y)] & = & \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})}
    \left[ \varphi (\alpha Z_1) \varphi \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right]
  \end{eqnarray*}
  so that
\begin{equation*}
\resizebox{\hsize}{!}{$
\begin{gathered}
    | \Phi (\Sigma) |  =  \left| \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} \left[ \varphi (\alpha Z_1) \varphi \left( \beta \left( \gamma
    Z_1 + \sqrt{1 - \gamma^2} Z_2 \right) \right) \right] \right|
    \\
     \leq  \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} \left[ |
    \varphi (\alpha Z_1) | \left| \varphi \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right| \right]
    \\
     \leq  M^2 \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} \left[
    (1 + | (\alpha Z_1) |) \left( 1 + \left| \left( \beta \left( \gamma Z_1 +
    \sqrt{1 - \gamma^2} Z_2 \right) \right) \right| \right) \right]
    \\
     =  M^2 \left[ 1 + \alpha \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} [| Z_1 |] + \beta \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} \left[ \left| \gamma Z_1 + \sqrt{1 - \gamma^2} Z_2 \right|
    \right]+ \alpha \beta \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})}
    \left[ | Z_1 | \left| \gamma Z_1 + \sqrt{1 - \gamma^2} Z_2 \right| \right]
    \right]
    \\
     \leq  M^2 \left[ 1 + (\alpha + \beta | \gamma |) \mathbb{E}_{Z
    \sim \mathcal{N} (0, \tmop{Id})} [| Z_1 |] + \beta \sqrt{1 -
    \gamma^2} \mathbb{E}_{Z \sim \mathcal{N} (0, \tmop{Id})} [| Z_2 |] +
    \alpha \beta | \gamma | \mathbb{E}_{Z \sim \mathcal{N} (0,
    \tmop{Id})} [| Z_1 |^2] + \alpha \beta \sqrt{1 - \gamma^2} \mathbb{E}_{Z
    \sim \mathcal{N} (0, \tmop{Id})} [| Z_1 Z_2 |] \right]
    \\
     \leq  \bar{M} \left( 1 + \alpha + \beta | \gamma | + \beta \sqrt{1 -
    \gamma^2} + \alpha \beta | \gamma | + \alpha \beta \sqrt{1 - \gamma^2}
    \right)
\end{gathered}
$}
\end{equation*}
  and using \tmcolor{orange}{$\tmcolor{black}{\gamma^2 \leq 1}$}
  \begin{eqnarray*}
    | \Phi (\Sigma) | & \leq & \tilde{M} (1 + \alpha + \beta + \alpha \beta) =
    \tilde{M} (1 + \alpha) (1 + \beta)
  \end{eqnarray*}
  
\end{proof}

\begin{definition}
  Fix $\mathcal{D} \assign \{ 0 = t_0 < \cdots < t_{\| \mathcal{D} \|} = 1 \}$
  and $\mathcal{D}' \assign \{ 0 = s_0 < \cdots < s_{\| \mathcal{D}' \|} = 1
  \}$ partitions of $[0, 1]$, the interval where the paths $x, y$ are defined.
  We define
  \[ K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} : \mathcal{D} \times
     \mathcal{D}' \rightarrow \mathbb{R} \]
  as the map satisfying
  \begin{eqnarray*}
    & K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_n) =
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_{m - 1}, s_n) +
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_{n - 1}) -
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_{n - 1}) + & \\
    & \sum_{k = 1}^d \left( \sigma_A^2 \mathbb{E}_{\tmscript{(Z_x, Z_y)
    \sim \mathcal{N} \left( 0,  \Sigma_{\tmscript{x, y}}^{\mathcal{D} \times \mathcal{D}'} (t_{m - 1}, s_{n -
    1}) \right)}} [\varphi (Z_x) \varphi (Z_y)] + \sigma_b^2 \right)
    \Delta^{\mathcal{D}} x_{{t_m} }^k \Delta^{\mathcal{D}'} y_{s_n}^k & \\
    & = K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_{m - 1}, s_n) +
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_{n - 1}) -
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_{n - 1}) + & \\
    & + \sum_{k = 1}^d \left( \sigma_A^2 \Phi \left(
    \Sigma_{{x, y}}^{\mathcal{D} \times \mathcal{D}'} (t_{m - 1}, s_{n -
    1}) \right) + \sigma_b^2 \right) \Delta^{\mathcal{D}} x_{{t_m} }^k
    \Delta^{\mathcal{D}'} y_{s_n}^k & \\
    & = \sigma^2_{S_0} + \sum_{\tmscript{\begin{array}{c}
      0 \leq k_1 < m\\
      0 \leq k_2 < n
    \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 \Phi \left(
    \Sigma_{\tmscript{ x, y}}^{\mathcal{D} \times \mathcal{D}'} (t_{k_1}, s_{k_2})
    \right) + \sigma_b^2 \right) \Delta^{\mathcal{D}} x_{{t_{k_1 + 1}} }^k
    \Delta^{\mathcal{D}'} y_{s_{k_2 + 1}}^k & 
  \end{eqnarray*}
  where
  \[ \Delta^{\mathcal{D}} x_{{t_m} }^k = (x^k_{t_m} - x^k_{t_{m - 1}}),
     \Delta^{\mathcal{D}'} y_{s_n}^l = (y^l_{s_n} - y^l_{s_{n - 1}}),
     K^{\mathcal{D}}_{0, s_n} (x, y) = K^{\mathcal{D}}_{t_m, 0} (x, y) =
     \sigma^2_{S_0} \]
  and
  \[ \Sigma_{\tmscript{\begin{array}{c}
       x, y
     \end{array}}}^{\mathcal{D} \times \mathcal{D}'} (t_m, s_n) =
     \left(\begin{array}{c}
       K^{\mathcal{D} \times \mathcal{D}}_{x, x} (t_m, t_m), K^{\mathcal{D}
       \times \mathcal{D}'}_{x, y} (t_m, s_n)\\
       K^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t_m, s_n), K^{\mathcal{D}'
       \times \mathcal{D}'}_{y, y} (s_n, s_n)
     \end{array}\right) \]
\end{definition}

\begin{definition}
  $| \mathcal{D} | \assign \max  \{ t_{m + 1} - t_m : 0 \leq m < \|
  \mathcal{D} \| \}$ is the \emph{mesh size} of the partition.
\end{definition}

\begin{definition}
  We extend
  \begin{eqnarray*}
    & K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} : \mathcal{D} \times
    \mathcal{D}' \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  to
  \begin{eqnarray*}
    & K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} : [0, 1] \times [0, 1]
    \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  as
  \begin{eqnarray*}
    & K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t, s) =
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_{m - 1}, s_n) +
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_{n - 1}) -
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_{n - 1}) & \\
    & + \int^t_{\tau = t_{m - 1}} \int^s_{\sigma = s_{n - 1}}
    \left( \sigma_A^2 \Phi \left( \Sigma_{\tmscript{x, y}}^{\mathcal{D} \times \mathcal{D}'} (t_{m - 1}, s_{n -
    1}) \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
  \end{eqnarray*}
  where $(t, s) \in [t_m - 1, t_m] \times [s_{n - 1}, s_n]$
  
  and to
  \begin{eqnarray*}
    & \tilde{K}^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} : [0, 1]
    \times [0, 1] \rightarrow \mathbb{R} & 
  \end{eqnarray*}
  as
  \begin{eqnarray*}
    \tilde{K}^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t, s) & = &
    \left\{\begin{array}{l}
      K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_n) \quad
      \tmop{if} \quad (t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times
      [s_n, s_{n + 1})\\
      K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (1, s_n) \quad
      \tmop{if} \quad (t, s) \in \{ 1 \} \times [s_n, s_{n + 1})\\
      K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_{m - 1}, 1) \quad
      \tmop{if} \quad (t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times \{ 1
      \}\\
      K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (1, 1) \quad \tmop{if}
      \quad (t, s) = (1, 1)
    \end{array}\right.
  \end{eqnarray*}
  and similarly for $\tilde{\Sigma}_{\tmscript{x, y}}^{\mathcal{D} \times \mathcal{D}'} (t, s)$
\end{definition}

\begin{notation}
  For ease of notation, if clear from the context, we will write 
  \[ K_{t, s} : = K^{\mathcal{D} \times \mathcal{D}'} (t, s) : = K_{x \comma
     y} (t, s) : = K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t, s) \]
  and similarly for $\tilde{K}^{\mathcal{D} \times \mathcal{D}'}_{x \comma y}
  (t, s)$ and the covariance matrices.
\end{notation}

\begin{remark}
  Note then how, for $(t, s) \in [t_m - 1, t_m] \times [s_{n - 1}, s_n]$,
  \begin{eqnarray*}
    & K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t, s) =
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_{m - 1}, s_n) +
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_{n - 1}) -
    K^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t_m, s_{n - 1}) + & \\
    & + \int^t_{\tau = t_{m - 1}} \int^s_{\sigma = s_{n - 1}} \left(
    \sigma_A^2 \Phi \left( \tilde{\Sigma}_{\tmscript{ x, y}}^{\mathcal{D} \times \mathcal{D}'} (\tau, \sigma)
    \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma & \\
    & = \sigma^2_{S_0} + \int^t_{\tau = 0} \int^s_{\sigma = 0} \left(
    \sigma_A^2 \Phi \left( \tilde{\Sigma}_{\tmscript{ x, y}}^{\mathcal{D} \times \mathcal{D}'} (\tau, \sigma)
    \right) + \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma & 
  \end{eqnarray*}
  
\end{remark}

Our goal is to prove the following result:

\begin{proposition}
  \label{simple_conv}As $| \mathcal{D} | \vee | \mathcal{D}' | \rightarrow 0$
  \ we have
  \[ K^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t, s) \rightarrow K_{x, y}
     (t, s) \]
  where $K_{x, y} (t, s)$ satisfies
  \begin{eqnarray*}
    K_{x, y} (t, s) & = & \sigma^2_{S_0} +  \int_{\tau = 0}^t
    \int_{\sigma = 0}^s \left( \sigma_A^2 \mathbb{E}_{(Z_x, Z_y) \sim
    \mathcal{N} (0,  \Sigma_{x, y}^{} (t, s))} [\varphi (Z_x) \varphi (Z_y)] +
    \sigma_b^2 \right) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma\\
    & = & \sigma^2_{S_0} +  \int_{\tau = 0}^t \int_{\sigma =
    0}^s (\sigma_A^2 \Phi (\Sigma_{x, y}^{} (t, s)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{ \Dot{y}_{\sigma}}_{\R^d}   d \tau d \sigma
  \end{eqnarray*}
  with
  \[ \Sigma_{x, y}^{} (t, s) = \left(\begin{array}{c}
       K_{x, x} (t, t), K_{x, y} (t, s)\\
       K_{x, y} (t, s), K_{y, y} (s, s)
     \end{array}\right) \]
\end{proposition}

The proof will rely on classic arguments used to prove convergence of Euler schemes to CDE solutions (see \cite{FrizVictoir} and \cite{EulerGoursat}).
Our setting is more complex than the ones we found in the literature though, this is due to the presence of two "independent" driving signals and on the unique nature of the driving fields, which not only depend on the "present" but also on "past" and "future". 
This complex dependency structure of the driving fields makes them completely non-local and requires more involved arguments for the solution to be made sense of.

\subsubsection{Case $x = y$}

Note that due to their definition as limiting kernels the $\tilde{\Sigma}^{\mathcal{D} \times
\mathcal{D}}_{x \comma x}$ are always PSD.

\begin{proposition}
  $\forall t \in \mathcal{D}. \quad \Tilde{K}^{\mathcal{D} \times \mathcal{D}}_{x, x}
  (t, t) \geq \sigma_{S_0}^2 $\quad for any choiche of $\mathcal{D}$.
\end{proposition}

\begin{proof}
  We have
  \[ K^{\mathcal{D} \times \mathcal{D}}_{x, x} (t_m, t_m) = \sigma^2_{S_0} +
     \sum_{\tmscript{\begin{array}{c}
       0 \leq k_1 < m\\
       0 \leq k_2 < m
     \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 \Phi \left(
     \Sigma_{\tmscript{x, x}}^{\mathcal{D} \times \mathcal{D}} (t_{k_1}, t_{k_2})
     \right) + \sigma_b^2 \right) \Delta^{\mathcal{D}} x_{{t_{k_1 + 1}} }^k
     \Delta^{\mathcal{D}} x_{t_{k_2 + 1}}^k \]
  and by Tensor Programs we know that
\begin{equation*}
\resizebox{\hsize}{!}{$
\begin{gathered}
\sum_{\tmscript{\begin{array}{c}
       0 \leq k_1 < m\\
       0 \leq k_2 < m
     \end{array}}} \sum_{k = 1}^d \left( \sigma_A^2 \Phi \left(
     \Sigma_{\tmscript{x, x}}^{\mathcal{D} \times \mathcal{D}} (t_{k_1}, t_{k_2})
     \right) + \sigma_b^2 \right) \Delta^{\mathcal{D}} x_{{t_{k_1 + 1}} }^k
     \Delta^{\mathcal{D}} x_{t_{k_2 + 1}}^k = \lim_{N \rightarrow \infty}
     \mathbb{E} \left[ \frac{\langle S_x^{N, \mathcal{D}} (x) - S^N_0, S_x^{N,
     \mathcal{D}} (x) - S^N_0 \rangle}{N} \right] \geq 0 
\end{gathered}
$}
\end{equation*}
  
  
  \ 
\end{proof}

\begin{lemma}
  There is a constant $C_x > 0$ independent of $\mathcal{D}$ such that
  \[ \| \tilde{K}^{\mathcal{D} \times \mathcal{D}}_{x \comma x} \|_{\infty,
     [0, 1] \times [0, 1]} \assign \sup_{(t, s) \in [0, 1]^2} |
     \tilde{K}^{\mathcal{D} \times \mathcal{D}}_{x \comma x} (t, s) | \leq C_x
  \]
\end{lemma}

\begin{proof}
  Wlog $(t, s) \in \left[ t_m {, t_{m + 1}}  \right) \times [s_n, s_{n + 1})$. Remember how
  \begin{eqnarray*}
    \tilde{K}^{\mathcal{D} \times \mathcal{D}}_{x \comma x} (t, s) & = &
    K^{\mathcal{D} \times \mathcal{D}}_{x \comma x} (t_m, s_n)\\
    & = & \sigma^2_{S_0} +  \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma =
    0} \left( \sigma_A^2 \Phi \left(
    \tilde{\Sigma}_{\tmscript{x, x}}^{\mathcal{D} \times \mathcal{D}} (\tau, \sigma) \right)
    + \sigma_b^2 \right)
    \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}   
    d\tau d\sigma
  \end{eqnarray*}
  thus
  \begin{eqnarray*}
    | \tilde{K}_{t, s} | & \leq & 
    \sigma^2_{S_0} + 
    \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    | \sigma_A^2 \Phi (\tilde{\Sigma}_{ \tau, \sigma})| 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma
    + \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    | \sigma_b^2 | 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma \\
    & = & \sigma^2_{S_0} + 
    \sigma_b^2 \norm{x}_{1-var, [0,t_m]}\norm{x}_{1-var, [0,s_n]} +
    \sigma_A^2 \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    |\Phi(\tilde{\Sigma}_{ \tau, \sigma})|  
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma \\
    & \leq & \sigma^2_{S_0} + 
    \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
    \tilde{M} 
    \tmscript{\left(
    1 + \sqrt{\tilde{K}_{\tau, \tau}} \right) \left( 1 +
    \sqrt{\tilde{K}_{\sigma, \sigma}} \right)} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma\\
    & = & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \tilde{M} 
    \tmscript{\left( \int^{t_m}_{\tau = 0} \left( 1 +
    \sqrt{\tilde{K}_{\tau, \tau}} \right) |\Dot{x}_{\tau}| d\tau \right) 
    \left(\int^{s_n}_{\sigma = 0} \left( 1 + \sqrt{\tilde{K}_{\sigma, \sigma}}
    \right)  |\Dot{x}_{\sigma}| d\sigma \right)}
  \end{eqnarray*}
  In particular
  \begin{eqnarray*}
    \tilde{K}_{t, t} = | \tilde{K}_{t, t} | & \leq & \sigma^2_{S_0} +
    \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} + \sigma_A^2 \tilde{M}
    \left| \int^{t_m}_{\tau = 0} \left( 1 +
    \sqrt{\tilde{K}_{\tau, \tau}} \right) |\Dot{x}_{\tau}| d\tau
    \right|^2\\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    \sigma_A^2 \tilde{M}  \| x \|_{1 - \tmop{var}, [0, t_m]}
    \tmscript{
    \left( \int^{t_m}_{\tau = 0} \left( 1 + \sqrt{\tilde{K}_{\tau, \tau}}
    \right)^2 |\Dot{x}_{\tau}| d\tau \right)}\\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    2 \sigma_A^2 \tilde{M} \| x \|_{1 - \tmop{var}, [0, 1]} 
    \int^{t_m}_{\tau = 0} (1 + \tilde{K}_{\tau, \tau}) 
    |\Dot{x}_{\tau}| d\tau \\
    & \leq & \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0, 1]} +
    2 \sigma_A^2 \tilde{M} \| x \|_{1 - \tmop{var}, [0, 1]}
    \int^t_{\tau = 0} (1 + \tilde{K}_{\tau, \tau}) 
    |\Dot{x}_{\tau}| d\tau
  \end{eqnarray*}
  
  
  and we can use Gronwall Inequality (\cite{FrizVictoir}, Lemma 3.2) to
  obtain
  \begin{eqnarray*}
    1 + \tilde{K}_{t, t} & \leq & (1 + \sigma^2_{S_0} + \sigma_b^2 \| x
    \|^2_{1 - \tmop{var}, [0, 1]}) \exp \{ 2 \sigma_A^2 \tilde{M} \| x \|^2_{1
    - \tmop{var}, [0, 1]} \}
  \end{eqnarray*}
  hence the thesis with
  \begin{eqnarray*}
    C_x & = & (1 + \sigma^2_{S_0} + \sigma_b^2 \| x \|^2_{1 - \tmop{var}, [0,
    1]}) {e^{2 \sigma_A^2 \tilde{M} \| x \|^2_{1 - \tmop{var}, [0, 1]}}}  - 1
  \end{eqnarray*}
  
\end{proof}

\begin{corollary}
  There is an $R \in \mathbb{R}$ such that $\tilde{\Sigma}^{\mathcal{D} \times
  \mathcal{D}}_{x \comma x}, \Sigma^{\mathcal{D} \times \mathcal{D}}_{x \comma
  x} \in \tmop{PSD} (R)$ for every $\mathcal{D}$.
\end{corollary}

\begin{proof}
  The diagonal elements $K^{\mathcal{D} \times \mathcal{D}}_{t , t }$ are
  bounded above by a common constant $C_x$ and below by $\sigma^2_{S_0}$.
\end{proof}

We are ready to prove {\tmstrong{Proposition.\ref{simple_conv}}} in the case
$x = y$

\begin{proof}
  We have
  \begin{eqnarray*}
    | K^{\mathcal{D} \times \mathcal{D}}_{t , s } - \tilde{K}^{\mathcal{D}
    \times \mathcal{D}}_{t , s} | 
    & = &
     \tmscript{\left| \int^t_{\tau = 0} \int^s_{\sigma = 0} 
     (\sigma_A^2 \Phi (\tilde{\Sigma}_{ \tau, \sigma}) + \sigma_b^2) 
     \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
     d\tau d\sigma
     - \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} 
     (\sigma_A^2 \Phi (\tilde{\Sigma}_{ \tau, \sigma}) + \sigma_b^2) 
    \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
    d\tau d\sigma \right|}\\
    & = & \left| \int_{\Omega_{t, s}} (
    \sigma_A^2 \Phi (\tilde{\Sigma}_{\tau, \sigma}) + \sigma_b^2) 
    \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
    d\tau d\sigma \right|
  \end{eqnarray*}
  with $\Omega_{t, s} \assign [0, t] \times [0, s] \setminus [0, t_m] \times [0, s_n]$. 
  
  Note that
  $\Omega_{t, s} \subseteq ([t_{m,} t_{m + 1}] \times [0, 1]) \cup ([0, 1]
     \times [s_n, s_{n + 1}]) $ thus
  $\mathcal{L}^2 (\Omega_{t, s}) \leq | \mathcal{D} | + | \mathcal{D} | =
     2 | \mathcal{D} | $
  and
  \begin{eqnarray*}
    | K^{\mathcal{D} \times \mathcal{D}}_{t , s } - \tilde{K}^{\mathcal{D}
    \times \mathcal{D}}_{t , s} | & \leq & \int_{\Omega_{t, s}} | \sigma_A^2
    \Phi (\tilde{\Sigma}_{ \tau, \sigma}) + \sigma_b^2 |  
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|  
    d\tau d\sigma\\
    & \leq & \sigma_A^2 \int_{\Omega_{t, s}} \tilde{M} \left( 1 +
    \sqrt{\tilde{K}_{\tau, \tau}} \right) \left( 1 + \sqrt{\tilde{K}_{\sigma,
    \sigma}} \right)  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|      
    d\tau d\sigma\\
    &  & + \sigma_b^2 \int_{\Omega_{t, s}} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
    & \leq & \sigma_A^2 \tilde{M} \left( 1 + \sqrt{C_x} \right)^2
    \int_{\Omega_{t, s}} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma + \sigma_b^2
    \int_{\Omega_{t, s}} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
    & = & (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2) \int_{[0, 1] \times
    [0, 1]} \mathbb{I}_{\Omega_{t, s}} (\tau, \sigma) 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
    & \leq & (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2) 
    \sqrt{\mathcal{L}^2(\Omega_{t, s})}
    \sqrt{\int_{[0, 1] \times [0, 1]} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|^2       
    d\tau d\sigma}\\
    & \leq & \textcolor{orange}{(2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2) \
    \sqrt{\mathcal{L}^2(\Omega_{t, s})}
    \int_0^1 |\Dot{x}_t|^2 dt }\\
    & \leq & 2 (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2) 
    \sqrt{|\mathcal{D}|}
   \norm{x}^2_{W^{1,2}}
  \end{eqnarray*}
  
  In particular as $| \mathcal{D} | \rightarrow 0$ we have
  \[ \sup_{[0, 1] \times [0, 1]} | K^{\mathcal{D} \times \mathcal{D}}_{t , s
     } - \tilde{K}^{\mathcal{D} \times \mathcal{D}}_{t , s} |  \rightarrow 0 \]
  
  
  Consider now another partition $\check{\mathcal{D}}$, we have
  \begin{eqnarray*}
    | K^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{t , s } -
    K^{\mathcal{D} \times \mathcal{D}}_{t , s} | 
    & = &
    \left| \sigma_A^2
    \int^t_{\tau = 0} \int^s_{\sigma = 0} 
    [\Phi(\tilde{\Sigma}^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{\tau, \sigma})
    - \Phi (\tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}}_{  \tau,\sigma})] 
    \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
    d\tau d\sigma \right|\\
    & \leq & \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} | \Phi
    (\tilde{\Sigma}^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{  \tau,
    \sigma}) - \Phi (\tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}}_{  \tau,
    \sigma}) |  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
    & \leq & \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} k_R |
    \tilde{\Sigma}^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{  \tau,
    \sigma} - \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma}
    |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
    & \leq & \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{  \tau,
    \sigma} - \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{  \tau,
    \sigma} |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
    &  & + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{  \tau, \sigma} -
    \Sigma^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma} |_{\infty} | d x
    _{\tau} | \cdot | d x _{\sigma} |\\
    &  & + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma} -
    \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma}
    |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
    & \leq & \sigma_A^2 2 (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2) 
    \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\mathcal{D}}|}
    \int^t_{\tau = 0} \int^s_{\sigma = 0}  
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|
    d\tau d\sigma\\
    &  & + \sigma_A^2 k_R 
    \int^t_{\tau = 0} \int^s_{\sigma = 0} 
    |\Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{\tau, \sigma}
    - \Sigma^{\mathcal{D} \times \mathcal{D}'}_{\tau, \sigma} |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|
    d\tau d\sigma\\
    &  & + \sigma_A^2 2 (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2)
    \norm{x}^2_{W^{1,2}} 
    \sqrt{|{\mathcal{D}}|}
    \int^t_{\tau = 0} \int^s_{\sigma = 0} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|
    d\tau d\sigma\\
    & \leq & 4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2) 
    \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\mathcal{D}} | \vee |\mathcal{D} |}\\
    &  & + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma =
    0} | \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{  \tau,
    \sigma} - \Sigma^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma}
    |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{eqnarray*}
  thus
  \begin{eqnarray*}
    \Xi_t \assign \sup_{0 \leq \tau, \sigma \leq t} |
    \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  \tau, \sigma}
    - \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  \tau, \sigma} |_{\infty} &
    \leq & 4 \sigma_A^2 \left( 2 \sigma_A^2 \tilde{M} \left( {1 + C_x} 
    \right) + \sigma_b^2 \right) 
    \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\mathcal{D}} | \vee |\mathcal{D} |}\\
    &  & + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^t_{\sigma =
    0} | \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}}_{  \tau,
    \sigma} - \Sigma^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma}
    |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{eqnarray*}
  and since
  \begin{eqnarray*}
    & \int^t_{\tau = 0} \int^t_{\sigma = 0} | \Sigma^{\check{\mathcal{D}}
    \times \check{\mathcal{D}}}_{  \tau, \sigma} - \Sigma^{\mathcal{D} \times
    \mathcal{D}}_{  \tau, \sigma} |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma
    \leq \int^t_{\tau = 0} \int^t_{\sigma = 0} \Xi_{\tau \vee
    \sigma} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma & \\
    & = \int^t_{\tau = 0} \int^{\tau}_{\sigma = 0} \Xi_{\tau} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|d\tau d\sigma
    + \int^t_{\tau = 0} \int^t_{\sigma = \tau}
    \Xi_{\sigma} |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}| d\tau d\sigma & \\
    & \leq  \int^t_{\tau = 0}  \| x \|_{1 - \tmop{var},
    [0, \tau]} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
    +  \int^t_{\sigma = 0} \int^{\sigma}_{\tau = 0} 
    \Xi_{\sigma} 
    |\Dot{x}_{\tau} | |\Dot{x}_{\sigma} | d\tau d\sigma 
    & \\
    & = \int^t_{\tau = 0}  \| x \|_{1 - \tmop{var},
    [0, \tau]} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
    + \int^t_{\sigma = 0}  \| x \|_{1 - \tmop{var},
    [0, \sigma]} \Xi_{\sigma} |\Dot{x}_{\sigma} | d\sigma  & \\
    & \leq 2 \| x \|_{1 - \tmop{var}, [0, 1]} 
     \int^t_{\tau = 0} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau & 
  \end{eqnarray*}
  we get
  \begin{eqnarray*}
    {\Xi_t}  & \leq & 4 \sigma_A^2 \left( 2 \sigma_A^2 \tilde{M} \left( {1 + C_x} 
    \right) + \sigma_b^2 \right) 
    \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\mathcal{D}} | \vee |\mathcal{D} |}\\
    &  & + 2 \sigma_A^2 k_R \| x \|_{1 - \tmop{var}, [0, 1]} 
    \int^t_{\tau = 0} \Xi_{\tau} |\Dot{x}_{\tau} | d\tau 
  \end{eqnarray*}
  thus, by Gronwall,
  \[ \Xi_t \leq 4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2)
     \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\mathcal{D}} | \vee |\mathcal{D} |}
      \cdot e^{2 \sigma_A^2 k_R \| x \|_{1 - \tmop{var}, [0, 1]}
     \| x \|_{1 - \tmop{var}, [0, t]}} \]
  hence
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \| K^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{t , s } -
     K^{\mathcal{D} \times \mathcal{D}'}_{t , s} \|_{\infty, [0, 1]^2} \leq 4
     \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_x) + \sigma_b^2) 
     \| x \|^2_{1 - \tmop{var}, [0, 1]} \norm{x}^2_{W^{1,2}} 
    \sqrt{|\check{\mathcal{D}} | \vee |\mathcal{D} |}
    \cdot
     e^{2 \sigma_A^2 k_R \| x \|^2_{1 - \tmop{var}, [0, 1]}} 
  \end{gathered} $} \end{equation*}
  This means that given any sequence of partitions $\{ \mathcal{D}_n \}$ with $|
  \mathcal{D}_n | \rightarrow 0$ we have
  \[ \{ K^{\mathcal{D}_n \times \mathcal{D}_n}_{t , s} \} \tmop{is} a
     \tmop{Cauchy} \tmop{sequence} \tmop{in} (C^0 ([0, 1] \times [0, 1] ;
     \mathbb{R}), \| \cdot \|_{\infty}) 
    \]
  and the limit $K_{t, s}$ does not depend on the sequence (i.e. the limit
  exists and is \tmcolor{orange}{unique})
  
  Since PSD matrices form a closed set the matrices $\Sigma_{x, x} (t, s)$
  obtained as limits are all PSD  (actually all $\tmop{PSD} (R)$).
  
  Let the limit be $K_{t, s}$ and let us prove it to be a solution of the PDE:
  \begin{eqnarray*}
    & \left| K_{t, s} - \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma =
    0}^s (\sigma_A^2 \Phi (\Sigma_{\tau, \sigma}^{}) + \sigma_b^2) 
    \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
    d\tau d\sigma
    \right| & \\
    \leq & | K_{t, s} - K^{\mathcal{D} \times \mathcal{D}}_{t , s} | +
    \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} | \Phi
    (\tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma}) - \Phi
    (\Sigma_{\tau, \sigma}^{}) |  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma & \\
    \leq & o (1) + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma} -
    \Sigma_{\tau, \sigma}^{} |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       
    d\tau d\sigma& \\
    \leq & o (1) + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}}_{  \tau, \sigma} -
    \Sigma^{\mathcal{D} \times \mathcal{D}}_{\tau, \sigma} |_{\infty}  
    |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       
    d\tau d\sigma & \\
    & + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\mathcal{D} \times \mathcal{D}}_{\tau, \sigma} - \Sigma_{\tau,
    \sigma}^{} |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma & \\
    = & o (1) + o (1) + o (1) = o (1) & 
  \end{eqnarray*}
  thus
  \[ \left| K_{t, s} - \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma = 0}^s
     (\sigma_A^2 \Phi (\Sigma_{\tau, \sigma}^{}) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
    d\tau d\sigma  \right| = 0 \]
  i.e
  \[ K_{t, s} = \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma = 0}^s
     (\sigma_A^2 \Phi (\Sigma_{\tau, \sigma}^{}) + \sigma_b^2) 
     \sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}   
    d\tau d\sigma  \]
  
\end{proof}

\subsubsection{Case $x \neq y$}

Now we can assume the kernels $K^{\mathcal{D} \times \mathcal{D}}_{x \comma
x}$, $K_{x \comma x}$ and $K^{\mathcal{D}' \times \mathcal{D}'}_{y \comma y}$,
$K_{y \comma y}$ to be given for all partitions $\mathcal{D}, \mathcal{D}'$.

\begin{remark}
  Once again the maps $\Sigma^{\mathcal{D} \times \mathcal{D}'}_{x \comma y}$
  are  PSD since they arise as such from Tensor limiting arguments, in particular
  \begin{eqnarray*}
    \nobracket | \nobracket \tilde{K}^{\mathcal{D} \times \mathcal{D}'}_{x
    \comma y} (t, s) | \leq \sqrt{\tilde{K}^{\mathcal{D} \times
    \mathcal{D}}_{x \comma x} (t, t) \tilde{K}^{\mathcal{D}' \times
    \mathcal{D}'}_{y \comma y} (s, s)} \leq \sqrt{C_x C_y} \leq C_x \vee C_y 
    &  & 
  \end{eqnarray*}
\end{remark}

thus there exists $C_{x, y}$ such that independently from $\mathcal{D} \times
\mathcal{D}'$ and for any $\alpha, \beta \in \{ x, y \}$ it holds
\[ \sup_{0 \leq t, s \leq 1} \nobracket | \nobracket K^{\mathcal{D}^{(')} \times
   \mathcal{D}^{(')}}_{\alpha \comma \beta} (t, s) | \leq C_{x, y} \]
Moreover, since membership in $\tmop{PSD} (R)$ only depends on the diagonal
elements, there is some $R = R_{x,y} = R_x \vee R_y \in \mathbb{R}$ such that for all $0 \leq t, s \leq
1$
\[ \Sigma^{\mathcal{D} \times \mathcal{D}'}_{x \comma y} (t, s) \in \tmop{PSD}
   (R_{x,y}) \]
We are now ready to prove {\tmstrong{Proposition.\ref{simple_conv}}} in the
case $x \neq y$

\begin{proof}
  We have
  \begin{eqnarray*}
    | K^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t, s) -
    \tilde{K}^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t, s) | & = & |
    \nobracket \int^t_{\tau = 0} \int^s_{\sigma = 0} (\sigma_A^2 \Phi
    (\widetilde{\Sigma }^{\mathcal{D} \times \mathcal{D}'}_{ x, y} (\tau,
    \sigma)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma\\
    &  & - \int^{t_m}_{\tau = 0} \int^{s_n}_{\sigma = 0} (\sigma_A^2 \Phi
    (\widetilde{\Sigma }^{\mathcal{D} \times \mathcal{D}'}_{ x, y} (\tau,
    \sigma)) + \sigma_b^2) \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma | \nobracket\\
    & = & \left| \int_{\Omega_{t, s}} (\sigma_A^2 \Phi (\widetilde{\Sigma
    }^{\mathcal{D} \times \mathcal{D}'}_{ x, y} (\tau, \sigma)) + \sigma_b^2)
    \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma \right|
  \end{eqnarray*}
  with
  \[ \Omega_{t, s} \assign [0, t] \times [0, s] \setminus [0, t_m] \times [0,
     s_n] \]
  Note that
  \[ \Omega_{t, s} \subseteq ([t_{m,} t_{m + 1}] \times [0, 1]) \cup ([0, 1]
     \times [s_n, s_{n + 1}]) \]
  thus
  \[ \mathcal{L}^2 (\Omega_{t, s}) \leq | \mathcal{D} | + | \mathcal{D}' |
     \leq 2 (| \mathcal{D} | \vee | \mathcal{D}' |) \]
  hence
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    | K^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t, s) -
    \tilde{K}^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t, s) |  \leq 
    \int_{\Omega_{t, s}} | \sigma_A^2 \Phi (\widetilde{\Sigma }^{\mathcal{D}
    \times \mathcal{D}'}_{ x, y} (\tau, \sigma)) + \sigma_b^2 |  |\sprod{\Dot{x}_{\tau}}{\Dot{x}_{\sigma}}_{\R^d}|       d\tau d\sigma
    \\
     \leq  \sigma_A^2 \int_{\Omega_{t, s}} \tilde{M} 
    \tmscript{\left( 1 +
    \sqrt{K^{\mathcal{D} \times \mathcal{D}}_{x, x} (\tau \comma \tau)}
    \right) \left( 1 + \sqrt{K^{\mathcal{D}' \times \mathcal{D}'}_{y, y}
    (\sigma \comma \sigma)} \right)} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma
       + \sigma_b^2 \int_{\Omega_{t, s}} 
       |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
       d\tau d\sigma\\
     \leq  \sigma_A^2 \tilde{M} \left( 1 + \sqrt{C_{x, y}} \right)^2
    \int_{\Omega_{t, s}} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
    d\tau d\sigma 
    + \sigma_b^2
    \int_{\Omega_{t, s}} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|      
    d\tau d\sigma\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) \int_{[0, 1]
    \times [0, 1]} \mathbb{I}_{\Omega_{t, s}} (\tau, \sigma) 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       
    d\tau d\sigma\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\int_{[0, 1] \times [0, 1]} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|^2       
    d\tau d\sigma}\\
    \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\int_{[0, 1] \times [0, 1]} 
    |\Dot{x}_{\tau}|^2 |\Dot{y}_{\sigma}|^2       
    d\tau d\sigma}\\
     \leq  (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{\mathcal{L}^2 (\Omega_{t, s})}
    \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}}\\
     \leq  2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\mathcal{D} | \vee | \mathcal{D}' |} 
     \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}}
  \end{gathered} $} \end{equation*}
  
  In particular as $(| \mathcal{D} | \vee | \mathcal{D}' |) \rightarrow 0$ we
  have
    \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \sup_{[0, 1] \times [0, 1]} | K^{\mathcal{D} \times \mathcal{D}'}_{x, y}
     (t, s) - \tilde{K}^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t, s) | \leq
     2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)   
     \sqrt{|\mathcal{D} | \vee | \mathcal{D}' |} 
     \sqrt{\norm{x}^2_{W^{1,2}}\norm{y}^2_{W^{1,2}}} \rightarrow 0
     \end{gathered} $} \end{equation*}
  
  
  and, since this holds with the same type of constant for $K^{\mathcal{D} \times
  \mathcal{D}}_{x, x}$and $K^{\mathcal{D}' \times \mathcal{D}'}_{y, y}$, we have
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
  \sup_{[0, 1] \times [0, 1]} | \Sigma^{\mathcal{D} \times \mathcal{D}'}_{ 
     x, y} (t, s) - \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}'}_{  x, y}
     (t, s) |_{\infty} \leq 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) +
     \sigma_b^2) 
     \sqrt{|\mathcal{D} | \vee | \mathcal{D}' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
     \end{gathered} $} \end{equation*}
  Consider now another partition $\check{\mathcal{D}} \times
  \check{\mathcal{D}}'$, we have
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    | K^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{x, y} (t, s) -
    K^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t, s) |  =  \left|
    \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} [\Phi
    (\tilde{\Sigma}^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  x, y}
    (\tau, \sigma)) - \Phi (\tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}'}_{
    x, y} (\tau, \sigma))] \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}        d\tau d\sigma 
    \right|\\
     \leq  \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} | \Phi
    (\tilde{\Sigma}^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  x, y}
    (\tau, \sigma)) - \Phi (\tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}'}_{
    x, y} (\tau, \sigma)) |  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} k_R |
    \tilde{\Sigma}^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  x, y}
    (\tau, \sigma) - \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}'}_{  x, y}
    (\tau, \sigma) |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  \tau,
    \sigma} - \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{ 
    \tau, \sigma} |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  \tau, \sigma}
    - \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  \tau, \sigma} |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  \tau, \sigma} -
    \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}'}_{  \tau, \sigma}
    |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  \sigma_A^2 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\check{\mathcal{D}} | \vee | \check{\mathcal{D}}'|}  
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    \int^t_{\tau = 0} \int^s_{\sigma = 0}  
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  \tau, \sigma}
    - \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  \tau, \sigma} |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
       + \sigma_A^2 2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\mathcal{D} | \vee | \mathcal{D}' |}
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
     \int^t_{\tau = 0} \int^s_{\sigma = 0} 
     |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma\\
     \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2) 
     \sqrt{|\check{\mathcal{D}} | \vee | \check{\mathcal{D}}'| \vee | \mathcal{D} | \vee | \mathcal{D}' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    {\| x \|_{1 - \tmop{var}, [0, 1]} \| y \|_{1 -\tmop{var}, [0, 1]}} 
    \\
       + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma =
    0} | \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  x, y}
    (\tau, \sigma) - \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  x, y} (\tau,
    \sigma) |_{\infty} |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{gathered} $} \end{equation*}
  thus
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \Xi^{x, y}_t \assign \sup_{0 \leq \tau, \sigma \leq t} |
    \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  \tau, \sigma}
    - \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  \tau, \sigma} |_{\infty} \\
    \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\mathcal{D}} | \vee | \check{\mathcal{D}}'| \vee | \mathcal{D} | \vee | \mathcal{D}' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    {\| x \|_{1 - \tmop{var}, [0, 1]} \| y \|_{1 -\tmop{var}, [0, 1]}} \\
       + \tmcolor{black}{\sigma_A^2 k_R \int^t_{\tau = 0} \int^t_{\sigma =
    0} | \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  \tau,
    \sigma} - \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  \tau, \sigma}|_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma}
  \end{gathered} $} \end{equation*}
  and since
  \begin{eqnarray*}
    & \int^t_{\tau = 0} \int^t_{\sigma = 0} 
    | \Sigma^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{  \tau, \sigma} 
    - \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  \tau, \sigma} |_{\infty} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma 
    \leq \int^t_{\tau = 0} \int^t_{\sigma = 0} {\Xi^{x, y}_{\tau
    \vee \sigma}}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma & \\
    & = \int^t_{\tau = 0} \int^{\tau}_{\sigma = 0} 
    \Xi^{x, y}_{\tau} 
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma 
    + \int^t_{\tau = 0} \int^t_{\sigma =\tau} 
    \Xi^{x, y}_{\sigma}
    |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma & \\
    & \leq 
    \int^t_{\tau = 0} \| y \|_{1 - \tmop{var}, [0, \tau]} 
    \Xi^{x, y}_{\tau} |\Dot{x}_{\tau}| d\tau 
    +  \int^t_{\sigma = 0} \int^{\sigma}_{\tau = 0} 
    \Xi^{x, y}_{\sigma} 
    |\Dot{x}_{\tau}| |\Dot{y}_{\sigma}| d\tau  d\sigma  & \\
    & = \int^t_{\tau = 0} \| y \|_{1 - \tmop{var}, [0, \tau]} 
    \Xi^{x, y}_{\tau} |\Dot{x}_{\tau}| d\tau 
    +  \int^t_{\sigma = 0} \| x \|_{1 - \tmop{var}, [0, \sigma]} 
    \Xi^{x,y}_{\sigma} |\Dot{y}_{\sigma}| d\sigma & \\
    & \leq (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1 - \tmop{var},[0, 1]}) 
    \int^t_{\tau = 0} \Xi^{x, y}_{\tau} (|\Dot{x}_{\tau}| +|\Dot{y}_{\tau}|) d\tau  & 
  \end{eqnarray*}
  we get
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
    \Xi^{x, y}_t  \leq  4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\mathcal{D}} | \vee | \check{\mathcal{D}}'| \vee | \mathcal{D} | \vee | \mathcal{D}' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    {\| x \|_{1 - \tmop{var}, [0, 1]} \| y \|_{1 -\tmop{var}, [0, 1]}}\\
     + 2 \sigma_A^2 k_R (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1
    - \tmop{var}, [0, 1]}) \int^t_{\tau = 0} \Xi^{x, y}_{\tau} (|\Dot{x}_{\tau}| +|\Dot{y}_{\tau}|) d\tau
  \end{gathered} $} \end{equation*}
  thus, by Gronwall,
  \begin{eqnarray*}
    \Xi_t & \leq & 4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\mathcal{D}} | \vee | \check{\mathcal{D}}'| \vee | \mathcal{D} | \vee | \mathcal{D}' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    {\| x \|_{1 - \tmop{var}, [0, 1]} \| y \|_{1 -\tmop{var}, [0, 1]}}\\
    &  & \cdot e^{2 \sigma_A^2 k_R (\| x \|_{1 - \tmop{var}, [0, 1]} \vee \|
    y \|_{1 - \tmop{var}, [0, 1]}) {(\| x \|_{1 - \tmop{var},
    [0, t]} + \| y \|_{1 - \tmop{var}, [0, t]})}}
  \end{eqnarray*}
  hence
  \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
     \| K^{\check{\mathcal{D}} \times \check{\mathcal{D}}'}_{x, y} (t, s) -
    K^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t, s) \|_{\infty, [0, 1]^2} \leq
    \\
    4 \sigma_A^2 (2 \sigma_A^2 \tilde{M} (1 + C_{x, y}) + \sigma_b^2)
    \sqrt{|\check{\mathcal{D}} | \vee | \check{\mathcal{D}}'| \vee | \mathcal{D} | \vee | \mathcal{D}' |} 
     (\norm{x}^2_{W^{1,2}} \vee \norm{y}^2_{W^{1,2}})
    {\| x \|_{1 - \tmop{var}, [0, 1]} \| y \|_{1 -\tmop{var}, [0, 1]}}
    \cdot e^{{4 \sigma_A^2 k_R (\| x
    \|_{1 - \tmop{var}, [0, 1]} \vee \| y \|_{1 - \tmop{var}, [0, 1]})}} 
  \end{gathered} $} \end{equation*}
  
  Once again this means that, given any sequence of partitions $\{ \mathcal{D}_n \times
  \mathcal{D}'_n \}$ with $| \mathcal{D}_n | \vee | \mathcal{D}_n' |
  \rightarrow 0$, we have
  \[ \{ K^{\mathcal{D}_n \times \mathcal{D}'_n}_{x , y} \} \tmop{is} a
     \tmop{Cauchy} \tmop{sequence} \tmop{in} (C^0 ([0, 1] \times [0, 1] ;
     \mathbb{R}), \| \cdot \|_{\infty}) \]
  and the limit $K_{x, y}$ does not depend on the sequence (i.e. the limit
  exists and is \tmcolor{orange}{unique})
  
  Since PSD matrices form a closed set the matrices $\Sigma_{x, y} (t, s)$
  obtained as limits using the previous result are all PSD, moreover all
  $\tmop{PSD} (R)$!
  
  Let us prove $K_{x, y}$ to be a solution of the PDE:
 \begin{equation*} \resizebox{\hsize}{!}{$ \begin{gathered}
     \left| K_{x, y} (t, s) - \sigma^2_{S_0} + \int_{\tau = 0}^t
    \int_{\sigma = 0}^s (\sigma_A^2 \Phi (\Sigma_{x, y}^{} (\tau, \sigma)) +
    \sigma_b^2) 
    \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma   \right|  \\
    \leq  | K_{x, y} (t, s) - K^{\mathcal{D} \times \mathcal{D}'}_{x, y} (t,
    s) | + \sigma_A^2 \int^t_{\tau = 0} \int^s_{\sigma = 0} | \Phi
    (\tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}'}_{  x, y} (\tau, \sigma))
    - \Phi (\Sigma_{x, y}^{} (\tau, \sigma)) |  
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma  \\
    \leq  o (1) + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}'}_{  x, y} (\tau, \sigma) -
    \Sigma_{x, y}^{} (\tau, \sigma) |_{\infty} 
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma\\
    \leq  o (1) + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \tilde{\Sigma}^{\mathcal{D} \times \mathcal{D}'}_{  x, y} (\tau, \sigma) -
    \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  x, y} (\tau, \sigma)
    |_{\infty}  |\sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}|       d\tau d\sigma  \\
     + \sigma_A^2 k_R \int^t_{\tau = 0} \int^s_{\sigma = 0} |
    \Sigma^{\mathcal{D} \times \mathcal{D}'}_{  x, y} (\tau, \sigma) -
    \Sigma_{x, y}^{} (\tau, \sigma) |_{\infty}  
    | \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d} |    d\tau d\sigma \\
    =  o (1) + o (1) + o (1) = o (1)  
   \end{gathered} $} \end{equation*}
  thus
  \[ \left| K_{x, y} (t, s) - \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma
     = 0}^s (\sigma_A^2 \Phi (\Sigma_{x, y}^{} (\tau, \sigma)) + \sigma_b^2) 
     \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma\right| = 0 \]
  i.e
  \[ K_{x, y} (t, s) = \sigma^2_{S_0} + \int_{\tau = 0}^t \int_{\sigma = 0}^s
     (\sigma_A^2 \Phi (\Sigma_{x, y}^{} (\tau, \sigma)) + \sigma_b^2) 
     \sprod{\Dot{x}_{\tau}}{\Dot{y}_{\sigma}}_{\R^d}     d\tau d\sigma\]
  
\end{proof}

